FlowShield: cryptocurrency anti-money laundering with transaction semantics parsing and fund flow tracking

Cryptocurrency anti-money laundering (Crypto AML) is increasingly challenged by sophisticated laundering behaviors that rapidly fragment stolen assets through diverse semantics and across multiple blockchains. Existing Crypto AML methods often simplify transaction semantics, rely on topology-centric signals, or output isolated detection labels. In this paper, we present \textsc{FlowShield}, a Crypto AML framework for transaction-level laundering detection and investigator-facing report generation. \textsc{FlowShield} first recovers behavior-level semantics from observable relations, making laundering intents explicit. To trace value provenance and redistribution, \textsc{FlowShield} reconstructs fund-flow subgraphs from three complementary perspectives. It then employs a text--structure fusion mechanism, enabling the interplay between large language model (LLM)-encoded semantics and flow texts with graph convolutional network (GCN)-encoded structure. Beyond mere detection, \textsc{FlowShield} further generates readable suspicious activity reports (SARs), offering investigators concise summaries and explainable red flags. To address the data scarcity in multi-chain detection, we construct and open-source \textit{BybitML}, the first public multi-chain laundering dataset. We evaluate \textsc{FlowShield} on \textit{BybitML} and two public laundering datasets and experimental results demonstrate that \textsc{FlowShield} achieves the best overall performance, with an average F1 score of 98.0\%. Further behavior and SAR analyses demonstrate that \textsc{FlowShield} can reveal diverse laundering strategies and produce readable reports for investigating complex multi-hop fund flows.

==> Alg/construct_alg.tex <==
% \begin{algorithm}[]
% \caption{Semantics Awareness}
% \DontPrintSemicolon
% \KwIn{Transaction set $\mathcal{T}$, parsing rules $\mathcal{R}_{swp}$, $\mathcal{R}_{ind}$, $\mathcal{R}_{crs}$, semantics template text ${Tmp}_{s}$}

% \KwOut{Semantics type $T_s$ and semantics text $Txt_{sem}$ for each transaction}

% \For{each transaction $tx_{h_i,j}$ in $\mathcal{T}$}{
%     \uIf{$\mathcal{R}_{swp}(tx_{h_i,j})$}{
%         $f_{sem}(tx_{h_i,j}) = T_{swp}$
%     }
%     \uElseIf{$\mathcal{R}_{ind}(tx_{h_i,j})$}{
%         $f_{sem}(tx_{h_i,j}) = T_{ind}$
%     }
%     \uElseIf{$\mathcal{R}_{crs}(tx_{h_i,j})$}{
%         $f_{sem}(tx_{h_i,j}) = T_{crs}$
%     }
%     \Else{
%         $f_{sem}(tx_{h_i,j}) = T_{dir}$
%     }
%     Generate semantics text via the template ${Tmp}_{s}$.}
% \label{alg:semantics}
% \end{algorithm}

\begin{algorithm}[t]
\caption{Fund Flow Awareness}
% \footnotesize
\small
\DontPrintSemicolon

\label{alg:flow_awareness}

\KwIn{Transaction MultiDiGraph $G $; flow template ${\mathsf{Tmp}}_{f}$; time window 
$\tau_t$, flow ratio $\tau_f$, and amount similarity $\tau_a$}
\KwOut{Upstream subgraph $SubG_{up}$, downstream subgraph $SubG_{down}$, parallel subgraph $SubG_{para}$, flow type $\text{T}_f$, and flow text $\mathsf{Txt}_{flow}$ for each transaction}

\For{each transaction edge $e_{tg} \in E$}{
    \tcp{\textcolor{teal}{Upstream subgraph extraction}}
    % $C_{in} \leftarrow$ incoming transactions to $e_{tg}(from)$ in $G$ before $e_{tg}(time)$ \;
    $C_{in} \leftarrow \mathrm{GetUpCandi}(G, e_{tg}, \tau_t)$ \;
    $\text{Tx}_{up} \leftarrow \{\mathrm{MatchTokenAmount}(C_{in}, e_{tg}, \tau_f) \}$\;
    % $U \leftarrow$ matchAmount($U$, $\tau_f$ \cdot amount$)$\;
    $SubG_{up} \leftarrow$ Subgraph induced by $\text{Tx}_{up} \cup \{ e_{tg} \}$\;
    
    \tcp{\textcolor{teal}{Downstream subgraph extraction}}
    % $C_{out} \leftarrow$ outgoing transactions from $e_{tg}(to)$ in $G$ after $e_{tg}(time)$ \;
    $C_{out} \leftarrow \mathrm{GetDwCandi}(G, e_{tg}, \tau_t)$ \;
    $\text{Tx}_{down} \leftarrow \{\mathrm{MatchTokenAmount}(C_{out}, e_{tg}, \tau_f)\}$\;
    $SubG_{down} \leftarrow$ subgraph induced by $\text{Tx}_{down}  \cup \{ e_{tg} \}$\;
    
    \tcp{\textcolor{teal}{Parallel subgraph extraction}}
    $C_{para} \leftarrow \mathrm{GetPaCandi}(G, e_{tg}, \tau_t)$ \;
    $\text{Tx}_{para}  \leftarrow \{\mathrm{MatchSimilarAmount}(C_{para}, e_{tg}, \tau_a)\}$\;
    $SubG_{para} \leftarrow$ subgraph induced by $\text{Tx}_{para} \cup \{ e_{tg} \}$\;
    
    % \tcp{\textcolor{teal}{Flow type classification}}
    % $sumA_{down} \leftarrow \sum_{e \in \text{Tx}_{down}} e(amount)$\;
    % \uIf{$ sumA_{down} \ge \tau_f \times e_{tg}(amount) $}{
    %     \uIf{$|\text{Tx}_{down}| = 1$}{$\text{T}_f \leftarrow$ single outflow}
    %     \Else{$\text{T}_f \leftarrow$ entire disperse}
    % }
    % \uElseIf{$|\text{Tx}_{para}| > 0$ \textbf{and} $sumA_{down} \ge e_{tg}(amount)$}{
    %     $\text{T}_f \leftarrow$ mix
    % }
    % \uElseIf{$|\text{Tx}_{down}| > 1$ \textbf{and} $sumA_{down} \le \tau_f \times e_{tg}(amount)$}{
    %     $\text{T}_f \leftarrow$ partial disperse
    % }
    % \uElseIf{$|Tx_{down}| = 0$}{
    %     $\text{T}_f \leftarrow$ no forward
    % }

        \tcp{\textcolor{teal}{Flow type classification}}
    $A_{\text{down}} \leftarrow \sum_{e \in \text{Tx}_{down}} e(\text{amount})$\;
    
    \uIf{$|\text{Tx}_{down}| = 0$}{
        $\text{T}_f \leftarrow$ No forward\;
    }
    \uElseIf{$|\text{Tx}_{\text{para}}| > 0$ \textbf{and} $A_{\text{down}} \ge e_{tg}(\text{amount})$}{
        $\text{T}_f \leftarrow$ Mix\;
    }
    \uElseIf{$A_{\text{down}} \ge \tau_f \cdot e_{tg}(\text{amount})$}{
        \uIf{$|\text{Tx}_{down}| = 1$}{
            $\text{T}_f \leftarrow$ Single outflow\;
        }
        \Else{
            $\text{T}_f \leftarrow$ Entire disperse\;
        }
    }
    \ElseIf{$|\text{Tx}_{down}| > 1$ \textbf{and} $A_{\text{down}} < \tau_f \cdot e_{tg}(\text{amount})$}{
        $\text{T}_f \leftarrow$ Partial disperse\;
    }

    
    \tcp{\textcolor{teal}{Flow text generation}}
    Use ${\text{Tmp}}_{f}$ with Tx information, and $\text{T}_f$ to generate flow text\;
}
\end{algorithm}


==> Alg/semantics_alg.tex <==
% \begin{algorithm}[t]
% \caption{Semantics Awareness}\footnotesize
% \DontPrintSemicolon
% \SetAlFnt{\scriptsize}
% \SetInd{0.3em}{0.3em}
% \SetAlgoNlRelativeSize{-1}
% \SetAlgoInsideSkip{small}
% \KwIn{Transaction set $\mathcal{T}$, parsing rules $\mathcal{R}_{swp}$, $\mathcal{R}_{ind}$, $\mathcal{R}_{crs}$, semantics template text ${Tmp}_{s}$}

% \KwOut{Semantics type $T_s$ and semantics text $Txt_{sem}$ for each transaction}

% % \ForEach{$tx_{h_i,j} \in \mathcal{T}$}{
% \For{each transaction $tx_{h_i,j}$ in $\mathcal{T}$}{
%     \uIf{$\mathcal{R}_{swp}(tx_{h_i,j})$}{
%         $f_{sem}(tx_{h_i,j}) = T_{swp}$
%     }
%     \uElseIf{$\mathcal{R}_{ind}(tx_{h_i,j})$}{
%         $f_{sem}(tx_{h_i,j}) = T_{ind}$
%     }
%     \uElseIf{$\mathcal{R}_{crs}(tx_{h_i,j})$}{
%         $f_{sem}(tx_{h_i,j}) = T_{crs}$
%     }
%     \Else{
%         $f_{sem}(tx_{h_i,j}) = T_{dir}$
%     }
%     % --- Generate semantic text ---
%     Generate semantics text via the template ${Tmp}_{s}$ and transaction information.}
% \label{alg:semantics}
% \end{algorithm}


\begin{algorithm}[]
\caption{Semantic Awareness}
\DontPrintSemicolon
\KwIn{Transaction set $\mathcal{T}$, parsing rules $\mathcal{R}_{swp}$, $\mathcal{R}_{ind}$, $\mathcal{R}_{crs}$, semantics template ${\mathsf{Tmp}}_{s}$}

\KwOut{Semantics type $\mathsf{T}_s$ and semantics text $\mathsf{Txt}_{sem}$ for each transaction}

\For{each transaction $\mathsf{tx}_{h_i}^j$ in $\mathcal{T}$}{
    \uIf{$\mathcal{R}_{swp}(\text{tx}_{h_i}^j)$}{
        $\text{f}_{sem}(\text{tx}_{h_i}^j) = \text{T}_{swp}$
    }
    \uElseIf{$\mathcal{R}_{ind}(\text{tx}_{h_i}^j)$}{
        $\text{f}_{sem}(\text{tx}_{h_i}^j) = \text{T}_{ind}$
    }
    \uElseIf{$\mathcal{R}_{crs}(\text{tx}_{h_i}^j)$}{
        $\text{f}_{sem}(\text{tx}_{h_i}^j) = \text{T}_{crs}$
    }
    \Else{
        $\text{f}_{sem}(\text{tx}_{h_i}^j) = \text{T}_{dir}$
    }
    Generate semantics text via the template ${\text{Tmp}}_{s}$.}
\label{alg:semantics}
\end{algorithm}





==> Tabs/tab_comparative_exp.tex <==
\begin{table*}[t]
\centering
%Effectiveness comparison with different AML methods on Bybit Hack datasets.
\caption{F1 scores (\%) of different methods on \textit{Bybit-EC}. Baselines include heuristic (Cyclic, XBlock), traditional machine learning  (MLP, LR, SVM), and graph learning (GCN, SAGE, Tracer), as well as the LLM-based method (Llama3).  \circledc{1} to \circledc{14} denote the data of \textit{Bybit-EC} from the first day to the fourteenth day. $\mathbf{F1}_{\text{avg}}$ denotes the mean F1 score across all 14 days for each method.}
\label{tab:avg_f1}
\resizebox{\textwidth}{!}{
\begin{tabular}{c c c c c c c c c c c c c c c c}
\toprule
\multicolumn{1}{c}{\textbf{Methods}} & $\mathbf{F1}_{\text{avg}}$ & \circled{1} & \circled{2} & \circled{3} & \circled{4} & \circled{5} & \circled{6} & \circled{7} & \circled{8} & \circled{9} & \circled{10} & \circled{11} & \circled{12} & \circled{13} & \circled{14} \\
\midrule
Cyclic~\cite{lv2023detection}     & 6.9 & 4.7 & 6.7 & 6.9 & 6.6 & 11.4 & 9.9 & 9.9 & 8.3 & 9.3 & 8.1 & 5.6 & 2.7 & 3.4 & 2.7 \\
XBlock~\cite{wu2023towards}     & 16.7 & 35.2 & 31.3 & 38.4 & 35.8 & 16.9 & 18.8 & 10.4 & 17.7 & 24.5 & 0.9 & 2.1 & 0.5 & 0.3 & 1.2 \\
\cmidrule{2-16}
MLP~\cite{rosenblatt1958perceptron}        & 53.0 & 50.3 & 59.0 & 68.9 & 66.3 & 65.8 & 67.6 & 58.3 & 49.9 & 48.0 & 72.8 & 52.6 & 13.9 & 34.0 & 34.2 \\
LR~\cite{cox1958regression}         & 65.0 & 69.3 & 76.1 & 67.5 & 70.4 & 87.7 & 87.1 & 88.5 & 67.1 & 79.8 & 83.1 & 80.4 & 0.0 & 34.4 & 18.2 \\
SVM~\cite{cortes1995support}        & 60.7 & 68.4 & 77.4 & 68.9 & 70.6 & 86.4 & 86.5 & 87.8 & 66.5 & 78.3 & 83.2 & 75.9 & 0.0 & 0.0 & 0.0 \\
\cmidrule{2-16}
GCN~\cite{kipf2016semi}        & 80.2 & 85.2 & 84.6 & 78.6 & 78.7 & 94.8 & 93.4 & 95.3 & 88.2 & 92.2 & 91.3 & 77.2 & 59.5 & 50.8 & 52.5 \\
SAGE~\cite{hamilton2017inductive}  & 87.3 & 89.0 & 88.1 & 86.0 & 91.4 & 96.7 & 91.0 & 96.1 & 94.3 & 95.2 & 92.7 & 89.6 & 72.5 & 63.5 & 76.4 \\
Tracer~\cite{wu2023tracer}     & 21.9 & 19.1 & 31.6 & 36.8 & 27.7 & 14.0 & 16.4 & 10.0 & 18.5 & 32.3 & 23.9 & 20.2 & 21.3 & 25.9 & 8.8 \\
\cmidrule{2-16}
% Llama3~\cite{grattafiori2024llama}      & $\underline{91.2}$ & $\underline{93.0}$ & $\underline{92.8}$ & $\underline{92.6 }$& $\underline{93.1}$ & $\underline{98.1}$ & $\underline{97.3}$ & $\underline{98.0}$ & $\underline{96.1}$ & $\underline{97.0}$ & $\underline{95.1}$ & $\underline{94.6}$ & $\underline{73.5}$ & $\underline{74.4}$ & $\underline{80.8}$ \\
Llama3~\cite{grattafiori2024llama}      & ${91.2}$ & ${93.0}$ & $ {92.8}$ & $ {92.6 }$& $ {93.1}$ & $ {98.1}$ & $ {97.3}$ & $ {98.0}$ & $ {96.1}$ & $ {97.0}$ & $ {95.1}$ & $ {94.6}$ & $ {73.5}$ & $ {74.4}$ & $ {80.8}$ \\
\midrule
\rowcolor{gray!10}
% \textbf{FlowShield} & \textbf{97.4\gain{6.2}} & \textbf{98.3\gain{5.3}} & \textbf{97.9\gain{5.1}} & \textbf{97.8\gain{5.2}} & \textbf{98.7\gain{5.6}} & \textbf{99.4\gain{1.3}} & \textbf{99.5\gain{2.2}} & \textbf{99.6\gain{1.6}} & \textbf{99.3\gain{3.2}} & \textbf{99.4\gain{2.4}} & \textbf{99.0\gain{3.9}} & \textbf{97.6\gain{3.0}} & \textbf{93.1\gain{19.6}} & \textbf{90.2\gain{15.8}} & \textbf{93.1\gain{12.3}} \\

\textbf{FlowShield} & \textbf{97.4\gain{6}} & \textbf{98.3\gain{5}} & \textbf{97.9\gain{5}} & \textbf{97.8\gain{5}} & \textbf{98.7\gain{6}} & \textbf{99.4\gain{1}} & \textbf{99.5\gain{2}} & \textbf{99.6\gain{2}} & \textbf{99.3\gain{3}} & \textbf{99.4\gain{2}} & \textbf{99.0\gain{4}} & \textbf{97.6\gain{3}} & \textbf{93.1\gain{20}} & \textbf{90.2\gain{16}} & \textbf{93.1\gain{12}} \\
\bottomrule
\end{tabular}
}
\end{table*}



==> Tabs/tab_comparative_precision.tex <==
\begin{table*}[ht]
\centering
\caption{Effectiveness comparison with different AML methods on Bybit Hack datasets. Baselines include heuristic rules (Cyclic, XBlock, Tracer), traditional machine learning models (MLP, LR, SVM), and graph learning models (GCN, SAGE), as well as the LLM-based method (Llama).  \circledc{1} to \circledc{14} indicate the dataset from the first day to the fourteenth day, and each value is the average F1 score (\%) over five runs. Avg. denotes the mean F1 score across all 14 datasets for each method.}
\resizebox{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c c c}
\toprule
Methods & Avg. & \circled{1} & \circled{2} & \circled{3} & \circled{4} & \circled{5} & \circled{6} & \circled{7} & \circled{8} & \circled{9} & \circled{10} & \circled{11} & \circled{12} & \circled{13} & \circled{14} \\
\midrule
Cyclic~\cite{lv2023detection}     & 6.87 & 4.7 & 6.7 & 6.9 & 6.6 & 11.4 & 9.9 & 9.9 & 8.3 & 9.3 & 8.1 & 5.6 & 2.7 & 3.4 & 2.7 \\
XBlock~\cite{wu2023towards}     & 16.7 & 35.2 & 31.3 & 38.4 & 35.8 & 16.9 & 18.8 & 10.4 & 17.7 & 24.5 & 0.9 & 2.1 & 0.5 & 0.3 & 1.2 \\
\midrule
MLP~\cite{rosenblatt1958perceptron}        & 53.0 & 50.3 & 59.0 & 68.9 & 66.3 & 65.8 & 67.6 & 58.3 & 49.9 & 48.0 & 72.8 & 52.6 & 13.9 & 34.0 & 34.2 \\
LR~\cite{cox1958regression}         & 65.0 & 69.3 & 76.1 & 67.5 & 70.4 & 87.7 & 87.1 & 88.5 & 67.1 & 79.8 & 83.1 & 80.4 & 0.0 & 34.4 & 18.2 \\
SVM~\cite{cortes1995support}        & 60.7 & 68.4 & 77.4 & 68.9 & 70.6 & 86.4 & 86.5 & 87.8 & 66.5 & 78.3 & 83.2 & 75.9 & 0.0 & 0.0 & 0.0 \\
\midrule
GCN~\cite{kipf2016semi}        & 80.2 & 85.2 & 84.6 & 78.6 & 78.7 & 94.8 & 93.4 & 95.3 & 88.2 & 92.2 & 91.3 & 77.2 & 59.5 & 50.8 & 52.5 \\
SAGE~\cite{hamilton2017inductive}  & 87.3 & 89.0 & 88.1 & 86.0 & 91.4 & 96.7 & 91.0 & 96.1 & 94.3 & 95.2 & 92.7 & 89.6 & 72.5 & 63.5 & 76.4 \\
Tracer~\cite{wu2023tracer}     & 21.9 & 19.1 & 31.6 & 36.8 & 27.7 & 14.0 & 16.4 & 10.0 & 18.5 & 32.3 & 23.9 & 20.2 & 21.3 & 25.9 & 8.8 \\
\midrule
Llama3~\cite{grattafiori2024llama}      & 91.2 & 93.0 & 92.8 & 92.6 & 93.1 & 98.1 & 97.3 & 98.0 & 96.1 & 97.0 & 95.1 & 94.6 & 73.5 & 74.4 & 80.8 \\
\midrule
\textbf{FlowShield} & \textbf{97.4} & \textbf{98.3} & \textbf{97.9} & \textbf{97.8} & \textbf{98.7} & \textbf{99.4} & \textbf{99.5} & \textbf{99.6} & \textbf{99.3} & \textbf{99.4} & \textbf{99.0} & \textbf{97.6} & \textbf{93.1} & \textbf{90.2} & \textbf{93.1} \\
\bottomrule
\end{tabular}}
\end{table*}



==> Tabs/tab_comparision_methods.tex <==
% \begin{table}
% \centering
% \tiny
% % \caption{Comparison of existing Crypto AML methods. \staricon~represents the number of transaction semantics the method is aware of; \LEFTcircle~represents the method with explainable design but without explainable result.}
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Method} & \textbf{Semantic Awareness} & \textbf{Cross-chain Capability} & \textbf{Result Explainability} & \textbf{Open Artifacts} \\
% \midrule
% CyclicML~\cite{lv2023detection} & \staricon & \redx & \LEFTcircle & \redx \\
% XBlockFlow~\cite{wu2023towards} & \staricon & \redx & \LEFTcircle & \redx \\
% MixerFunc~\cite{kuccuk2023investigation} & \staricon & \redx & \LEFTcircle & \redx \\
% Elliptic++~\cite{elmougy2023demystifying} & \staricon & \redx & \redx & \greencheck \\
% FraudLens~\cite{nicholls2023fraudlens} & \staricon & \redx & \redx & \redx \\
% DensFlow~\cite{lin2024denseflow} & \staricon & \redx & \greencheck & \greencheck \\
% Tracer~\cite{wu2023tracer} & \staricon\staricon & \redx & \greencheck & \greencheck \\
% \rowcolor{gray!10}
% \techName{} & \staricon\staricon\staricon\staricon & \greencheck & \greencheck & \greencheck \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of existing Crypto AML methods. \staricon~represents the number of transaction semantics the method is aware of; \LEFTcircle~represents the method with explainable design but without explainable result.}
% \label{tab:aml_comparison}
% \end{table}
% %为什么这个caption和表格的距离那么近？


% \usepackage{caption} % 导入caption宏包
% \captionsetup[table]{skip=6pt} % 控制caption与表格的距离，6pt可以改大

% \begin{table}
% \centering
% \tiny
% \setlength{\tabcolsep}{4pt} % 调整列间距
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Method} & 
% \textbf{Semantic\newline Awareness} & 
% \textbf{Cross-chain\newline Capability} & 
% \textbf{Result\newline Explainability} & 
% \textbf{Open\newline Artifacts} \\
% \midrule
% CyclicML~\cite{lv2023detection} & \staricon & \redx & \LEFTcircle & \redx \\
% XBlockFlow~\cite{wu2023towards} & \staricon & \redx & \LEFTcircle & \redx \\
% MixerFunc~\cite{kuccuk2023investigation} & \staricon & \redx & \LEFTcircle & \redx \\
% Elliptic++~\cite{elmougy2023demystifying} & \staricon & \redx & \redx & \greencheck \\
% FraudLens~\cite{nicholls2023fraudlens} & \staricon & \redx & \redx & \redx \\
% DensFlow~\cite{lin2024denseflow} & \staricon & \redx & \greencheck & \greencheck \\
% Tracer~\cite{wu2023tracer} & \staricon\staricon & \redx & \greencheck & \greencheck \\
% \rowcolor{gray!10}
% \techName{} & \staricon\staricon\staricon\staricon & \greencheck & \greencheck & \greencheck \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of existing Crypto AML methods. \staricon~represents the number of transaction semantics the method is aware of; \LEFTcircle~represents the method with explainable design but without explainable result.}
% \label{tab:aml_comparison}
% \end{table}


% \begin{table}
% \centering
% % \footnotesize
% % %\small
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{lcccc}
% \toprule
% \thead{Method} &
% \thead{Semantic\\Awareness} &
% \thead{Fund Flow\\Awareness} &
% \thead{Result\\Explainability} &
% \thead{Open\\Artifacts} \\
% \midrule
% CyclicML~\cite{lv2023detection} & \staricon & \redx & \LEFTcircle & \redx \\
% XBlockFlow~\cite{wu2023towards} & \staricon & \redx & \LEFTcircle & \redx \\
% MixerFunc~\cite{kuccuk2023investigation} & \staricon & \redx & \LEFTcircle & \redx \\
% Elliptic++~\cite{elmougy2023demystifying} & \staricon & \greencheck & \redx & \greencheck \\
% FraudLens~\cite{nicholls2023fraudlens} & \staricon & \greencheck & \redx & \redx \\
% DensFlow~\cite{lin2024denseflow} & \staricon & \redx & \redx & \greencheck \\
% Tracer~\cite{wu2023tracer} & \staricon\staricon & \greencheck  & \LEFTcircle & \greencheck \\
% \rowcolor{gray!10}
% \techName{} & \staricon\staricon\staricon\staricon & \greencheck & \greencheck & \greencheck \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of existing Crypto AML methods. \staricon~represents the number of transaction semantics the method is aware of; \LEFTcircle~represents the method with explainable design but without explainable result.}
% \label{tab:aml_comparison}
% \end{table}


% \begin{table}
% \centering
% \caption{Comparison of existing Crypto AML methods. \directicon~represents Direct Transfer; 
% \indirectswap~represents Indirect Transfer; 
% \faRetweet~represents Token Swap; 
% \faExchange~represents Cross-chain Transfer; \LEFTcircle~represents the method with an explainable design but without explainable results.  \qw{extend this table}}
% % \footnotesize
% % %\small
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{lcccc}
% \toprule
% \thead{Method} &
% \thead{Semantic\\Awareness} &
% \thead{Fund Flow\\Awareness} &
% \thead{Result\\Explainability} \\
% \midrule



% Cyclic~\cite{lv2023detection} & \directicon & \redx & \LEFTcircle  \\
% XBlock~\cite{wu2023towards} &  \directicon & \redx & \LEFTcircle \\
% MixerFunc~\cite{kuccuk2023investigation} &  \directicon & \redx & \LEFTcircle \\
% Elliptic++~\cite{elmougy2023demystifying} &  \directicon & \greencheck & \redx \\
% FraudLens~\cite{nicholls2023fraudlens} &  \directicon& \greencheck & \redx  \\
% DensFlow~\cite{lin2024denseflow} &  \directicon & \redx & \redx  \\
% Tracer~\cite{wu2023tracer} &  \directicon\faRetweet & \greencheck  & \LEFTcircle  \\
% \rowcolor{gray!10}
% \techName{} & \directicon \indirectswap \faRetweet \faExchange & \greencheck & \greencheck  \\
% \bottomrule
% \end{tabular}

% \label{tab:aml_comparison}
% \end{table}

\begin{table*}[t]
\centering
\caption{Comparison of representative Crypto AML methods.}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cc|cccc|cc}
\toprule
\multirow{2}{*}{\textbf{Crypto AML}} 
& 
\multirow{2}{*}{\textbf{Method}} 
& \multicolumn{2}{c}{\textbf{Blockchain}} 
& \multicolumn{4}{c}{\textbf{Laundering techniques}} 
& \multirow{2}{*}{\makecell[c]{\textbf{Laundering}\\\textbf{flow}}}  
& \multirow{2}{*}{\makecell[c]{\textbf{Explainable}\\\textbf{result}}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-8}
 &  & UTXO & Account & Direct transfer & Token swap & Indirect swap & Cross-chain &  &  \\
\midrule
Elliptic++\cite{elmougy2023demystifying} & Machine learning &  \greencheck& \redx &  \greencheck& \redx & \redx & \redx &  \greencheck& \redx \\
FraudLens\cite{nicholls2023fraudlens} & Graph-based       &  \greencheck& \redx &  \greencheck& \redx & \redx & \redx & \redx & \redx \\
MixerFunc\cite{kuccuk2023investigation} & Heuristic     &  \greencheck& \redx &  \greencheck& \redx & \redx & \redx & \redx & \redx \\
Cyclic\cite{lv2023detection}    & Heuristic     & \redx     &  \greencheck&  \greencheck& \redx & \redx & \redx & \redx & \redx \\
XBlock\cite{wu2023towards}   & Heuristic     & \redx     &  \greencheck&  \greencheck& \redx & \redx & \redx & \redx & \redx \\
DenseFlow\cite{lin2024denseflow} & Graph-based       & \redx     &  \greencheck&  \greencheck& \redx & \redx & \redx & \redx & \redx \\
Tracer\cite{wu2023tracer}    & Graph-based       & \redx     &  \greencheck&  \greencheck&  \greencheck& \redx & \redx &  \redx  & \redx \\
\midrule
\rowcolor{gray!10}
 \techName{}  & Graph + LLM    &  \greencheck&  \greencheck&  \greencheck&  \greencheck&  \greencheck&  \greencheck&  \greencheck&  \greencheck\\
\bottomrule
\end{tabular}
\label{tab:aml_comparison}
}
\end{table*}


% \begin{table*}[t]
% \centering
% \caption{Comparison of representative Crypto AML methods.}
% \begin{tabular}{l l cccccccc}
% \toprule
% \textbf{Crypto AML} & \textbf{Method} & \multicolumn{2}{c}{\textbf{Blockchain}} & \multicolumn{4}{c}{\textbf{Laundering techniques}} & \textbf{Laundering flow} & \textbf{Explainable result} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-8}
%  &  & UTXO & Account & Direct transfer & Token swap & Indirect swap & Cross-chain &  &  \\
% % \midrule
% Elliptic++ & Machine learning & \greencheck  & \greencheck  & \greencheck  & \redx & \redx & \redx & \greencheck  & \redx \\
% FraudLens & Graph-based       & \greencheck  & \redx      & \greencheck  & \redx & \redx & \redx & \redx & \redx \\
% MixerFunc & Heuristic rule    & \greencheck  & \redx      & \greencheck  & \redx & \redx & \redx & \redx & \redx \\
% % \midrule
% Cyclic    & Heuristic rule    & \redx      & \greencheck  & \greencheck  & \redx & \redx & \redx & \redx & \redx \\
% XBlock    & Heuristic rule    & \redx      & \greencheck  & \greencheck  & \redx & \redx & \redx & \greencheck  & \redx \\
% % \midrule
% DenseFlow & Graph-based       & \redx      & \greencheck  & \greencheck  & \redx & \redx & \redx & \greencheck  & \redx \\
% Tracer    & Graph-based       & \greencheck  & \greencheck  & \greencheck  & \greencheck  & \greencheck & \greencheck & \greencheck  & \greencheck  \\
% \bottomrule
% \end{tabular}
% \end{table*}


==> Tabs/tab_effectiveness_avg.tex <==
% \begin{table}[ht]
% \centering
% \caption{Average Precision, Recall, and F1 score (\%) of different methods on BybitHack datasets.}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Method} & \textbf{P} & \textbf{R} & \textbf{F1} \\
% \midrule
% Cyclic    & 6.3  & 8.4  & 6.9  \\
% XBlock  & 75.2  & 9.9  & 16.7  \\
% \midrule
% MLP         & 74.0  & 48.1  & 53.0  \\
% LR          & 67.3  & 66.9  & 65.0  \\
% SVM         & 60.4  & 62.8  & 60.7  \\
% \midrule
% GCN         & 77.0  & 86.3  & 80.2  \\
% SAGE   & 82.1  & 95.4  & 87.3  \\
% Tracer      & 52.3  & 15.3  & 21.9  \\
% \midrule
% Llama3    & 94.6  & 88.4  & 91.2  \\
% \textbf{FlowShield} & \textbf{98.3} & \textbf{96.7} & \textbf{97.4} \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[]
% \centering
% \caption{Average Precision, Recall, F1 score, and MCR (\%) of different methods on 14-day BybitHack dataset.}\label{tab:avg_metrics}
% \begin{tabular}{ccccc}
% \toprule
% \multicolumn{1}{c}{\textbf{Methods}} & $\mathbf{P}_{\text{avg}}$
%  & $\mathbf{R}_{\text{avg}}$
%  & $\mathbf{F1}_{\text{avg}}$
%  & $\mathbf{MCR}_{\text{avg}}$
%  \\
% \midrule
% Cyclic & 6.3  & 8.4  & 6.9  &$\approx 0.0$
%  \\
% XBlock & 75.2 & 9.9  & 16.7 & $\approx 0.0$
%  \\
% \cmidrule{2-5}
% MLP & 74.0 & 48.1 & 53.0 & 76.2 \\
% LR & 67.3 & 66.9 & 65.0 & 49.7 \\
% SVM & 60.4 & 62.8 & 60.7 & 59.0 \\
% \cmidrule{2-5}
% GCN & 77.0 & 86.3 & 80.2 & 70.0 \\
% SAGE & 82.1 & $\underline{95.4}$ & 87.3 &  \textbf{97.4} \\
% Tracer & 52.3 & 15.3 & 21.9 & $\approx 0.0$ \\
% \cmidrule{2-5}
% Llama3 &$\underline{94.6}$ & 88.4 & $\underline{91.2}$ & 72.4 \\
% \midrule
% \textbf{FlowShield} & \textbf{98.3} & \textbf{96.7} & \textbf{97.4} & $\underline{88.0}$ \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[t]
% \centering
% \caption{Average Precision, Recall, F1 score, and MCR (\%) of different methods on \textit{Bybit-EC}.}
% \label{tab:avg_metrics_ec}
% \begin{tabular}{ccccc}
% \toprule
% \textbf{Method} 
%  & $\mathbf{P}_{\text{avg}}$
%  & $\mathbf{R}_{\text{avg}}$
%  & $\mathbf{F1}_{\text{avg}}$
%  & $\mathbf{MCR}_{\text{avg}}$ \\
% \midrule
% Cyclic & 6.3  & 8.4  & 6.9  & $\approx 0$ \\
% XBlock & 75.2 & 9.9  & 16.7 & $\approx 0$ \\
% \cmidrule{1-5}
% MLP    & 74.0 & 48.1 & 53.0 & 76.2 \\
% LR     & 67.3 & 66.9 & 65.0 & 49.7 \\
% SVM    & 60.4 & 62.8 & 60.7 & 59.0 \\
% \cmidrule{1-5}
% GCN    & 77.0 & 86.3 & 80.2 & 70.0 \\
% SAGE   & 82.1 & 95.4 & 87.3 & 97.4 \\
% Tracer & 52.3 & 15.3 & 21.9 & $\approx0$ \\
% \cmidrule{1-5}
% Llama3 & 94.6 & 88.4 & 91.2 & 72.4 \\
% \midrule
% \rowcolor{gray!10}
% \textbf{Ours}
%  & \textbf{98.3\gain{3.7}}
%  & \textbf{96.7\gain{8.3}}
%  & \textbf{97.4\gain{6.2}}
%  & \textbf{88.0} \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Average Precision, Recall, F1 score, and MCR (\%) of different methods on \textit{Bybit-BC}.}
% \label{tab:avg_metrics_bc}
% \begin{tabular}{ccccc}
% \toprule
% \textbf{Method} 
%  & $\mathbf{P}_{\text{avg}}$
%  & $\mathbf{R}_{\text{avg}}$
%  & $\mathbf{F1}_{\text{avg}}$
%  & $\mathbf{MCR}_{\text{avg}}$ \\
% \midrule
% Cyclic & 1.0 & 0.5 & 0.7 & $\approx 0$ \\
% XBlock & \multicolumn{4}{c}{Not applicable to Bitcoin} \\
% \cmidrule{1-5}
% MLP    & 58.7 & 54.8 & 55.8 & 59.5 \\
% LR     & 60.0 & 79.9 & 68.5 & 81.1 \\
% SVM    & 60.4 & 82.5 & 69.7 & 84.3 \\
% \cmidrule{1-5}
% GCN    & 73.0 & 93.6 & 81.7 & 97.0 \\
% SAGE   & 82.5 & 94.5 & 88.1 & 91.1 \\
% Tracer & \multicolumn{4}{c}{Not applicable to Bitcoin} \\
% \cmidrule{1-5}
% Llama3 & 83.4 & 80.7 & 82.1 & 96.0 \\
% \midrule
% \rowcolor{gray!10}
% \textbf{Ours}
%  & \textbf{97.5\gain{14.1}}
%  & \textbf{96.8\gain{2.3}}
%  & \textbf{97.2\gain{9.1}}
%  & \textbf{98.2\gain{1.2}} \\
% \bottomrule
% \end{tabular}
% \end{table}


\begin{table}[t]
\small
\centering
\caption{Performance of different methods on \textit{Bybit-EC} and \textit{Bybit-BC}. The best and runner-up results are in bold and underline, respectively.}
\label{tab:avg_metrics}
% \resizebox{0.46\textwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}
  & \multicolumn{4}{c}{\textbf{\textit{Bybit-EC}}}
  & \multicolumn{4}{c}{\textbf{\textit{Bybit-BC}}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
 & $\mathbf{P}$
 & $\mathbf{R}$
 & $\mathbf{F1}$
 & $\mathbf{MCR}$
 & $\mathbf{P}$
 & $\mathbf{R}$
 & $\mathbf{F1}$
 & $\mathbf{MCR}$ \\
\midrule
Cyclic & 6.3  & 8.4  & 6.9  & $\approx 0$ & 1.0 & 0.5 & 0.7 & $\approx0.0$ \\
XBlock & 75.2 & 9.9  & 16.7 & $\approx 0$ & \multicolumn{4}{c}{not applicable to Bitcoin} \\
\cmidrule{2-9}
MLP    & 74.0 & 48.1 & 53.0 & 76.2          & 58.7 & 54.8 & 55.8 & 59.5  \\
LR     & 67.3 & 66.9 & 65.0 & 49.7          & 60.0 & 79.9 & 68.5 & 81.1 \\
SVM    & 60.4 & 62.8 & 60.7 & 59.0          & 60.4 & 82.5 & 69.7 & 84.3 \\
\cmidrule{2-9}
GCN    & 77.0 & 86.3 & 80.2 & 70.0         & 73.0 & 93.6 & 81.7 & \underline{97.0}\\
SAGE   & 82.1 & \underline{95.4} & 87.3 &  \textbf{97.4}         & 82.5 & \underline{94.5} & \underline{88.1} & 91.1 \\
Tracer & 52.3 & 15.3 & 21.9 & $\approx0.0$ &  \multicolumn{4}{c}{not applicable to Bitcoin} 
 \\
\cmidrule{2-9}
Llama3 & \underline{94.6} & 88.4 & \underline{91.2} & 72.4        & \underline{83.4} & 80.7 & 82.1 & 96.0 \\
\midrule
\rowcolor{gray!10}
\textbf{Ours}
 & \textbf{98.3}
 & \textbf{96.7} &\textbf{ 97.4} & \underline{88.0}
 & \textbf{97.5}
 & \textbf{96.8}
 & \textbf{97.2}
 & \textbf{98.2} \\

\bottomrule
\end{tabular}
% }
\end{table}


% \begin{table*}[t]
% \centering
% \caption{Average Precision, Recall, F1 score, and MCR (\%) of different methods on \textit{Bybit-EC} and \textit{Bybit-BC}.}
% \label{tab:avg_metrics}
% % \resizebox{0.46\textwidth}{!}{
% \begin{tabular}{ccccccccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}
%   & \multicolumn{4}{c}{\textbf{\textit{Bybit-EC}}}
%   & \multicolumn{4}{c}{\textbf{\textit{Bybit-BC}}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%  & $\mathbf{P}_{\text{avg}}$
%  & $\mathbf{R}_{\text{avg}}$
%  & $\mathbf{F1}_{\text{avg}}$
%  & $\mathbf{MCR}_{\text{avg}}$
%  & $\mathbf{P}_{\text{avg}}$
%  & $\mathbf{R}_{\text{avg}}$
%  & $\mathbf{F1}_{\text{avg}}$
%  & $\mathbf{MCR}_{\text{avg}}$ \\
% \midrule
% Cyclic & 6.3  & 8.4  & 6.9  & $\approx 0$ & 1.0 & 0.5 & 0.7 & $\approx0.0$ \\
% XBlock & 75.2 & 9.9  & 16.7 & $\approx 0$ & \multicolumn{4}{c}{not applicable to Bitcoin} \\
% \cmidrule{2-9}
% MLP    & 74.0 & 48.1 & 53.0 & 76.2          & 58.7 & 54.8 & 55.8 & 59.5  \\
% LR     & 67.3 & 66.9 & 65.0 & 49.7          & 60.0 & 79.9 & 68.5 & 81.1 \\
% SVM    & 60.4 & 62.8 & 60.7 & 59.0          & 60.4 & 82.5 & 69.7 & 84.3 \\
% \cmidrule{2-9}
% GCN    & 77.0 & 86.3 & 80.2 & 70.0         & 73.0 & 93.6 & 81.7 & 97.0\\
% SAGE   & 82.1 & 95.4 & 87.3 & 97.4         & 82.5 & 94.5 & 88.1 & 91.1 \\
% Tracer & 52.3 & 15.3 & 21.9 & $\approx0.0$ &  \multicolumn{4}{c}{not applicable to Bitcoin} 
%  \\
% \cmidrule{2-9}
% Llama3 & 94.6 & 88.4 & 91.2 & 72.4        & 83.4 & 80.7 & 82.1 & 96.0 \\
% \midrule
% \rowcolor{gray!10}
% \textbf{Ours}
%  & \textbf{98.3\gain{3.7}}
%  & \textbf{96.7\gain{8.3}} &\textbf{ 97.4\gain{6.2}} & \textbf{88.0}
%  & \textbf{97.5\gain{14.1}}
%  & \textbf{96.8\gain{2.3}}
%  & \textbf{97.2\gain{9.1}}
%  & \textbf{98.2\gain{1.2}} \\


 
% \bottomrule
% \end{tabular}
% % }
% \end{table*}

% 98.3\gain{3.7}

 % & \textbf{$\overset{\gain{3.7}}{\textbf{98.3}}$}
 % & \textbf{96.7\gain{8.3}} &\textbf{ 97.4\gain{6.2}} & \textbf{88.0}
 % & \textbf{97.4\gain{4.9}} & \textbf{98.2\gain{1.9}} & \textbf{97.7\gain{3.4}} & \textbf{99.1\gain{0.6}} \\


  % & $\overset{\gain{3.7}}{\textbf{98.3}}$
 % & $\overset{\gain{8.3}}{\textbf{96.7}}$
 % & $\overset{\gain{6.2}}{\textbf{97.4}}$
 % & \textbf{88.0}
 % & $\overset{\gain{4.9}}{\textbf{97.4}}$
 % & $\overset{\gain{1.9}}{\textbf{98.2}}$
 % & $\overset{\gain{3.4}}{\textbf{97.7}}$
 % & $\overset{\gain{0.6}}{\textbf{99.1}}$ \\

==> Tabs/tab_wild_exp.tex <==
% \begin{table*}[ht]
% \centering
% \caption{\textbf{Comparison of same-day and in-the-wild detection performance of \textsc{FlowShield}.} 
% The model is trained on day \circledc{$t$} and tested on the same day 
% (Orig.) or the following day (Wild). }
% \begin{tabular}{c*{14}{c}}
% \toprule
% & \multicolumn{2}{c}{\circledc{6}} & \multicolumn{2}{c}{\circledc{7}} & \multicolumn{2}{c}{\circledc{8}} 
% & \multicolumn{2}{c}{\circledc{9}} & \multicolumn{2}{c}{\circledc{10}} & \multicolumn{2}{c}{\circledc{11}} & \multicolumn{2}{c}{\circledc{12}} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}
% & Orig. & Wild & Orig. & Wild & Orig. & Wild & Orig. & Wild & Orig. & Wild & Orig. & Wild & Orig. & Wild \\
% \midrule
% \textbf{R (\%)}   & 99.3 & 99.1 & 99.6 & 98.6 & 98.8 & 97.5 & 99.2 & 96.0 & 98.7 & 98.0 & 97.9 & 94.3 & 89.3 & 66.7 \\
% \textbf{MCR (\%)} & 97.9 & 98.1 & 95.7 & 83.4 & 99.3 & 99.1 & 99.5 & 94.7 & 94.6 & 91.7 & 99.9 & 98.6 & 97.7 & 96.6 \\
% \bottomrule
% \label{tab:wild}
% \end{tabular}
% \end{table*}


\begin{table}[t]
\centering
\small
\caption{\textbf{Same-day vs next-day detection performance of \textsc{FlowShield}.}
Train on Day~\circledc{$t$}, test on the same day (Orig.) or next day (Next.).}
\label{tab:wild}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{c c c c c}
\toprule
\textbf{Day} & \textbf{MCR Orig.} & \textbf{MCR Next.} & \textbf{F1 Orig.} & \textbf{F1 Next.} \\
\midrule
\circledc{6}  & 97.9 & 98.1 & 99.5 & 99.5 \\
\circledc{7}  & 95.7 & 83.4 & 99.6 & 99.3 \\
\circledc{8}  & 99.3 & 99.1 & 99.3 & 98.0 \\
\circledc{9}  & 99.5 & 94.7 & 99.4 & 97.8 \\
\circledc{10} & 94.6 & 91.7 & 99.0 & 98.4 \\
\circledc{11} & 99.9 & 98.6 & 97.6 & 96.3 \\
\circledc{12} & 97.7 & 96.6 & 93.1 & 66.3 \\
\bottomrule
\end{tabular}
\end{table}


% \begin{table}[t]
% \centering
% \small
% \caption{\textbf{Same-day vs next-day detection performance of \textsc{FlowShield}.}
% Train on Day~\circledc{$t$}, test on the same day (Orig.) or next day (Next.).}
% \label{tab:wild}
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{c c c c c}
% \toprule
% \textbf{Day} & \textbf{F1 Orig.} & \textbf{F1 Next.} & \textbf{MCR Orig.} & \textbf{MCR Next.} \\
% \midrule
% \circledc{6}  & 99.5 & 99.5 & 97.9 & 98.1 \\
% \circledc{7}  & 99.6 & 99.3 & 95.7 & 83.4 \\
% \circledc{8}  & 99.3 & 98.0 & 99.3 & 99.1 \\
% \circledc{9}  & 99.4 & 97.8 & 99.5 & 94.7 \\
% \circledc{10} & 99.0 & 98.4 & 94.6 & 91.7 \\
% \circledc{11} & 97.6 & 96.3 & 99.9 & 98.6 \\
% \circledc{12} & 93.1 & 66.3 & 97.7 & 96.6 \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[ht]
% \centering
% \small
% \caption{\textbf{Comparison of same-day and next-day detection performance of \textsc{FlowShield}.} 
% The model is trained on day \circledc{$t$} and tested on the same day 
% (Orig.) or the next day (Next.). }
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{c*{14}{c}}
% \toprule
% & \multicolumn{2}{c}{\circledc{6}} & \multicolumn{2}{c}{\circledc{7}} & \multicolumn{2}{c}{\circledc{8}} 
% & \multicolumn{2}{c}{\circledc{9}} & \multicolumn{2}{c}{\circledc{10}} & \multicolumn{2}{c}{\circledc{11}} & \multicolumn{2}{c}{\circledc{12}} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}
% % & Orig. & Next. & Orig. & Next. & Orig. & Next. & Orig. & Next. & Orig. & Next. & Orig. & Next. & Orig. & Next. \\
% & O. & N. & O. & N. & O. & N. & O. & N. & O. & N. & O. & N. & O. & N. \\
% \midrule
% \textbf{F1 (\%)}   & 99.5 & 99.5 & 99.6 & 99.3 & 99.3 & 98.0 & 99.4 & 97.8 & 99.0 & 98.4 & 97.6 & 96.3  & 93.1  & 66.3\\
% \textbf{MCR (\%)} & 97.9 & 98.1 & 95.7 & 83.4 & 99.3 & 99.1 & 99.5 & 94.7 & 94.6 & 91.7 & 99.9 & 98.6 & 97.7 & 96.6 \\
% \bottomrule
% \label{tab:wild}
% \end{tabular}
% }
% \end{table}




==> chapter/0-abstract.tex <==
\begin{abstract}
%-------------------------------------------------------------------------------


%The rapid development of blockchain gives rise to frequent financial security incidents. These incidents often involve laundering illicit funds through increasingly diverse strategies, posing severe threats to the blockchain financial ecosystem. However, existing cryptocurrency anti-money laundering (Crypto AML) methods have a limited ability to capture such diverse laundering strategies and generally fail to provide explainable detection results, restricting their applicability in real-world investigations.   

%We present \textsc{FlowShield}, a novel framework for detecting and explaining money laundering on blockchain. \textsc{FlowShield} integrates semantics awareness to capture transaction intents and fund flow awareness to model the origins and destinations of funds, and employs a semantics–structure fusion mechanism that combines Large Language Model (LLM)-based semantic embeddings with Graph Convolutional Network (GCN)-based structural embeddings. It further generates investigator-friendly suspicious activity reports (SARs) with fund flow visualizations, summaries, and red-flag indicators.

%\textsc{FlowShield} further generates investigator-oriented suspicious activity reports (SARs) with interpretable flow graphs, summaries, and red flags.


\textit{``At block $T$, an exchange hot wallet is drained. Within minutes, the stolen assets spread across new addresses, swap on decentralized exchanges, and move across chains through bridges, some hidden in internal contract calls.''}
This is not fiction but the daily reality of on-chain laundering: automated, transparent, yet discontinuous to investigators. Existing cryptocurrency anti money-laundering (Crypto~AML) methods lose the flow amid these fragmented trails as they fail to capture the semantic links between tokens, chains, and contracts.


We present \textsc{FlowShield}, a framework for detecting and explaining money laundering on blockchain. \textsc{FlowShield} integrates \textit{semantics awareness} to capture transaction intents and \textit{fund flow awareness} to model the origins and destinations of funds, and employs a \textit{semantics–structure fusion} mechanism that combines LLM-based semantic embeddings with Graph Convolutional Network (GCN)-based structural embeddings. \textsc{FlowShield} detects complex laundering strategies previously unattainable, covering heterogeneous combinations of chains (e.g., Ethereum to Bitcoin), token types (e.g., ERC-20 to ETH), and infrastructures (e.g., via cross-chain bridges).

We construct and release \textit{BybitML}, the first multi-chain laundering dataset derived from the Bybit Hack, and evaluate \textsc{FlowShield} on both Ethereum (\textit{BybitML-EC}) and Bitcoin (\textit{BybitML-BC}) subsets. \textsc{FlowShield} outperforms nine mainstream baselines, improving F1 by 6.2\% and 9.1\% with fund coverage of 88.0\% and 98.2\%. It detects four laundering strategies and two evasion behaviors, uncovers US\$930M of cross-chain laundering and 1,878 cross-chain addresses on Bitcoin, and reveals a strong preference for stablecoin-based swaps. Our method further produces accurate and explainable Suspicious Activity Reports (SARs) for forensic analysis.

%1. 基于 Bybit Hack 案件构建了首个多链洗钱数据集，并在其中验证了方法的有效性。
%2. 在整体性能上优于 9 个基线模型，F1 分数在以太坊和比特币子集上分别提升 6.2% 与 3.7%，资金覆盖率分别达 88% 与 99.8%。
%3. 该方法可识别 4 类洗钱策略 与 2 类规避行为，并保持稳定的cross-period generalization
%4. 揭示约 9.3 亿美元 的跨链桥洗钱流水及 1878 个 BTCs链上的跨链地址，并发现洗钱者倾向于利用稳定币进行换币洗钱
%5. The generated SARs are accurate and explainable for forensic analysis.

%后面还要加上检测时间的结论

%数据集起一个名字：BybitML 里面有以太坊数据集 (\textit{BybitML-EC})和比特币数据集(\textit{BybitML-BC})






% We evaluate \textsc{FlowShield} on real-world laundering transactions from the 14-day Bybit Hack dataset. The framework outperforms nine baselines, improving F1 score by 6.2\% (up to 90.7\%) and covering 88\% of the total laundered value. It further identifies four laundering strategies and two evasion behaviors, while maintaining stable cross-period generalization. The generated SARs are accurate, explainable, and actionable for forensic analysis. \qw{add more hilights}

%你看看第一段和不和你的taste 我感觉有点画面感那种切入比较有趣？lose flow可以call back下题目 然后discontinous可以呼应那个trace discontinuity的chanllegne 牛！

% To fill these gaps, we present \techName{}, a novel security system for detecting and explaining money laundering in blockchain networks. \techName{} introduces semantic awareness by parsing transactions into common intents, and fund flow awareness by constructing flow subgraphs that reveal the origins and destinations of funds. \techName{} further incorporates a semantics–structure fusion module that integrates large language model (LLM)-based semantic embeddings with graph convolutional network (GCN)-based structural embeddings via a cross-attention mechanism. Moreover, \techName{} generates investigator-friendly suspicious activity reports (SARs), including fund flow visualizations, summaries, and red-flag indicators. 


\end{abstract}

==> chapter/1-intro-qs-260202.tex <==
\section{Introduction} \label{sec:intro}

%P1：Background
Billions in stolen funds on the blockchain do not disappear — they flow.  Through decentralized exchanges, cross-chain bridges, and automated bots, illicit funds race across blockchains~\cite{chainalysis2025}. Each hop fragments the trail: a swap here, a bridge there, an internal contract call in between. Within minutes, stolen assets are scattered across hundreds of addresses and multiple chains, leaving only cryptic traces of what really happened~\cite{report}. 

This form of \textit{cryptocurrency money laundering}
(Crypto ML)~\cite{campbell2018bitcoin} has become a central threat to blockchain financial regulation and risk controls. Crypto ML often manifests as composable fund-flow paths~\cite{CASTILLOLEON2026102916}. 
To cover such combinations, monitoring systems broaden alert sets to improve recall, but alerts grow faster than investigative capacity, inducing alert fatigue and raising compliance costs~\cite{pwc2024_emea_aml_survey}. 
Meanwhile, DeFi~\cite{auer2024technology} enables swaps and cross-chain moves without a single centralized intermediary, weakening regulatory chokepoints such as consistent identity collection and reporting entry points, making early intervention and attribution harder~\cite{ustreasury2023_defi_risk}.


 % Following major thefts and protocol exploits, launderers routinely automate laundering pipelines that combine diverse on-chain operations to disperse and disguise stolen assets before regulators can freeze them. 

%P2：Case-->challenge
% In practice, modern laundering rarely relies on a single technique. Instead, launderers chain multiple routes to maximize obfuscation. Figure~\ref{fig:intro} illustrates a representative segment from the Bybit Hack, the largest crypto laundering incident to date~\cite{bybit25}.
% The stolen funds are first dispersed to accomplice addresses, then routed through smart contracts to perform indirect transfers into cross-chain bridges, where the assets are moved to another blockchain, while parallel flows undergo token swaps on a decentralized exchange. Such composed laundering behaviors give rise to two challenges for tracing laundering funds: (i)  \textbf{\emph{structure complexity}}: dispersal and automated execution multiply nodes and edges, creating highly entangled graphs that obscure causal links and strain scalability; and (ii)  \textbf{\emph{trace discontinuity}}: swaps, cross-chain hops, and internal contract calls break value continuity boundaries, so surface-level transaction graphs fail to reveal the true flow of funds. How, then, do we sniff out dirty money both smartly and swiftly?

% \begin{figure}[t]
% \centering
%   % \includegraphics[width=\linewidth]{Figs/example_ml_technique_2.png}
%     \includegraphics[width=0.75\linewidth]{Figs/bybit_case.pdf}
% \caption{A typical laundering segment of Bybit Hack.}
% \label{fig:intro}
% \end{figure}

%P3: Existing work
Crypto AML~\cite{sok25fu} is the technique for tracing and preventing illicit on-chain fund flows.  
Unlike traditional AML~\cite{calafos2022cyber}, it deals with pseudonymous, multi-layered blockchain transactions beyond regulated intermediaries. Table~\ref{tab:aml_comparison} summarizes representative Crypto AML methods. Existing Crypto AML techniques broadly fall into three categories: (i) 
\textbf{\textit{Rule-based heuristics}} rely on manually designed patterns~\cite{lv2023detection} and blacklists~\cite{wu2023towards}, which are effective for known laundering behaviors but fragile against evolving and composed strategies~\cite{sok25fu}; 
(ii) \textbf{\textit{Machine-learning approaches}} improve adaptability by learning statistical features from historical data~\cite{elmougy2023demystifying,wang2024graphalm,zhou2023visual}, yet typically treat transactions as independent samples and struggle to reason over multi-hop fund flows;
(iii) \textbf{\textit{Graph-based methods}} further model structural relations, but most remain address-centric and structure-driven~\cite{alarab2020competence,lin2024denseflow,nicholls2023fraudlens,weber2019anti,wu2023tracer}, where transaction semantics are simplified or ignored. 
%\textbf{As a result}, existing crypto AML methods struggle to handle both the structural complexity and trace discontinuity exhibited by modern laundering behaviors. These approaches share core limitations (\textbf{L}). We reinterpret technically as follows:
These approaches share core limitations (\textbf{L}). We interpret technically as follows:


\begin{packeditemize}

\item \textbf{L1: Limited understanding of advanced laundering techniques.} 
% 现有多数 AML 方法将链上行为简化为“直接转账”，难以刻画现代洗钱管线中多样且组合式的交易意图（如换币、跨链转移与间接转账等）。这会直接挑战 AI/ML 的有效性：在缺少显式语义证据的情况下，模型只能依赖局部图结构与统计特征，而链上意图并不天然可见，必须从日志中推断；同时，结构上相似甚至局部同构的交易可能对应完全不同的意图（例如同链 swap 与跨链 deposit），导致仅凭结构学习容易混淆与误判。因此，想让 AI 在该场景可靠工作，必须先把交易意图显式化。
Most AML methods~\cite{alarab2020competence,elmougy2023demystifying,lin2024denseflow,lv2023detection,nicholls2023fraudlens,wang2024graphalm,weber2019anti,wu2023towards,zhou2023visual} model blockchain transactions as direct transfers, failing to capture the diverse intents (e.g., swaps, cross-chain transfers, and indirect transfer) that compose modern laundering pipelines. This directly challenges the effectiveness of AI: without explicit semantic evidence, models must rely on local graph structure and statistical features, yet intent is not natively observable and has to be inferred from logs. Moreover, transactions that are structurally similar or even locally isomorphic can correspond to fundamentally different intents, making structure-only learning prone to confusion and misclassification.

\item \textbf{L2: Limited capabilities in tracking fund flow.} 
% 许多 AML 方法构建地址级交易图，用边表示“发生过转账”。但这种图刻画的是交互关系，不等价于资金如何在多笔下游交易中分配与传播：当地址在入金后产生多笔出金时，仅凭结构与特征无法判断上游资金是否被拆分、集中转移，或根本未被使用。由于账户模型链上缺少“入金—出金”的显式链接，金额级归因本质上欠定，纯粹依赖AI只能学习交易相关性，影响多跳追踪与检测的可靠性。因此，需要引入资金传播。
Most AML approaches~\cite{lin2024denseflow, lv2023detection, wu2023towards,wu2023tracer} model address-level transaction graphs, where an edge indicates that a transfer occurred. However, such graphs capture interactions rather than how value is allocated and propagated across multiple downstream spends: when an address fans out to multiple downstream transactions, it is ambiguous whether (and how much of) the upstream funds are split, concentrated in one, or not used. Because raw transactions in account-based blockchains do not explicitly link a specific inflow to a specific outflow, relying on AI alone tends to learn address correlations, undermining the reliability of multi-hop tracing and detection.


\item \textbf{L3 (AI can tackle): Limited multi-view representation.} 
% 现代洗钱行为往往同时涉及多维信号，但现有方法多视角证据通常被割裂建模，或以浅层方式拼接，缺少统一、对齐的联合表征。AI在此可以发挥关键作用：通过分别学习不同视角的表征,再用融合机制对齐并整合互补，获得更稳健的联合表示，从而更好地区分洗钱和正常交易。
Crypto ML transactions often involve multi-dimensional signals, yet prior approaches~\cite{alarab2020competence,elmougy2023demystifying,lin2024denseflow,lv2023detection,nicholls2023fraudlens,wang2024graphalm,weber2019anti,wu2023towards,wu2023tracer} often treat different views as separate features or rely on shallow aggregation, without learning an aligned multi-view representation. AI-based representation learning can help unify these heterogeneous cues into a coherent view, enabling more reliable separation of laundering and benign transactions.

\item \textbf{L4 (AI can tackle): Lack of user-friendly explainable results.} 
% 尽管近年的方法提升了检测准确率，但输出往往停留在“洗钱/非洗钱”的二分类，难以为调查提供可用证据与可读结论（如可疑资金路径、关键换币/跨链操作及异常模式），限制了其在取证与合规流程中的实用性。AI/ML 可用于把“检测”转化为“可交付解释”
Despite improved detection accuracy, most AML systems still output only binary labels~\cite{alarab2020competence,elmougy2023demystifying,lin2024denseflow,lv2023detection,nicholls2023fraudlens,wang2024graphalm,weber2019anti,wu2023tracer,wu2023towards,zhou2023visual}, without translating predictions into case-ready evidence such as suspicious flow summaries, key operations (e.g., swaps/cross-chain moves), and actionable red flags. 
AI-based generation offers a practical path to produce concise, evidence-grounded reports for investigators and auditors.


% ：在多视角融合表征上先用轻量分类器（如 MLP）完成可疑交易识别，再将检测到的洗钱资金流及其证据化描述输入 LLM，生成包含过程摘要与 red flags 的 SAR，使输出具备可读性与可复核性，从而支持调查与审计。


\end{packeditemize}




% \begin{packeditemize}
% %L1： Limited Understanding of Diverse Laundering Intents.
% %现有加密货币反洗钱研究普遍将区块链交易视作同质化的资金转移，忽视了交易背后的洗钱意图。在现实场景中，洗钱者会通过多种交易行为来隐藏资金来源、切断追踪路径。这些洗钱交易行为反映了不同的意图，referred to as transaction semantics, 是刻画复杂洗钱行为的重要依据。然而，现有研究仅对少部分语义进行建模，仍存在显著的语义空缺，导致模型难以识别多样化的洗钱交易。

% % \smallskip
% \item \textbf{L1 : Limited understanding of advanced laundering techniques.}  
% Most AML methods~\cite{alarab2020competence,elmougy2023demystifying,lin2024denseflow,lv2023detection,nicholls2023fraudlens,wang2024graphalm,weber2019anti,wu2023towards,zhou2023visual} model blockchain transactions as direct transfers, failing to capture the diverse intents (e.g., swaps, cross-chain transfers, and indirect transfer) that compose modern laundering pipelines. Although Tracer~\cite{wu2023tracer} distinguishes basic transfer and swap operations, other critical semantics remain unmodeled.
% \end{packeditemize}

% \noindent\textit{Why is this hard?} Transaction semantics are not explicitly encoded on-chain and must be inferred from transaction logs. From a graph perspective, transactions that are structurally similar or even locally isomorphic can correspond to fundamentally different intents (e.g., a same-chain swap versus a cross-chain deposit), making it difficult to disambiguate laundering behaviors using structure alone.

%\footnote{Event logs are structured records emitted by smart contracts that describe on-chain actions such as transfers or calls.}

% \begin{packeditemize}
% \item \textbf{L2: Limited capabilities in tracking fund flow.}  
% %在账户模型区块链（如 Ethereum）中，现有 AML 方法通常构建地址级交易图，仅刻画地址之间是否发生过交易。这种抽象使得边级别的资金流向信息丢失，难以判断某一笔资金的具体来源与去向。洗钱检测关注的并非地址关系，而是资金如何沿交易路径传播并完成转移。相比之下，UTXO 模型能够通过显式输入与输出刻画资金流向，但其方法高度依赖比特币式账本结构，难以推广至账户模型区块链。
% Most AML approaches~\cite{lin2024denseflow, lv2023detection, wu2023towards,wu2023tracer} in account-based blockchains (e.g., Ethereum) construct address-level graphs but ignore how funds propagate across transactions. As a result, fund sources and destinations cannot be precisely attributed. While UTXO-based methods~\cite{elmougy2023demystifying,nicholls2023fraudlens,weber2019anti} explicitly model inputs and outputs, they are confined to the Bitcoin-style ledger design and cannot extend to account-based systems.
% \end{packeditemize}

% \noindent\textit{Why is this hard?} 
% %账户模型区块链的原始交易数据仅提供账户之间的交易信息，并未提供可直接用于资金传播建模的数据，使得现有方法难以在交易图上刻画资金如何从上游传播至下游。现有交易图通常以地址为节点、以交易为边，这种表示天然适合刻画交互关系，却难以表达资金在交易序列中的流动过程。因此，需要在现有交易图之上引入新的建模方法，使资金传播成为可显式分析的对象。
% In account-based blockchains, the raw transaction data does not explicitly model fund-flow structures across transactions. Existing transaction graphs typically model addresses as nodes and transactions as edges, which are insufficient for representing how value propagates through transactions. As a result, additional modeling is required to make fund-flow propagation an explicit and analyzable object.

% \begin{packeditemize}
% \item \textbf{L2: Limited capabilities in tracking fund flow.}  
% % 现有许多 AML 方法在账户模型链（如 Ethereum）上构建地址级交易图，把“地址之间发生过交易”作为边来刻画结构关系。但交易边只说明发生了转账交互，并不等价于“资金如何沿下游边传播”：当一个地址在某笔入金之后产生多笔出金时，单靠交易图无法判断该入金在这些下游交易中的分配关系——它可能被分散到多条边、可能几乎全部沿某一条边转移，也可能根本未在这些交易中被使用（例如使用的是该地址已有余额）。换言之，图结构提供的是“可达路径”，但洗钱追踪需要的是“价值守恒下的资金归因”：每条下游边到底承接了多少来自上游的资金、哪些下游交易真正继承了可疑资金。由于缺少对这种资金分配/归因的显式建模，现有方法往往只能做结构相关性分析，而难以重建资金流向与金额级传播。
% Most AML approaches~\cite{lin2024denseflow, lv2023detection, wu2023towards,wu2023tracer} model address-level transaction graphs, where an edge indicates that a transfer occurred. 
% However, such graphs capture interactions but not how value is propagated: when an address fans out to multiple downstream transactions, it is ambiguous whether (and how much of) the upstream funds are split, concentrated in one, or not used. 
% Without explicit allocation modeling, existing methods cannot reliably reconstruct amount-level fund-flow propagation.
% \end{packeditemize}

% \noindent\textit{Why is this hard?} 
% %在账户模型中，原始交易数据不提供“某笔入金对应哪笔出金”的显式链接；当下游存在多笔出金时，资金传播必须结合语义以及相关信息才能推断“钱到底怎么流”。
% Raw transactions in account-based blockchains do not explicitly link a specific inflow to a specific outflow. When an address has multiple downstream spends, inferring how the money actually moved requires additional context (e.g., semantics and related evidence) beyond the graph itself.

% \begin{packeditemize}
% \item \textbf{L3: Lack of user-friendly explainable results.}  
% %现有多数 AML 方法虽提升了检测准确率，但其输出通常仅为洗钱与否的二分类结果，缺乏对判断结果的解释。模型难以揭示可疑资金的传播路径、关键的换币或跨链行为，以及相关的异常模式，因而难以支撑调查取证流程。
% Although recent solutions improved detection accuracy, their outputs are typically limited to binary classifications~\cite{alarab2020competence,elmougy2023demystifying,lin2024denseflow,lv2023detection,nicholls2023fraudlens,wang2024graphalm,weber2019anti,wu2023tracer,wu2023towards,zhou2023visual}  (laundering or not).  
% They rarely provide interpretable evidence of fund-flow propagation, key swap or cross-chain operations, or abnormal behavioral patterns, limiting their usefulness for investigative and forensic purposes. 
% \end{packeditemize}

% \noindent\textit{Why this is hard?}  
% %现有图模型和深度学习方法通常将多跳交易关系压缩为高维表示，从而掩盖了交易之间的因果路径。例如，图神经网络 (GNN) 可能基于聚合的邻域特征将某个地址或交易标记为洗钱，但它无法揭示导致这一结论的具体转账行为。 类似地，统计分类器可以检测特征空间中的异常值，但却忽略了潜在的交易结构。
% Graph-based and deep learning models compress multi-hop transaction dependencies into high-dimensional embeddings, obscuring causal transaction paths. For example, a GNN may flag an address or transaction as laundering based on aggregated neighborhood features, yet cannot identify the specific transfers responsible. Similarly, statistical classifiers detect outliers in feature space while discarding the underlying transactional structure.


%P4: Ours
% We present \textsc{FlowShield}, a new framework for detecting and explaining Crypto ML transactions. 
% % \textsc{FlowShield} closes the three gaps through an integrated pipeline that (i) parses transaction \emph{semantics}, (ii) reconstructs fine-grained \emph{fund-flow} subgraphs, and (iii) fuses semantics and structure for accurate and explainable detection. 
% Specifically, \textbf{to address L1}, \textsc{FlowShield} introduces a \emph{semantics-aware module} that parses high-level transaction intents from raw on-chain transaction records, enabling the model to distinguish heterogeneous transaction intents such as token swaps, cross-chain transfers, and indirect transfers beyond simple direct transfers. 
% These semantics are inferred by jointly analyzing event logs, token transitions, and address linkages within transaction groups.
% \textbf{To address L2}, \textsc{FlowShield} employs a \emph{fund-flow aware module} that explicitly models fund-flow propagation by reconstructing transaction-level fund-flow subgraphs from three complementary perspectives, tracing where transaction value originates, how it is redistributed downstream, and whether parallel flows occur.
% Finally, \textbf{to address L3}, \textsc{FlowShield} integrates a \emph{semantics–structure fusion module} that learns structural representations using GCNs, and semantic representations by encoding textual descriptions of transaction semantics and fund flows with an LLM, and fuses them via a cross-attention mechanism for laundering detection. \emph{SAR generation module} in \textsc{FlowShield} subsequently generates reports by prompting the LLM with detected laundering fund flows. 

%P4: Ours
We present \textsc{FlowShield}, a new framework for detecting and explaining Crypto ML transactions.
Specifically, 
\textbf{to address L1}, \textsc{FlowShield} introduces a \emph{semantic-awareness module} that makes transaction intent explicit by mapping raw on-chain transfers to a set of \emph{semantic types} via \emph{pre-defined parsing rules}. It further generates a textualized semantics description using templates.
\textbf{To address L2}, \textsc{FlowShield} employs a \emph{fund-flow awareness module} that explicitly models fund-flow propagation by reconstructing transaction-level fund-flow subgraphs from three complementary perspectives, tracing where transaction value originates, how it is redistributed downstream, and whether parallel flows occur.
\textbf{To address L3}, \textsc{FlowShield} adopts a \emph{semantics-structure fusion module} that learns \emph{multi-view representations} by encoding semantics and flow texts with an LLM and atructure with GCNs, and fuses the two views via cross-attention for detection.
Finally, \textbf{to address L4}, \textsc{FlowShield} uses a lightweight classifier over fused multi-view representations to flag suspicious transactions, then prompts an LLM with the detected laundering flows to generate SARs with concise summaries and key red flags for investigation and audit.


We benchmark \textsc{FlowShield} against representative Crypto AML methods on our multi-chain dataset \textit{BybitML}. Experimental results show that \textsc{FlowShield} consistently outperforms all baselines, achieving F1 improvements of 6.2\% on Ethereum and 9.1\% on Bitcoin, with fund coverage reaching 88\% and 98.2\%, respectively. Beyond detection accuracy, \textsc{FlowShield} enables fine-grained analysis of laundering strategies, uncovers large-scale cross-chain laundering activities, and generates high-quality, interpretable SAR-style reports, demonstrating both effectiveness and practical utility.

% P5: Contribution
In summary, this paper makes the following key contributions:
\begin{packeditemize}
%C1: 新的洗钱行为建模方式。据我们所知，本文首次在加密货币反洗钱场景中同时考虑交易行为语义与资金传播过程进行建模，将洗钱检测从基于地址或交易的判别，扩展为对资金如何通过多种交易行为在交易网络中传播的刻画，从而更好地描述复杂洗钱过程。
    \item \textbf{A new modeling perspective.} To the best of our knowledge, this work is the first to jointly model \emph{transaction semantics} and \emph{fund-flow propagation} for Crypto AML. 
    We move beyond address- or transaction-level classification and instead model how funds propagate through diverse transaction behaviors, enabling more faithful characterization of complex laundering processes.

    
%C2: 创新的反洗钱检测框架。我们提出了一种新的反洗钱检测框架 \textsc{FlowShield}，由语义感知、资金流建模、语义–结构融合以及 SAR 生成四个模块组成，能够联合分析交易意图与资金流结构，实现对复杂洗钱行为的准确检测与可解释分析。
% qs:这里直接写via GCNs and LLM有点怪，不知道要怎么写合适
    \item \textbf{A unified detection framework.} We propose \textsc{FlowShield}, a novel Crypto AML framework consisting of four modules. 
    The framework jointly captures transaction intent and fund-flow structure, enabling accurate and explainable detection of complex laundering behaviors via GCNs and LLM.

    
%C3: 首个公开的多链洗钱数据集。我们构建并公开了首个基于真实重大安全事件的多链洗钱数据集 \textit{BybitML}，覆盖 Ethereum 与 Bitcoin 两条主流区块链，并提供交易语义标注与洗钱交易标注，为相关研究提供可复现的实验基准。
    \item \textbf{The first multi-chain AML dataset.}  We construct and release BybitML\footnote{\textit{BybitML} is publicly available at \url{https://osf.io/nx7aj/overview?view_only=663038fbea43491bb4010011c7f28b23}.}, the first public multi-chain Crypto AML dataset derived from a real-world major security incident. 
    The dataset covers two major blockchains and provides transaction-level semantic annotations and laundering labels.
    
%C4：全面的实验验证。我们在 \textit{BybitML} 数据集上对 \textsc{FlowShield} 进行了系统评估，并与九种代表性基线方法进行了对比。实验结果表明，该方法在整体检测性能上显著优于现有方法。我们开源了数据集与代码。
    \item \textbf{Extensive experimental validation.} We conduct comprehensive evaluations of \textsc{FlowShield}\footnote{The implementation of \textsc{FlowShield} is available at \url{https://osf.io/9s3j2/overview?view_only=9b15fcf6978b47ddbdcc8a850d1666c9}.} on \textit{BybitML} and compare it against nine representative baseline methods. 
    Experimental results demonstrate that \textsc{FlowShield} consistently outperforms existing approaches in detection performance. 

% \item \textbf{Insights:} We perform an in-depth analysis of laundering transactions detected by \textsc{FlowShield}, summarizing diverse laundering strategies and evasion behaviors, which provides insights for regulatory and investigative practice.
    
\end{packeditemize}

%

\begin{table*}[h]
\centering
\scriptsize
% \qw{maybe more metrics?}
\caption{Comparison of typical Crypto AML methods.}\label{tab:aml_comparison}

\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c|c|c|c@{\hspace{1.6pt}}c|c@{\hspace{1.6pt}}c@{\hspace{1.6pt}}c@{\hspace{1.6pt}}c|c@{\hspace{1.6pt}}c}
\toprule
\multirow{2}{*}{\textbf{Crypto AML}} 
&  \multirow{2}{*}{\textbf{Method}} 
& \multirow{2}{*}{\textbf{Dataset (Year)}} 
& \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Blockchain}}} 
& \multicolumn{4}{c}{\textbf{Semantics}} 
& \multirow{2}{*}{\makecell[c]{\textbf{Laundering}\\\textbf{flow}}}  
& \multirow{2}{*}{\makecell[c]{\textbf{Explainable}\\\textbf{result}}} \\
 \cmidrule(lr){6-9}
 % \textcolor{red!80}{P2}
 &  & & UTXO & Account & $\text{S}_{dir}$ & $\text{S}_{ind}$ & $\text{S}_{swp}$  & $\text{S}_{crs}$  &   \\
\midrule
Youssef\cite{elmougy2023demystifying} & Machine learning & \textit{Elliptic}~(2019) &\greencheck & \redx & \greencheck &  \redx & \redx &   \redx & \greencheck &  \redx \\
FraudLens\cite{nicholls2023fraudlens} & Graph-based       & \textit{Elliptic}~(2019)  & \greencheck & \redx & \greencheck &  \redx & \redx & \redx & \greencheck  & \redx \\
Weber\cite{weber2019anti} & Graph-based     & \textit{Elliptic}~(2019) & \greencheck & \redx & \greencheck &  \redx & \redx & \redx & \greencheck  & \redx \\
Cyclic\cite{lv2023detection}    & Heuristic & \textit{Not available} & \redx & \greencheck &  \greencheck & \redx & \redx & \redx & \redx & \redx \\
XBlock\cite{wu2023towards}   & Heuristic & \textit{EthereumHeist}~(2022) &\redx & \greencheck &  \greencheck& \redx & \redx & \redx & \redx & \redx \\
DenseFlow\cite{lin2024denseflow} & Graph-based & \textit{EthereumHeist}~(2022) &\redx & \greencheck &  \greencheck& \redx & \redx & \redx & \redx & \redx \\
Tracer\cite{wu2023tracer}    & Graph-based & \textit{Not available} & \redx & \greencheck &  \greencheck&  \greencheck& \redx & \redx &  \redx  & \redx \\
\midrule
\rowcolor{gray!10}
 \techName{}  & Graph + LLM    & \textit{BybitML}~(2025) &\greencheck & \greencheck &  \greencheck&  \greencheck&  \greencheck&  \greencheck&  \greencheck&  \greencheck\\
\bottomrule
\end{tabular}
}
\end{table*}


% \begin{table}[h]
% \centering
% \scriptsize
% % \qw{maybe more metrics?}
% % \caption{Comparison of typical Crypto AML methods}\label{tab:aml_comparison}
% \caption{Comparison of typical Crypto AML methods. U/A denote UTXO- and account-based blockchains; D/I/S/C denote direct transfer, indirect transfer, token swap, and cross-chain transfer semantics; Expl. denotes explainable results.}\label{tab:aml_comparison}

% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|cc|cccc|c@{\hspace{1.3pt}}c}
% \toprule
% \multirow{2}{*}{\textbf{Crypto AML}} 
% &  \multirow{2}{*}{\textbf{Method}} 
% & \multirow{2}{*}{\textbf{Dataset (Year)}} 
% & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Chain}}} 
% & \multicolumn{4}{c}{\textbf{Semantics}} 
% & \multirow{2}{*}{\textbf{Flow}}
% & \multirow{2}{*}{\textbf{Expl.}} \\
%  \cmidrule(lr){6-9}
%  % \textcolor{red!80}{P2}
%  &  & & U & A & D & I & S  & C  &   \\
% \midrule
% Youssef\cite{elmougy2023demystifying} & Machine learning & \textit{Elliptic}~(19) &\greencheck & \redx & \greencheck &  \redx & \redx &   \redx & \greencheck &  \redx \\
% FraudLens\cite{nicholls2023fraudlens} & Graph-based       & \textit{Elliptic}~(19)  & \greencheck & \redx & \greencheck &  \redx & \redx & \redx & \greencheck  & \redx \\
% Weber\cite{weber2019anti} & Graph-based     & \textit{Elliptic}~(19) & \greencheck & \redx & \greencheck &  \redx & \redx & \redx & \greencheck  & \redx \\
% Cyclic\cite{lv2023detection}    & Heuristic & \textit{Not available} & \redx & \greencheck &  \greencheck & \redx & \redx & \redx & \redx & \redx \\
% XBlock\cite{wu2023towards}   & Heuristic & \textit{EthereumHeist}~(22) &\redx & \greencheck &  \greencheck& \redx & \redx & \redx & \redx & \redx \\
% DenseFlow\cite{lin2024denseflow} & Graph-based & \textit{EthereumHeist}~(22) &\redx & \greencheck &  \greencheck& \redx & \redx & \redx & \redx & \redx \\
% Tracer\cite{wu2023tracer}    & Graph-based & \textit{Not available} & \redx & \greencheck &  \greencheck&  \greencheck& \redx & \redx &  \redx  & \redx \\
% \midrule
% \rowcolor{gray!10}
%  \techName{}  & Graph + LLM    & \textit{BybitML}~(25) &\greencheck & \greencheck &  \greencheck&  \greencheck&  \greencheck&  \greencheck&  \greencheck&  \greencheck\\
% \bottomrule
% \end{tabular}
% }
% \end{table}



% \input{chapter/2-backgraound}

% \section{PRELIMINARY}
% \subsection{Problem definition}

%qs: 如果后面还有空间，可以加上洗钱和交易数据的简单介绍？








==> chapter/1-intro-yixin.tex <==
\textit{Cryptocurrency money laundering}
(Crypto ML)~\cite{campbell2018bitcoin} has become a central threat to blockchain financial regulation and risk controls. Through the combinations of fund-flow paths with different intent, such as fund dispersal, token swap, indirect transfer, and cross-chain transfer (their definitions are described in Appendix~\ref{app:paths}), stolen assets are scattered across hundreds of addresses and multiple chains, leaving only cryptic traces of what really happened within minutes~\cite{report}. The Decentralized Finance (DeFi) ecosystem~\cite{CASTILLOLEON2026102916} in blockchain further enables swaps and cross-chain moves without a single centralized intermediary, weakening regulatory chokepoints such as consistent identity collection and reporting entry points, making early intervention and attribution harder~\cite{ustreasury2023_defi_risk}.
 
The key to identifying Crypto ML activities lies in \ding{182}~\textit{\textbf{semantic-level understanding of laundering fund-flow paths}} and \ding{183}~\textit{\textbf{end-to-end tracking of fund flows}}. Taking a representative segment from the Bybit Hack (the largest crypto laundering incident to date~\cite{bybit25}) as an example, as shown in Figure~\ref{fig:intro}, the stolen funds are routed through combinations of laundering paths with different semantic intents (e.g., token swaps and cross-chain transfers), resulting in multiple parallel fund flows that rapidly fragment the transaction trail. In order to detect such complex and multi-stage laundering behaviors, an effective approach must understand the semantic intent behind diverse transactions to distinguish heterogeneous laundering operations; at the same time, the entire chain of fund flows should be modeled holistically to capture how illicit value propagates across paths.

While the existing cryptocurrency anti-money laundering (Crypto AML)~\cite{sok25fu} approaches employ various techniques to trace and prevent illicit on-chain fund flows, they struggle to address the above requirements jointly. Specifically, {\textit{Rule-based heuristics} rely on manually designed patterns~\cite{lv2023detection} and blacklists~\cite{wu2023towards}, which are effective for known laundering behaviors but fragile against evolving and composed strategies~\cite{sok25fu}. \textit{Machine learning-based approaches}, in contrast, improve adaptability by learning statistical features from historical data~\cite{elmougy2023demystifying,wang2024graphalm,zhou2023visual}, yet typically treat transactions as independent samples and struggle to reason over multi-hop fund flows. \textit{Graph-based methods} further model structural relations, but most remain address-centric and structure-driven~\cite{alarab2020competence,lin2024denseflow,nicholls2023fraudlens,weber2019anti,wu2023tracer}, where transaction semantics are simplified or ignored.  

To overcome the limitations of existing approaches and develop next-generation reliable Crypto AML solutions, we identify three core challenges, which are summarized as follows. 

\textit{\textbf{Challenge 1: Transaction semantics understanding.}} Understanding transaction semantics is fundamental to accurately interpreting on-chain behaviors, as identical transaction structures may serve vastly different purposes in laundering pipelines. However, transaction semantics are not explicitly encoded on-chain and must be inferred from transaction logs. From a graph perspective, transactions that are structurally similar or even locally isomorphic can correspond to fundamentally different intents (e.g., a same-chain swap versus a cross-chain deposit), making it difficult to disambiguate laundering behaviors using structure alone. \textcolor{blue}{more details about "difficulty" can be given here} % 比如：他们都是转账的形式，光从表面难以分辨之类的。

\textit{\textbf{Challenge 2: Fund flow tracking.}} Tracking fund flows is essential for understanding how illicit value propagates through laundering pipelines, particularly when funds are split, merged, and relayed across multiple transactions. Nevertheless, in account-based blockchains, raw transaction data does not provide explicit links between incoming and outgoing transfers, i.e., which specific inflow gives rise to which downstream outflow. Existing transaction graphs typically model addresses as nodes and transactions as edges, which are insufficient for representing how value propagates across transactions.
When multiple downstream transfers exist, fund-flow propagation cannot be determined from structure alone and must instead be inferred by jointly considering transaction semantics and contextual information, making accurate flow tracking fundamentally challenging.

\textit{\textbf{Challenge 3: Bridging detection and interpretability.}} 
Explainability is critical for reliable Crypto AML, enabling investigators to understand how illicit funds propagate, where key laundering operations occur, and why specific behaviors are deemed suspicious. Although recent solutions improved detection accuracy, their outputs are typically limited to binary classifications~\cite{alarab2020competence,elmougy2023demystifying,lin2024denseflow,lv2023detection,nicholls2023fraudlens,wang2024graphalm,weber2019anti,wu2023tracer,wu2023towards,zhou2023visual}  (laundering or not).  
They rarely provide interpretable evidence of fund-flow propagation, key swap or cross-chain operations, or abnormal behavioral patterns, limiting their usefulness for investigative and forensic purposes. However, generating such interpretable evidence is challenging, as modern detection models often compress multi-hop fund-flow dependencies into high-dimensional representations, obscuring the causal paths and decision rationales required for audit-ready analysis.


To address the above challenges, we present \textsc{FlowShield}, a new framework for detecting and explaining Crypto ML transactions. 
% \textsc{FlowShield} closes the three gaps through an integrated pipeline that (i) parses transaction \emph{semantics}, (ii) reconstructs fine-grained \emph{fund-flow} subgraphs, and (iii) fuses semantics and structure for accurate and explainable detection. 
Specifically, to address \textit{\textbf{Challenge 1}}, \textsc{FlowShield} introduces a \emph{transaction semantics parsing module} that parses high-level transaction intents from raw on-chain transaction records, enabling the model to distinguish heterogeneous transaction intents such as token swaps, cross-chain transfers, and indirect transfers beyond simple direct transfers. 
These semantics are inferred by jointly analyzing event logs, token transitions, and address linkages within transaction groups.
To address \textit{\textbf{Challenge 2}}, \textsc{FlowShield} employs a \emph{fund-flow construction module} that explicitly models fund-flow propagation by reconstructing transaction-level fund-flow subgraphs from three complementary perspectives, tracing where transaction value originates, how it is redistributed downstream, and whether parallel flows occur.
Finally, to address \textit{\textbf{Challenge 3}}, \textsc{FlowShield} integrates a \emph{semantics–structure fusion module} that learns structural representations using GCNs, and semantic representations by encoding textual descriptions of transaction semantics and fund flows with an LLM, and fuses them via a cross-attention mechanism for laundering detection. \emph{SAR generation module} in \textsc{FlowShield} subsequently generates reports by prompting the LLM with detected laundering fund flows. 
We benchmark \textsc{FlowShield} against representative Crypto AML methods on our multi-chain dataset \textit{BybitML}. Experimental results show that \textsc{FlowShield} consistently outperforms all baselines, achieving F1 improvements of 6.2\% on Ethereum and 9.1\% on Bitcoin, with fund coverage reaching 88\% and 98.2\%, respectively. %Beyond detection accuracy, \textsc{FlowShield} enables fine-grained analysis of laundering strategies, uncovers large-scale cross-chain laundering activities, and generates high-quality, interpretable SAR-style reports, demonstrating both effectiveness and practical utility.
% P5: Contribution
In summary, this paper makes the following key contributions:
\begin{packeditemize}
%C1: 新的洗钱行为建模方式。据我们所知，本文首次在加密货币反洗钱场景中同时考虑交易行为语义与资金传播过程进行建模，将洗钱检测从基于地址或交易的判别，扩展为对资金如何通过多种交易行为在交易网络中传播的刻画，从而更好地描述复杂洗钱过程。
    \item \textbf{A new modeling perspective.} To the best of our knowledge, this work is the first to jointly model \emph{transaction semantics} and \emph{fund-flow propagation} for Crypto AML. 
    We move beyond address- or transaction-level classification and instead model how funds propagate through diverse transaction behaviors, enabling more faithful characterization of complex laundering processes.
    
%C2: 创新的反洗钱检测框架。我们提出了一种新的反洗钱检测框架 \textsc{FlowShield}，由语义感知、资金流建模、语义–结构融合以及 SAR 生成四个模块组成，能够联合分析交易意图与资金流结构，实现对复杂洗钱行为的准确检测与可解释分析。
% qs:这里直接写via GCNs and LLM有点怪，不知道要怎么写合适
    \item \textbf{A unified detection framework.} We propose \textsc{FlowShield}, a novel Crypto AML framework consisting of four modules. 
    The framework jointly captures transaction intent and fund-flow structure, enabling accurate and explainable detection of complex laundering behaviors via GCNs and LLM.

    
%C3: 首个公开的多链洗钱数据集。我们构建并公开了首个基于真实重大安全事件的多链洗钱数据集 \textit{BybitML}，覆盖 Ethereum 与 Bitcoin 两条主流区块链，并提供交易语义标注与洗钱交易标注，为相关研究提供可复现的实验基准。
    \item \textbf{The first multi-chain AML dataset.}  We construct and release BybitML\footnote{\textit{BybitML} is publicly available at \url{https://osf.io/nx7aj/overview?view_only=663038fbea43491bb4010011c7f28b23}.}, the first public multi-chain Crypto AML dataset derived from a real-world major security incident. 
    The dataset covers two major blockchains and provides transaction-level semantic annotations and laundering labels.
    
%C4：全面的实验验证。我们在 \textit{BybitML} 数据集上对 \textsc{FlowShield} 进行了系统评估，并与九种代表性基线方法进行了对比。实验结果表明，该方法在整体检测性能上显著优于现有方法。我们开源了数据集与代码。
    \item \textbf{Extensive experimental validation.} We conduct comprehensive evaluations of \textsc{FlowShield}\footnote{The implementation of \textsc{FlowShield} is available at \url{https://osf.io/9s3j2/overview?view_only=9b15fcf6978b47ddbdcc8a850d1666c9}.} on \textit{BybitML} and compare it against nine representative baseline methods. 
    Experimental results demonstrate that \textsc{FlowShield} consistently outperforms existing approaches in detection performance. 

% \item \textbf{Insights:} We perform an in-depth analysis of laundering transactions detected by \textsc{FlowShield}, summarizing diverse laundering strategies and evasion behaviors, which provides insights for regulatory and investigative practice.
    
\end{packeditemize}

==> chapter/1-introduction-old.tex <==
\section{Introduction} \label{sec:intro}
With the rapid development of the cryptocurrency (Crypto) ecosystem, blockchain has not only fueled the prosperity of decentralized finance (DeFi) but has also become the foundation of various emerging financial applications~\cite{werner2022sok,jiang2023decentralized}. However, the pseudonymous nature~\cite{lubbertsenghost} of blockchain poses significant threats to financial security~\cite{LI2020841}, because it facilitates illicit activities such as scams, stolen funds, and ransomware attacks~\cite{291271}. 
%According to the Blockchain Security and AML Annual Report 2024 released by the security firm SlowMist, 
Blockchain security incidents in 2024 resulted in economic losses of up to \$2 billion in crypto, while less than 10\% of the illicit funds were eventually recovered, with the vast majority rapidly transferred and laundered \cite{report}. Following such incidents, illicit funds are often moved immediately through complex transaction paths and diverse obfuscation tools for laundering, known as cryptocurrency money laundering (Crypto ML), which has become a critical threat to the security of the blockchain financial system.

%https://www.csis.org/analysis/bybit-heist-and-future-us-crypto-regulation

Take the largest blockchain financial security incident to date, the Bybit hack~\cite{bybit25}, as an example.
After stealing approximately USD\$1.46 billion in crypto from the Bybit exchange, the attackers employed a combination of strategies to conceal the funds. They first converted the stolen tokens (stETH, cmETH, and mETH) into Ether (ETH) via decentralized exchanges (DEXs). The funds were then fragmented and distributed across numerous addresses to complicate forensic tracing. Next, the attackers leveraged cross-chain services to move the funds across different blockchains, creating highly complex transaction paths. These complex laundering techniques pose significant challenges to current Crypto AML systems.


%add Layered Laundering definition
% add citation
\heading{Layered laudering.}
In the observable cryptocurrency ecosystem\footnote{Referring to public blockchains where transactions 
are transparent and traceable}, Launderers strategically execute transactions with multiple intents~\cite{sok25fu} such as direct transfers, token swaps, cross-chain transfers, and indirect transfers to enable funds to circulate through multi-hop transfers, asset conversions, and cross-chain operations. The resulting multi-layered fund flow structure is known as Layered Laundering~\cite{wu2023towards}. In essence, launderers repeatedly split, reorganize, and relocate funds to weaken the logical linkage between their sources and destinations, making the flow of assets visible on the ledger yet difficult to interpret in terms of intent. Unlike privacy-preserving laundering through mixers or privacy coins~\cite{chanalysis24}, layered laundering does not conceal transaction data but rather achieves obfuscation through structural complexity, rendering the funds observable but unintelligible. With the rapid expansion of DeFi, layered laundering has become the dominant form of on-chain money laundering~\cite{report}, and its detection and interpretation have emerged as a core challenge in cryptocurrency security and regulation.


\heading{Crypto AML.}
Crypto AML~\cite{campbell2018bitcoin} refers to the set of techniques and systems designed to detect, analyze, and prevent illicit fund flows within blockchain ecosystems. Unlike traditional AML~\cite{calafos2022cyber}, which relies on regulated intermediaries and fiat transaction monitoring, Crypto AML operates directly on blockchain data, where transactions are pseudonymous, often involve complex layering processes, and exhibit diverse types. 

Prior research on Crypto AML can be broadly categorized into three types: heuristic rule-based methods~\cite{wu2023towards,lv2023detection,kuccuk2023investigation}, which rely on predefined suspicious behavior patterns; traditional machine learning-based methods~\cite{elmougy2023demystifying,wang2024graphalm,zhou2023visual}, which extract features from transaction data and train classifiers; graph-based methods~\cite{wu2023tracer,lin2024denseflow,wu2023tracer}, which exploit structural relationships among accounts or transactions. These methods are effective in detecting certain money laundering activities. However, they remain inadequate when confronted with the growing sophistication of laundering strategies. As summarized in Table~\ref{tab:aml_comparison}, their major limitations are as following:


\begin{packeditemize}
\item \textbf{L1: lack of transaction semantic awareness.} Most AML methods \cite{lv2023detection,wu2023towards,kuccuk2023investigation,elmougy2023demystifying,nicholls2023fraudlens,lin2024denseflow} treat blockchain transactions as simple transfers, ignoring the rich transaction intents. In reality, blockchain transactions encompass not only direct transfers but also token swaps, cross-chain transfers, and indirect transfers. These high-level behavioral intents, referred to as transaction semantics, are crucial for characterizing and detecting complex and diverse money laundering patterns. Although Tracer~\cite{wu2023tracer} introduces Xfer (token transfer) and Swap (token exchange), other critical semantics remain unmodeled, leaving a semantic gap that constrains the detection of diverse and evolving laundering strategies.
    
\item \textbf{L2: absence of fund flow awareness.} In account-based blockchains such as Ethereum, most AML approaches~\cite{wu2023towards,lin2024denseflow,wu2023tracer,lv2023detection,WU2026128900} construct address-level graphs and ignore the actual flow of funds between transactions. This omission makes it impossible to explicitly determine where the funds in a transaction originated and where they were sent. For example, in address-level graphs, if address A transfers 100 ETH to B and B subsequently sends 150 ETH to C, it is hard to determine how much of the 150 ETH originated from A’s transfer and how much came from B’s pre-existing balance. Such information is critical for identifying laundering patterns such as layering and integration. While some Bitcoin-focused studies~\cite{kuccuk2023investigation,bellei2024shape,nicholls2023fraudlens} model UTXO-level flows, these model methods are not directly applicable to account-based blockchains because account-based blockchains record only balance changes rather than explicit inputs and outputs.

\item \textbf{L3: lack of explainability in detection results.} Although recent AML models have improved detection accuracy, their outputs are typically limited to binary classification results~\cite{lv2023detection,kuccuk2023investigation,elmougy2023demystifying,nicholls2023fraudlens,lin2024denseflow,elmougy2023demystifying,wang2024graphalm,zhou2023visual}(suspicious or not). They rarely provide interpretable evidence for regulatory reports, such as Suspicious Activity Report~\cite{AMLWatcher} (SARs, which flag suspected money laundering and provide critical intelligence for regulators and law enforcement), limiting the system’s trustworthiness and real-world applicability.

\end{packeditemize}




\smallskip\
\noindent
\textbf{Our contributions.}
To address these limitations, we propose \techName{}, a novel security system for Crypto AML. To tackle \textbf{L1}, \techName{} parses transactions into four kinds of common behavioral intents to capture diverse laundering strategies that are invisible to prior research. To tackle \textbf{L2}, \techName{} constructs three kinds of fund flow subgraphs in account-based blockchains to reveal the source and destination of the funds. Building on these two components, \techName{} introduces a Semantics–Structure Fusion module, which aligns semantic representations encoded by an LLM with structural representations by graph convolutional networks (GCNs), leveraging a cross-attention mechanism. To tackle \textbf{L3}, \techName{} generates SARs, including fund flow visualizations, path summaries, and red-flag indicators, ensuring that detection results can support forensic investigation.
% To evaluate the effectiveness of  \techName{},
In summary, our contributions are as follows:

\begin{packeditemize}
    \item \textbf{Method:} We design and develop \techName{}, a novel security system for detecting and explaining money laundering transactions in blockchain networks, combining semantic awareness, fund flow awareness, and explainable report generation.
    \item \textbf{Evaluation:} We conduct extensive experiments on real-world ML transactions spanning 14 days, showing that \techName{} outperforms baselines, achieves high fund coverage, maintains generalization, and produces accurate and convincing SARs.
    \item \textbf{Insights:} We perform an in-depth analysis of laundering transactions detected by \textsc{FlowShield}, summarizing diverse laundering strategies and evasion behaviors, which provides insights for regulatory and investigative practice.

\end{packeditemize}


\input{Tabs/tab_comparision_methods}


==> chapter/1-introduction.tex <==
\section{Introduction} \label{sec:intro}


Billions\footnote{Within 2024, the resulted crypto economic losses reached up to \$2 billion, while less than 10\% of the illicit funds were eventually recovered, with the vast majority rapidly transferred and laundered \cite{report}.} in stolen crypto do not disappear — they flow. Through decentralized exchanges, bridges, and automated bots, illicit funds race across blockchains. Each hop fragments the trail: a swap here, a bridge there, an internal contract call in between. Within minutes, stolen assets are scattered across hundreds of addresses and multiple chains, leaving only cryptic traces of what really happened.

This form of \textit{cryptocurrency money laundering}\footnote{Crypto AML is the technique for tracing and preventing illicit on-chain fund flows.  
Unlike traditional AML~\cite{calafos2022cyber}, it deals with pseudonymous, multi-layered blockchain transactions beyond regulated intermediaries.} (Crypto ML)~\cite{campbell2018bitcoin} has become a central threat to blockchain security. Following major thefts and protocol exploits, launderers routinely automate laundering pipelines that disperse and disguise stolen assets before regulators can freeze them. These pipelines combine several basic paths (\textcolor{red}{P}):


\begin{packeditemize}
\item (\textcolor{red!80}{P1}) \textit{fund dispersal}~\cite{Dispersal}: Split large sums into many smaller transfers and distribute them across multiple addresses to obscure the origin and flow of funds.
\item (\textcolor{red!80}{P2}) \textit{token swap}~\cite{CoinSwapping}: Use decentralized exchanges (DEXs) to exchange one token for another, thereby obtaining more liquid-compatible tokens (e.g., ERC20). 
\item (\textcolor{red!80}{P3}) \textit{indirect transfer}~\cite{under25zhang}: Invoke smart contracts to indirectly transfer funds, executing multi-step internal transfers within a single visible transaction.
\item (\textcolor{red!80}{P4}) \textit{cross-chain transfer}~\cite{Crosschain}: Move funds across different blockchains via cross-chain bridges to break traceability and conceal the destinations of illicit funds.
\end{packeditemize}

Modern launderers rarely rely on a single path; instead, they chain multiple routes to maximize obfuscation. We show a real-world case below, which is in the largest crypto money laundering incident to date~\cite{bybit25}. This example captures a representative portion of the broader laundering flow.



% \vspace{-0.1in}
\begin{center}
  % \fbox{
% \colorbox{red!9}{
\colorbox{red!6}{
\begin{minipage}{0.95\linewidth}
  \textbf{Bybit Hack} (Figure~\ref{fig:intro}): the launderer address \hlhref{https://etherscan.io/address/0xfa3fcccb897079fd83bfba690e7d47eb402d6c49}{0xfa3f} dispersed stolen funds into multiple transfers to accomplices \hlhref{https://etherscan.io/address/0x515C1dd01E03387329384FBb64055A2A28901cEb}{{0x515c}} and \hlhref{https://etherscan.io/address/0xf45284cAb67b8E98f6462976Da1C1a7d39822612}{{0xf452}} (\textcolor{red!80}{P1}).  
\hlhref{https://etherscan.io/address/0x515C1dd01E03387329384FBb64055A2A28901cEb}{{0x515c}} repeatedly invoked a \hlhref{https://etherscan.io/address/0x515c1dd01e03387329384fbb64055a2a28901ceb}{LiFi router} for indirect transfers (\textcolor{red!80}{P3}) through the \hlhref{https://etherscan.io/address/0xd37bbe5744d730a1d98d8dc97c42f0ca46ad7146}{Thorchain bridge} (\textcolor{red!80}{P4}), which cross-chained the funds to Bitcoin address \hlhref{https://etherscan.io/tx/0x417f2ffbb6192d389100f860bc655188596aaa17666b2dc18c179e7fe821beaa\#eventlog}{{bc1qu4}}.  
Concurrently, \hlhref{https://etherscan.io/address/0xf45284cAb67b8E98f6462976Da1C1a7d39822612}{{0xf452}} forwarded assets to \hlhref{https://etherscan.io/address/0x86a302D73f785dEb3f933Ff5ab742B643C675dB6}{{0x86a3}}, which used an \hlhref{https://www.oklink.com/zh-hans/ethereum/address/0xf3de3c0d654fda23dad170f0f320a92172509127}{OKX router} to swap {ETH} for {DAI} and sent them to \hlhref{https://etherscan.io/address/0xD2422D70e23C9544B4754cb87787910381ac59eb}{{0xd242}}, where the DAI was swapped back to ETH (\textcolor{red!80}{P2}).

\end{minipage}
      }
 %  }
\end{center}

\smallskip
We observe two major challenges in tracing such laundering pipelines: 
(i) \emph{structure complexity}: dispersal and automated execution multiply endpoints and transactions, creating highly entangled graphs that obscure causal links and strain scalability; and (ii) \emph{trace discontinuity}: swaps, cross-chain hops, and internal contract calls break value continuity boundaries, so surface-level transaction views fail to reveal the true flow of funds. How, then, do we sniff out dirty money both smartly and swiftly?



%With the rapid development of the cryptocurrency (Crypto) ecosystem, blockchain has not only fueled the prosperity of decentralized finance (DeFi) but has also become the foundation of various emerging financial applications~\cite{shirole2020cryptocurrency}. However, the pseudonymous nature~\cite{lubbertsenghost} of blockchain poses significant threats to financial security~\cite{LI2020841}, because it facilitates illicit activities such as scams, stolen funds, and ransomware attacks~\cite{291271}.  Blockchain security incidents in 2024 resulted in economic losses of up to \$2 billion in crypto, while less than 10\% of the illicit funds were eventually recovered, with the vast majority rapidly transferred and laundered \cite{report}. Following such incidents, illicit funds are often moved immediately through complex transaction paths and diverse obfuscation tools for laundering, known as cryptocurrency money laundering (Crypto ML), which has become a critical threat to the security of the blockchain financial system.



%https://www.csis.org/analysis/bybit-heist-and-future-us-crypto-regulation

%P2:介绍洗钱典型手法（新加的）
% 随着区块链的可编程性与跨链互操作性不断增强，洗钱手法也日趋多样与复杂。图X展示了典型的洗钱手法：（dispersal）将大额资金转移到大量地址以增加追踪分支； （token swap）借助去中心化交易所（DEX）换币以改变资产形态并获取更高流动性或便于跨链搬运的代币； （cross-chain transfer）通过跨链桥将资产从一条链迁移到另一条链以扩展分析域并利用链间差异； （indirect transfer）通过调用智能合约完成间接转账，将多步资金流封装在单次链上交互中； （automation transaction）以及通过交易机器人批量并行执行相似交易以放大规模与速度。(加个图解释)。

%Question:
%1. techniques or strategies?
%2. 需要在这里加图描述这几种手法嘛？
%3. Fund dispersal: 这里用：还是.比较合适？还是都行
% 加news

%\heading{Crypto ML.}
%Driven by advances in blockchain programmability and cross-chain interoperability, Crypto ML techniques have become increasingly diverse and sophisticated. There are several representative Crypto ML techniques:


%P3：洗钱案例（新加的）
% 今年 2 月发生的 Bybit 事件（约 14.6 亿美元被盗）呈现出典型的复合洗钱流程。事件初期，攻击者通过 Uniswap、Paraswap 等去中心化交易所将被盗的 stETH、mETH 等衍生资产兑换为 原生代币ETH，以提高后续搬运的灵活性。随后，资金通过前述五类手法被有策略地分层清洗，形成多条复杂的资金流。图X 展示了其中一条具有代表性的洗钱支路：洗钱地址0x515c连续接收来自同一上游洗钱地址的多笔资金，这些交易金额相近，呈现出明显的自动化交易的特点。每当收到一笔资金后，该地址立即调用 LI.FI: LiFi Diamond 合约，将 ETH 间接转至 Thorchain 跨链桥的 Router 合约，并借助 Thorchain 将资金跨链转移至比特币区块链上的同一个地址 bc1qu4jhsz3uf4zdr7v46ssf0904ghyutafaqmv83j。这一过程充分体现了合约封装、跨链桥接与自动化执行等洗钱手法的协同使用，进一步加剧了资金追踪与路径还原的难度。

%In February 2025, the Bybit hack incident (Figure~\ref{fig:intro}), , demonstrated typical Crypto ML techniques.   One laundering address 0xfa3f splits funds into multiple transfers and distributes them to downstream accomplice addresses~\hlhref{https://etherscan.io/tx/0xb4eb16ea61bad86184b02075f8e8f7c64e95b60f8a6b8ec199093a0ccadfc9f9}{0x515c} and~\hlhref{https://etherscan.io/tx/0x9927c310f27a689d17dca9a70d8692399daa583c772da56c2d998ddd6a60fcc0}{0xf452}. Upon receiving each transfer, 0x515c repeatedly executes an ~\hlhref{https://etherscan.io/tx/0x417f2ffbb6192d389100f860bc655188596aaa17666b2dc18c179e7fe821beaa}{automated} sequence: it invokes a LiFi router contract to perform an indirect transfer to Thorchain bridge router,  and Thorchain then cross-chains the funds to address ~\hlhref{https://etherscan.io/tx/0x417f2ffbb6192d389100f860bc655188596aaa17666b2dc18c179e7fe821beaa\#eventlog}{bc1qu4} on Bitcoin Blockchain. Meanwhile, 0xf452 forwards the funds to ~\hlhref{https://etherscan.io/tx/0xd30ca809634fe71dd8bfb1a831539b1bc35cc7aeab0c078f7b699c6bd80ae34a}{0x86a3}, which uses an OKX router contract to~\hlhref{https://etherscan.io/tx/0x7482331f19bfef6b0aee250bb59adf646cf5c1c2329c066a0f4af01ddcf7425c}{swap} ETH into DAI and sends them to~\hlhref{https://etherscan.io/tx/0xc57467e1a32a470b3b2be6778d83a316c557ed5dbedf7d83ab484af75d70b532}{0xd242}. 0xd242 subsequently ~\hlhref{https://etherscan.io/tx/0xea171e141b58174d80de7e94e953ec92628195c3a6f64668f904bf5f42e862d1}{swap} the DAI back to ETH via the OKX router.


% In February 2025, the Bybit hack incident~\cite{bybit25}, the largest blockchain financial security incident to date, demonstrated typical Crypto ML techniques. In the early stage, the launderers converted the stolen tokens, such as stETH and mETH, into native ETH through DEXs like Uniswap and Paraswap. %increasing the flexibility of subsequent fund movements. 
% The illicit funds were then strategically laundered through multiple Crypto ML techniques. Figure~\ref{fig:intro} illustrates one representative laundering process~\footnote{\href{https://etherscan.io/address/0x515c1dd01e03387329384fbb64055a2a28901ceb}{Representative laundering information on Etherscan}}. The laundering address 0x515c continuously received a similar amount of ETH from the same upstream laundering addressc 0x3a21, which shows clear signs of automated execution. Upon receiving each transfer, 0x515c immediately invoked the LiFi Diamond contract to indirectly transfer ETH to Thorchain’s Router contract, and then leveraged Thorchain to bridge the funds to the Bitcoin blockchain, specifically to the same address bc1qu4. 

%还缺少对图中完整的描述（新增了一个分支的例子）

% 今年 2 月发生的 Bybit 事件（约 14.6 亿美元被盗）呈现出典型的复合洗钱流程。图X 展示了其中一条具有代表性的洗钱支路：洗钱地址0xfa3f 将资金拆分为多笔分别发送给同伙地址0x515c和0xf452。0x515c 在收到每笔款项后重复性地执行自动化流程：调用 LiFi 的路由合约，将 ETH 以间接方式传递至 Thorchain 的桥路由合约，进而借助 Thorchain 将资金跨链转至同一比特币地址。与此同时，0xf452 将款项转给 0x86a3，0x86a3 通过 OKX 路由合约将 ETH 换成大量 DAI 并转给 0xd242，随后 0xd242 再通过 OKX 路由将 DAI 换回 ETH。



\begin{comment}
\begin{figure}[h]
\centering
\begin{subfigure}{0.46\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figs/example_ml_technique_1.pdf}
  \caption{Transaction-level graph showing raw transactions.}
  \label{fig:eg_1}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figs/example_ml_technique_2.pdf}
  \caption{Semantic-level abstraction illustrating Crypto ML techniques.}
  \label{fig:eg_2}
\end{subfigure}
\caption{A typical example of Crypto ML flow from Bybit hack incident. \qs{comment about fig.1}}
\label{fig:intro}
\end{figure}
\end{comment}



%P4:洗钱手法带来了挑战（新加的）
% 这些链上洗钱手法给资金溯源带来了双重挑战：
% C1: Structural Complexity 结构复杂：攻击者通过Fund dispersal和Automated transaction拆分大额资金并在批量执行相似交易，导致洗钱交易和洗钱地址数量急剧膨胀，生成复杂的洗钱网络结构。
% C2: Link Discontinuity 链路断裂： （token swap）、跨链转移（cross-chain transfer）与合约内中转（indirect transfer）分别从代币变化、跨区块链、合约调用的角度断开资金链路，资金在表层交易视图中不连续，难以只利用基础交易信息来还原真实的资金传播路径，
%这两类挑战共同削弱了资金来源与去向之间的逻辑联系，使得洗钱资金呈现出结构复杂而链路断裂的特征。

%Question:
%1. 这两点挑战总结的合适嘛？会有overlap嘛？
%2. 突然想到洗钱者用attacker表示还是Launderer来表示更好呢？
%3. 这段首句有点干巴巴.... 在这前面加点什么过渡句比较好呢



% --废弃这段，这段写的不清楚，我觉得需要分点概括一下! 这些链上洗钱手法给资金溯源带来了挑战，他们削弱了资金来源与去向之间的逻辑链条削弱，制造了“可见但难解”的混淆现象。首先，资金经多次拆分与再分配后混合了来自不同来源的资金，使得单笔资金的上游来源与下游去向难以精确定位；其次，若不识别换币行为的代币种类与换前换后金额关系，资金链在语义层面即被截断，后续追踪失去连续性；此外，跨链转账会在不同区块链上留下不连续的交易记录，若不能解析桥事件并建立链间对应关系，就无法确定赃款最终落在哪条链的哪个地址；第四，智能合约的内部调用常将多步交易封装为表面上的单次交易，从而隐藏真实的资金流；最后，自动化执行交易使得洗钱交易数量爆炸，进一步加剧还原难度。这些洗钱手法共同增加了洗钱交易的结构复杂性和意图复杂性，致使仅凭基础交易信息难以还原接近真实的资金传播路径。

%P5:现有AML工作的limitations
% \heading{Crypto AML.}
% Crypto AML~\cite{campbell2018bitcoin} refers to the set of techniques and systems designed to detect, analyze, and prevent illicit fund flows within blockchain ecosystems. Unlike traditional AML~\cite{calafos2022cyber}, which relies on regulated intermediaries and fiat transaction monitoring, Crypto AML operates directly on blockchain data, where transactions are pseudonymous, often involve complex layering processes, and exhibit diverse types. 

% Prior research on Crypto AML can be broadly categorized into three types: heuristic rule-based methods~\cite{wu2023towards,lv2023detection,kuccuk2023investigation}, which rely on predefined suspicious behavior patterns; traditional machine learning-based methods~\cite{elmougy2023demystifying,wang2024graphalm,zhou2023visual}, which extract features from transaction data and train classifiers; graph-based methods~\cite{wu2023tracer,lin2024denseflow,wu2023tracer}, which exploit structural relationships among accounts or transactions. These methods are effective in detecting certain money laundering activities. However, they remain inadequate when confronted with the growing sophistication of laundering strategies. As summarized in Table~\ref{tab:aml_comparison}, their major limitations are as following:


%Crypto AML~\cite{campbell2018bitcoin} refers to the set of techniques and systems designed to detect, analyze, and prevent illicit fund flows within blockchain ecosystems. Unlike traditional AML~\cite{calafos2022cyber}, which relies on regulated intermediaries and fiat transaction monitoring, Crypto AML operates directly on blockchain data, where transactions are pseudonymous, often involve complex layering processes, and exhibit diverse types. 


%需要在这里说明：前人的方法不可以同时用在UTXO-based和Account-hased

\subsection{Why Existing Solutions Fall Short} 

We briefly review existing crypto AML approaches.
They fall into three categories: 

\begin{packeditemize}

\item \textit{Rule-based heuristics} approaches rely on manually defined rules derived from known laundering patterns, such as blacklist matching~\cite{wu2023towards} and cyclic flows~\cite{lv2023detection}.  They are straightforward and effective based on rich experience.

%They are straightforward and effective in capturing previously observed typologies but lack generalization. Once adversaries alter scripts or layer new protocols, static rules quickly become obsolete.

\item \textit{Machine learning} approaches train classifiers on statistical features extracted from transactions, leveraging techniques such as feature refinement~\cite{elmougy2023demystifying}, active learning~\cite{wang2024graphalm}, and anomaly detection~\cite{zhou2023visual}. 

%While more adaptive than rule-based systems, their performance depends on handcrafted feature engineering and they often overlook inter-transaction dependencies essential to fund-flow reasoning.

\item \textit{Graph-based} approaches model transaction records as a graph and identify suspicious accounts or subgraphs through subgraph search (DenseFlow~\cite{lin2024denseflow}, Tracer~\cite{wu2023tracer}) or graph neural networks~\cite{alarab2020competence,nicholls2023fraudlens,weber2019anti}. 

%Despite their improved ability to capture structural correlations, they remain largely \emph{structure-centric}: transaction semantics are ignored, and the resulting detections are difficult to interpret or justify in compliance workflows.
%,lo2023inspection, guo2023lb

\end{packeditemize}


\smallskip
Despite their differences, these approaches share core limitations (\textbf{L}). We reinterpret technically as follows:


\begin{packeditemize}
%L1： Limited Understanding of Diverse Laundering Intents.
%现有加密货币反洗钱研究普遍将区块链交易视作同质化的资金转移，忽视了交易背后的洗钱意图。在现实场景中，洗钱者会通过多种交易行为来隐藏资金来源、切断追踪路径。这些洗钱交易行为反映了不同的意图，referred to as transaction semantics, 是刻画复杂洗钱行为的重要依据。然而，现有研究仅对少部分语义进行建模，仍存在显著的语义空缺，导致模型难以识别多样化的洗钱交易。

\smallskip
\item \textbf{L1: Limited understanding of advanced or combined laundering techniques.}  
Most AML methods~\cite{alarab2020competence,elmougy2023demystifying,lin2024denseflow,lv2023detection,nicholls2023fraudlens,wang2024graphalm,weber2019anti,wu2023towards,zhou2023visual} treat blockchain transactions as direct transfers, ignoring the rich transaction intents. In reality, blockchain transactions encompass not only direct transfers but also token swaps, cross-chain transfers, and indirect contract-mediated transfers. These high-level behavioral intents, referred to as transaction semantics, are crucial for characterizing and detecting complex laundering patterns. Although Tracer~\cite{wu2023tracer} introduces Xfer (token transfer) and Swap (token exchange), other critical semantics remain unmodeled.
\end{packeditemize}

\smallskip
\noindent\textit{Why this is hard?} Extracting semantics requires reconstructing the logical purpose of each transaction from event logs\footnote{Event logs are structured records emitted by smart contracts that describe on-chain actions such as transfers or calls.}. Even subtle differences in router design can blur whether a transaction is a swap, bridge, or internal forwarding. For example, two Ethereum transactions may appear identical: both emit {Transfer} events (topic0$=${0xddf2}) to the same router address with the same selector. Yet one performs a same-chain DEX swap, while the other triggers a deposit that locks assets on Ethereum and mints on the destination chain. The surface traces align, but the intents diverge. 

%Existing parsers lack the cross-protocol generalization to recover such high-level behaviors systematically.


\smallskip
\begin{packeditemize}
\item \textbf{L2: Limited capabilities in tracking fund flow.}  
In account-based blockchains such as Ethereum, most AML approaches~\cite{lin2024denseflow, lv2023detection, wu2023towards,wu2023tracer} construct address-level graphs and ignore the actual flow of funds between transactions. 
This abstraction makes it impossible to pinpoint how value propagates across transactions. For instance, if address $A$ transfers 100~ETH to $B$, and $B$ subsequently sends 150~ETH to $C$, traditional models cannot tell how much of the 150~ETH originated from $A$ versus $B$’s existing balance. Such ambiguity obscures the true flow of funds across dispersal, making laundering flows difficult to trace. While UTXO-based methods~\cite{elmougy2023demystifying,nicholls2023fraudlens,weber2019anti} explicitly model inputs and outputs, they are confined to the Bitcoin-style ledger design and cannot extend to account-based systems.
\end{packeditemize}

\smallskip
\noindent\textit{Why this is hard?}  
UTXO and account-based models differ fundamentally in transaction semantics.  
UTXO records explicit inputs and outputs~\cite{qi2025sok}, enabling precise fund provenance tracking. Account-based ledgers only store net balance updates, implicitly mixing multiple inflows and outflows in one state variable. This aggregation breaks deterministic fund lineage. Bridging the two paradigms requires reconstructing virtual UTXOs from balance deltas or building hybrid models that combine address topology with value-transfer semantics. Existing efforts remain specialized to either UTXO or account models, failing to generalize across both and leaving cross-ledger laundering untracked.


\smallskip
\begin{packeditemize}
\item \textbf{L3: Lack of user-friendly explainable results.}  
Although recent solutions improved detection accuracy, their outputs are typically limited to binary classifications~\cite{alarab2020competence,elmougy2023demystifying,lin2024denseflow,lv2023detection,nicholls2023fraudlens,wang2024graphalm,weber2019anti,wu2023tracer,wu2023towards,zhou2023visual}  (laundering or not).  
% They rarely provide interpretable evidence that investigators can incorporate into Suspicious Activity Reports (SARs)~\cite{AMLWatcher}, which require explicit transaction linkages, fund-flow provenance, and interpretable behavioral context.
They rarely provide interpretable evidence that reveals how suspicious funds propagate, where swaps or cross-chain transfers occur, or what abnormal behavioral patterns arise.  This limits their usefulness in investigation and forensics, and falls short of SAR~\cite{AMLWatcher} requirements for explicit transaction linkages, fund-flow provenance, and interpretable behavioral evidence.
\end{packeditemize}

\smallskip
\noindent\textit{Why this is hard?}  
Graph-based or deep learning models compress multi-hop transaction dependencies into high-dimensional embeddings, obscuring the causal paths between transactions.  
% For instance, a GNN node may be classified as ``suspicious'' based on aggregated neighborhood features, yet the model cannot reveal which specific transfers led to that conclusion.  
For instance, a GNN may flag an address or transaction as laundering based on aggregated neighborhood features, yet it cannot reveal which specific transfers led to that conclusion.
Similarly, statistical classifiers detect outliers in feature space but discard the underlying transactional structure. Generating explainable and audit-ready outputs requires models that can both reason over structured flow graphs and verbalize those results in user-friendly form.




\begin{figure}[t]
\centering
  % \includegraphics[width=\linewidth]{Figs/example_ml_technique_2.png}
    \includegraphics[width=0.98\linewidth]{Figs/bybit_case.pdf}
\caption{A typical laundering segment of Bybit Hack.}
\label{fig:intro}
\end{figure}



\subsection{Our Approach}

% \qs{add ref}

We present \textsc{FlowShield}, a new framework for detecting and explaining Crypto ML transactions. \textsc{FlowShield} closes the three gaps through an integrated pipeline that (i) parses transaction \emph{semantics}, (ii) reconstructs fine-grained \emph{fund-flow} subgraphs, and (iii) fuses semantics and structure for accurate and explainable detection. 

We show how we make it in a stepwise manner. 

\begin{itemize}
  \item \textbf{Semantic parsing of laundering behaviors}~(\S\ref{subsec-semantic}).
\end{itemize}

%与将链上交互简单视为“转账”不同，\textsc{FlowShield} 通过解析事件日志并分析交易组内部的关系结构来恢复交易背后的高层意图。我们将异构协议中常见的交互模式归纳为四类规范化语义：\emph{直接转账}、\emph{代币交换}、\emph{跨链转移}和\emph{合约中继式转发}。这些语义由事件信息、token 变化轨迹、地址之间的衔接关系以及交易组中的路径结构综合推断，从而能够区分表面结构相似的不同行为。例如，在同一个交易组中，如果某笔转账的发送者恰好出现在另一笔转账的接收者位置，且两者涉及不同的代币，则为一次代币交换；对于跨链操作，通过解析事件日志中跨链相关字段，从而将其与代币交换区分。语义层的构建使这些高层行为得以被显式化，从而为后续的洗钱检测提供更具判别力的特征基础。
(\textit{addressing L1}) Rather than treating each on-chain interaction as a direct transfer, \textsc{FlowShield} recovers the \emph{intent} behind a transaction by parsing its event logs and analyzing the relational structure within the transaction group. We normalize heterogeneous protocols into four canonical intents that frequently compose laundering pipelines: \emph{direct transfer}, \emph{token swap}, \emph{cross-chain transfer}, and \emph{indirect (contract-mediated) transfer}. These semantics are inferred by combining event logs, token transition patterns, address linkages, and the path structure formed among the transaction group, disambiguating ambiguities that defeat prior work. For instance, within the same transaction group, if the sender of one transfer reappears as the recipient in another and the two involve different tokens, the interaction is as a token swap. For cross-chain operations, parsing bridge-specific fields in the event logs makes them distinguishable from same-chain swaps. By making such high-level behaviors explicit, the semantic layer provides more discriminative features for downstream laundering detection.
  

% Ambiguities that defeat prior work are disambiguated using contextual signals; e.g., two transactions may both emit ERC-20 {Transfer} events and invoke the same swap selector, yet one is a same-chain swap while the other is a bridge deposit. The semantic layer exposes behavior that address-level models miss and provides protocol-agnostic features for downstream detection.

\begin{itemize}
  \item \textbf{Fund-flow reconstruction}~(\S\ref{fund_flow_aware}).
\end{itemize}

(\textit{addressing L2})  To restore value provenance that is absent in address graphs, \textsc{FlowShield} maintains \emph{transaction-level flow subgraphs}. Instead of linking addresses, we model how value moves between transactions over time. Concretely, we build three complementary subgraph views:  
(i) \emph{Inflow provenance} subgraphs capture where the value consumed by a transaction originates (distinguishing fresh inflows from pre-existing balances);  
(ii) \emph{Outflow redistribution} subgraphs capture how the value produced by a transaction is split and forwarded downstream;  
(iii) \emph{Parallel-flow} subgraphs identify value-aligned and structurally similar transactions, revealing parallel or coordinated flows.
This hybrid view approximates virtual-UTXO lineage on account-based chains and bridges the modeling gap with UTXO systems, enabling precise recognition of layering, structuring, and integration patterns even when funds are mixed within balances.

% \textit{iii)} \emph{Temporal dependency} subgraphs encode short-horizon ordering/amount constraints to reduce spurious linkages under concurrency.  

\begin{itemize}
  \item  \textbf{Semantics–structure fusion}~(\S\ref{subsec-fusion}) and \textbf{SAR explanation}~(\S\ref{subsec-sar}).
\end{itemize}
% (\S\ref{subsec-fusion}-\S\ref{subsec-sar})

(\textit{addressing L3}) Detection quality and forensic usability hinge on \emph{both} what a transaction means and how value propagates. To address this, \textsc{FlowShield}: (i) aligns \emph{semantic embeddings} (capturing intent) with \emph{structural embeddings} (capturing flow) via a cross-attention fusion module.  The fused representation primarily supports a high-precision laundering detector that is sensitive to diverse laundering behaviors; (ii) passes these laundering flows to an LLM, which generates SAR-ready outputs, including concise flow summaries (who/what/when/how much), and red-flag rationales. These artifacts turn model decisions into audit-ready evidence for compliance workflows.

%The fused representation supports two outputs:  
% (i) a high-precision laundering detector that is sensitive to composed behaviors (e.g., swap$\to$multi-hop dispersal$\to$bridge); and  
% (ii) an explanation generator that compiles SARs with investigator-oriented artifacts: flow diagrams of the implicated paths, concise natural-language summaries (who/what/when/how-much), and rule-linked red-flag rationales. These artifacts turn model decisions into audit-ready evidence for compliance workflows.

\smallskip
Then, \textbf{we implement and evaluate\footnote{\techName{} code is available at \url{https://osf.io/9s3j2/overview?view_only=9b15fcf6978b47ddbdcc8a850d1666c9}} \textsc{FlowShield} on our newly curated dataset, \textit{BybitML}}~(\S\ref{sec:exps}).

% \qs {link}
% \footnote{Released at \url{https://osf.io/nx7aj/overview?view_only=663038fbea43491bb4010011c7f28b23}.}

\textit{BybitML}\footnote{\textit{BybitML} dataset is released at \url{https://osf.io/nx7aj/overview?view_only=663038fbea43491bb4010011c7f28b23}.} is a multi-chain laundering dataset derived from the Bybit Hack incident. It spans a range from  February 21 to March 6, 2025, covering over 2.75M transactions across Ethereum and Bitcoin.  
To construct it, we traced laundering paths using public explorers (\hlhref{https://etherscan.io/}{Etherscan}, \hlhref{https://www.oklink.com/}{OKLink}) and bridge logs (\hlhref{https://thorchain.org/}{Thorchain}).  
Each transaction was semantically labeled into four behavioral intents (i.e., direct transfer, token swap, indirect transfer, and cross-chain transfer).  
We further conducted multi-source validation and manual tracing to establish ground-truth laundering flows.  
The final dataset is divided into two synchronized subsets: \textit{BybitML-EC} (Ethereum) and \textit{BybitML-BC} (Bitcoin). 


% Cross-chain mappings were then aligned by temporal correlation and bridge contract verification.


We benchmark \textsc{FlowShield} against AML approaches spanning heuristic, machine-learning, and graph-based methods (Table~\ref{tab:aml_comparison}). Results (\S\ref{sec:exps}) show that


\begin{packeditemize}
    \item \textbf{High detection performance.} \textsc{FlowShield} improves F1 by +6.2\% on Ethereum and +9.1\% on Bitcoin, with fund coverage of 88\% and 98.2\%, respectively.  Ablation studies show the necessity of each component of \textsc{FlowShield}, as removing any one degrades performance.
    
    \item \textbf{Laundering strategy analysis.} \textsc{FlowShield} tracks how laundering semantics shift over time , exposes common evasion behaviors, and uncovers dominant cross-chain migration routes, tracing over US\$930M and linking 1,878 Bitcoin addresses to their upstream Ethereum flows.
    
    \item \textbf{Practical robustness and scalability.} Cross-period evaluations show stable performance, and inference runs at near real-time speed, enabling large-scale deployment.
    
    \item \textbf{High-quality SAR generation.} \textsc{FlowShield} generates explainable SARs with an average expert score above 8.5/10 in correctness, clarity, and convincingness. 
    
\end{packeditemize}

% \begin{packeditemize}
%     \item achieves an average F1 improvement of +6.2\% on Ethereum and +9.1\% on Bitcoin, with fund coverage of 88\% and 98.2\%, respectively. 
    
%     \item accurately recovers diverse laundering semantics and reveals dominant cross-chain migration routes from Ethereum to Bitcoin, tracing over US\$930M in illicit assets and linking 1,878 downstream Bitcoin addresses to upstream Ethereum flows.  
    
%     \item generates explainable SARs with an average expert score above 8.5/10 in correctness, clarity, and convincingness. 
    
% \end{packeditemize}
 
\smallskip
To be noted, we further conducted \textbf{responsible actions and disclosure} to the mainstream AML communities\footnote{Accessible at \url{https://www.lazarusbounty.com/en}. 
We reported a verified subset of key laundering transactions invloving 300,000~ETH and 5,019,091~USDT, covering major cross-chain transfers, swap routes, and deposits to exchanges.}.  
%27615枚ETH和5019091枚USDT （关键洗钱交易）

We summarized key findings and high-risk laundering patterns identified in \textit{BybitML}, including bridge-based cross-chain migration and automated dispersal strategies, and submitted anonymized reports to relevant intelligence platforms for validation.  
Only aggregated, non-identifiable transaction information was disclosed to ensure compliance with data-handling and ethical research standards.  

%\qs{add importance}

\smallskip
Last, we make a brief \textbf{clarification of our study and excluded scope.}  We focus on blockchain-native laundering detection and operate solely on publicly available on-chain data, without relying on private exchange records, off-chain KYC information, or proprietary blacklists.  

We cover the upstream phases of anonymity-enhanced laundering, detecting illicit flows before they enter privacy mechanisms. Privacy coins, and centralized exchange mixers are excluded. These stages constitute only a minor portion of laundering activity~\cite{LazarusBounty} ($<$20\% laundering value). 

%The scope of our study. 本研究专注于检测区块链上的多样洗钱交易行为，并提供解释性的结果供取证分析。通过收集公共区块链的交易数据，并进行语义解析和资金流重构，识别典型的四大洗钱行为（资金分散、换币、间接转账、跨链转移）。其中跨链洗钱检测是聚焦于识别不同区块链之间的黑钱流向，如检测某一地址在源区块链上将代币兑换至目标区块链的另一地址。这弥补了现有反洗钱研究无法识别跨链迁移的空白，为后续的全链资金追踪提供了关键信息。


%We focus on detecting diverse Crypto ML behaviors and generating explainable results to support forensic analysis. Based on public blockchain transaction data, \techName{} performs semantic parsing and fund-flow reconstruction to identify four representative laundering behaviors: fund dispersal, token swapping, indirect transfer, and cross-chain transfer. In particular, cross-chain laundering detection focuses on identifying the flow of illicit funds across different blockchains, for example, detecting when an address on the source chain exchanges tokens to another address on a destination chain. This capability fills a key gap in existing AML research that lacks cross-chain laundering detection and provides essential information for subsequent full-chain fund tracing.


\begin{comment}
    

We propose \techName{}, a novel security system for Crypto AML. To tackle \textbf{L1}, \techName{} parses transactions into four kinds of common behavioral intents to capture diverse laundering strategies that are invisible to prior research. To tackle \textbf{L2}, \techName{} constructs three kinds of fund flow subgraphs in account-based blockchains to reveal the source and destination of the funds. Building on these two components, \techName{} introduces a Semantics–Structure Fusion module, which aligns semantic representations encoded by an LLM with structural representations by graph convolutional networks (GCNs), leveraging a cross-attention mechanism. To tackle \textbf{L3}, \techName{} generates SARs, including fund flow visualizations, path summaries, and red-flag indicators, ensuring that detection results can support forensic investigation.
% To evaluate the effectiveness of  \techName{},

\heading{Contributions.} The contributions of the work can be summarized as follows:


Table~\ref{tab:aml_comparison}

\begin{packeditemize}
    \item \textbf{Method:} We design and develop \techName{}, a novel security system for detecting and explaining money laundering transactions in blockchain networks, combining semantic awareness, fund flow awareness, and explainable report generation.
    \item \textbf{Evaluation:} We conduct extensive experiments on real-world ML transactions spanning 14 days, showing that \techName{} outperforms baselines, achieves high fund coverage, maintains generalization, and produces accurate and convincing SARs.
    \item \textbf{Insights:} We perform an in-depth analysis of laundering transactions detected by \textsc{FlowShield}, summarizing diverse laundering strategies and evasion behaviors, which provides insights for regulatory and investigative practice.
    \item \textbf{Dataset and code:}

\end{packeditemize}
\end{comment}



%
\begin{table*}[t]
\centering
% \qw{maybe more metrics?}
\caption{Comparison of typical Crypto AML methods.}\label{tab:aml_comparison}
%没有给AML方法取名字的paper，我把作者的姓放在AML那一列了hh 
%没问题 一般也是这样处理的！
%\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|cc|cccc|cc}
\toprule
\multirow{2}{*}{\textbf{Crypto AML}} 
&  \multirow{2}{*}{\textbf{Method}} 
& \multirow{2}{*}{\textbf{Dataset (Year)}} 
& \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Blockchain}}} 
& \multicolumn{4}{c}{\textbf{Path}} 
& \multirow{2}{*}{\makecell[c]{\textbf{Laundering}\\\textbf{flow}}}  
& \multirow{2}{*}{\makecell[c]{\textbf{Explainable}\\\textbf{result}}} \\
 \cmidrule(lr){6-9}
 &  & & UTXO & Account & \textcolor{red!80}{P1} & \textcolor{red!80}{P2} & \textcolor{red!80}{P3}  & \textcolor{red!80}{P4}  &   \\
\midrule
Youssef\cite{elmougy2023demystifying} & Machine learning & \textit{Elliptic}~(2019) &\greencheck & \redx & \greencheck &  \redx & \redx &   \redx & \greencheck &  \redx \\
FraudLens\cite{nicholls2023fraudlens} & Graph-based       & \textit{Elliptic}~(2019)  & \greencheck & \redx & \greencheck &  \redx & \redx & \redx & \greencheck  & \redx \\
Weber\cite{weber2019anti} & Graph-based     & \textit{Elliptic}~(2019) & \greencheck & \redx & \greencheck &  \redx & \redx & \redx & \greencheck  & \redx \\
Cyclic\cite{lv2023detection}    & Heuristic & \textit{Not available} & \redx & \greencheck &  \greencheck & \redx & \redx & \redx & \redx & \redx \\
XBlock\cite{wu2023towards}   & Heuristic & \textit{EthereumHeist}~(2022) &\redx & \greencheck &  \greencheck& \redx & \redx & \redx & \redx & \redx \\
DenseFlow\cite{lin2024denseflow} & Graph-based & \textit{EthereumHeist}~(2022) &\redx & \greencheck &  \greencheck& \redx & \redx & \redx & \redx & \redx \\
Tracer\cite{wu2023tracer}    & Graph-based & \textit{Not available} & \redx & \greencheck &  \greencheck&  \greencheck& \redx & \redx &  \greencheck& \redx \\
\midrule
\rowcolor{gray!10}
 \techName{}  & Graph + LLM    & \textit{BybitML}~(2025) &\greencheck & \greencheck &  \greencheck&  \greencheck&  \greencheck&  \greencheck&  \greencheck&  \greencheck\\
\bottomrule
\end{tabular}
%}
\end{table*}





==> chapter/2-backgraound.tex <==
\section{Background} \label{sec:back}

\subsection{Blockchain Transaction Model}

Blockchain transaction models can generally be categorized into two types: account-based~\cite{wood2014ethereum} and Unspent Transaction Output (UTXO)-based~\cite{nakamoto2008peer} models. In both models, addresses are pseudonymous~\cite{zhang2019security}, meaning they are publicly visible on the blockchain but are not directly linked to real-world identities, and they can be generated without limitation. In the account-based model (e.g., Ethereum), each account has a unique address, and transaction records typically include the sender address, receiver address, transferred amount, token name (the cryptocurrency transferred), time, gas fee, and event logs. Account-based blockchains support interactions with smart contracts~\cite{wood2014ethereum}, enabling more diverse transaction types, such as token swaps on decentralized exchanges~\cite{malamud2017decentralized} and token transfers to other blockchains via cross-chain bridges~\cite{ou2022overview}. While the UTXO model (e.g., Bitcoin) does not support smart contracts. It is based on unspent transaction outputs, where transactions consume one or more previous outputs and create new outputs to transfer value. Address information in this model must be obtained by parsing the previous outputs referenced by the transaction inputs~\cite{conti2018survey}.

\subsection{Crypto ML}
%%%%% Not that important, let's save some space here %%%%%
% Cryptocurrencies (Crypto) are decentralized digital assets built on blockchain technology~\cite{shirole2020cryptocurrency}. The decentralized architecture and global accessibility of Crypto enable cross-border fund transfers without central intermediaries, while programmability allows blockchains supporting smart contracts to facilitate diverse transfers. Although these features have driven the growth of the digital economy, they have also provided new means for criminals to covertly move funds, giving rise to cryptocurrency money laundering (Crypto ML) as an emerging form of financial crime.

Cryptocurrency money laundering (Crypto ML) is the process by which criminals exploit cryptocurrencies on blockchain networks to convert illicit funds into ones that appear legitimate. Compared to traditional money laundering, Crypto ML is characterized by a variety of transaction types and laundering tools, pseudonymous addresses, and generating new addresses freely~\cite{sok25fu}. These characteristics enable highly complex fund flow patterns that effectively obscure the true origin of the assets.

As shown in the part \circlednum{1} to \circlednum{3} of Figure~\ref{fig:threat}, the laundering process typically unfolds in three stages~\cite{wu2023towards}: \circlednum{1}  Placement: Illicit funds are introduced into laundering addresses controlled by criminals on the blockchain; \circlednum{2}  Layering: The movement of funds is obfuscated through techniques such as multi-hop transfers, token swaps, cross-chain transfers~\cite{bridge}, or the use of mixing services, thereby reducing traceability; \circlednum{3}  Integration: The “cleaned” funds are reintroduced into the legitimate economy. Among these, the layering stage is the most complex, often involving combinations of multiple techniques, and is therefore the primary focus and challenge in cryptocurrency anti-money laundering efforts.


% \subsection{}





==> chapter/3-threat-model-old.tex <==


%All papers submitted should provide a threat model that clearly articulates the (i) envisioned attacker(s), (ii) threat surfaces (e.g., system components including but not limited to the underlying machine learning algorithm), (iii) generality and (iv) practicality of the attack.
\begin{figure}[th]
\begin{center}
\includegraphics[width=0.5\textwidth]{Figs/threat model num.pdf}
\end{center}
\caption{\label{fig:threat} Crypto ML and its Threat model.}
\end{figure}

% \cleardoublepage
\section{Threat Model} \label{sec:threat}

Figure~\ref{fig:threat} illustrates the overall threat model Crypto ML, highlighting the attack process and the corresponding defense process of AML detection and forensics. In the following, we detail the threat scenario, the attacker’s capabilities, the victim profile, and the defender’s capabilities.

\heading{Threat scenario.} In a typical cryptocurrency money laundering incident, as the part \circlednum{1} to \circlednum{3} of Figure~\ref{fig:threat}  shows, the attacker first acquires substantial illicit funds from the victim through hacking, fraud, ransomware attacks, and so on. Once these funds are transferred to addresses under the attacker’s control on the blockchain, the attacker employs various techniques to launder the funds. Following the incident, as the part \circlednum{4} to \circlednum{6} of Figure~\ref{fig:threat} shows, defenders attempt to identify suspicious laundering transactions and trace the associated fund flows from transaction data on the blockchain. Defenders then generate SARs to support AML compliance teams and law enforcement agencies~\cite{FAFT} in taking timely actions, such as freezing the detected funds to prevent further transfers or cash-outs.

\heading{Attacker capabilities.} ~~The envisioned attacker is an individual or an organized group engaged in laundering illicit funds on the blockchain. Typical examples include hacking groups, fraud syndicates, ransomware operators, and other actors involved in major financial crimes. These attackers share a common characteristic: they obtain large amounts of illegal funds and exploit blockchain ecosystems to conceal the origins and destinations of the funds, ultimately integrating them into the legitimate financial system~\cite{lin2024denseflow}. As part \circlednum{2} of Figure~\ref{fig:threat} shows, we assume the attacker possesses the following capabilities: (1) Control of large-scale addresses. Attackers can create and operate an unlimited number of blockchain addresses at negligible cost, enabling them to evade fixed blacklist detection; (2) Use of fund obfuscation tools~\cite{wu2023towards}. Attackers are proficient in employing DEXs for token swaps and indirect transfers, leveraging cross-chain bridges to move funds across different blockchains, and performing self-mixing through multi-address splitting and recombination of funds to obscure transaction flows; (3) Automation transaction execution. Attackers can use scripts or bots to perform large-scale, multi-hop, and high-frequency fund transfers. \sout{Also, we assume the attacker has certain limitations: they cannot modify and delete transaction data on the blockchain, they do not utilize privacy coins~\cite{scharnowski2024dark} (e.g., Monero, Zcash) or specialized mixing services~\cite{299657} (e.g., Tornado Cash).}

\heading{Victim profile.}~~ As the part \circlednum{1} of Figure~\ref{fig:threat} shows, the victims are the original legitimate owners of the funds involved in Crypto ML incidents. The victims may be individual users or service platforms, such as centralized exchanges, DeFi protocols~\cite{qin21defi}. For example, an attacker may compromise a cryptocurrency exchange’s system and transfer large sums from the exchange’s wallet address to addresses under their control. It is hard for these victims to prevent such attacks and to track transactions on the blockchain, and they do not collaborate with the attacker’s laundering activities.

\heading{Defender capabilities.}
Defenders are AML detection and forensics systems (e.g., ours). Their objective is to identify and report suspicious ML transactions during the layering stage of Crypto ML, before the illicit funds are integrated into the legitimate financial system. As the part \circlednum{4} to \circlednum{6} of Figure~\ref{fig:threat}  shows, the defender’s capabilities include: (1) acquiring Blockchain transaction data because of blockchain transparency; (2) detecting ML transactions by rules, graph analysis, and artificial intelligence techniques; (3) generating SARs to relevant authorities for further investigation and intervention. \sout{However, the defenders cannot access off-chain identity information, have difficulty monitoring privacy coins, specialized mixing services, and lack direct enforcement power or the authority to freeze assets, relying on authorized agencies to take such actions.} Defenders primarily focus on tracking funds in account-based blockchains, since the vast majority of victims currently operate on such chains~\cite{chainalysis25}. When funds are transferred across chains from an account-based blockchain to a UTXO-based blockchain, defenders can still identify the target chain and the corresponding receiving address. \sout{However, they are not able to further trace the subsequent fund flows within the UTXO-based blockchain.}



% \subsection{Threat Model}


% \textbf{Protection Scenario.} In the scenario we assume, as shown in Figure~\ref{fig:threat}, there are three parties involved: victims, attackers, and the defender. (\textit{i}) \textbf{Victims} are blockchain investors and on-chain infrastructures, including fund-holding investors and financial infrastructures operating on the blockchain, such as centralized exchanges, decentralized finance protocols, and cross-chain bridges. In the blockchain network, these parties typically interact with others through one or more on-chain addresses, which may become compromised or defrauded; (\textit{ii}) \textbf{Attackers} are money laundering groups who quickly transfer and conceal them once the funds are stolen by them. They often control a large number of blockchain addresses and employ complex transaction patterns (such as multi-path fund splitting, and amount structuring) combined with various money laundering techniques, including token swaps, cross-chain transfers, and indirect transactions, to obscure the fund trail and evade tracing; (\textit{iii}) The \textbf{Defender} is the protection service provider(such as \techName{}), responsible for monitoring blockchain transactions, detecting potentially suspicious transactions and corresponding fund flows, and generating Suspicious Activity Reports (SARs) to facilitate regulatory review and investigation.
% %为什么被hacked或者defrauded需要说嘛


% %感觉现在system goal写的像介绍方法。
% \textbf{System Goal.} \techName{} aims to assist blockchain investors and on-chain financial infrastructures in safeguarding their assets and transaction security, responding to sophisticated money laundering activities, and generating SARs for compliance review and asset tracing. Its primary objective is to efficiently and accurately detect and explain suspicious laundering activities in large-scale blockchain networks. To achieve this, the system performs a comprehensive analysis of both the structural and semantic characteristics of transactions to enhance its ability to identify diverse laundering patterns. Based on the detection results, it produces SARs that include fund flow visualizations, summaries, and red flags, thereby supporting compliance teams in conducting in-depth analysis, tracing illicit funds, and making informed decisions.


% \textbf{Knowledge Assumption.} In our assumed scenario, the protection service provider has access to publicly available on-chain data, including blockchain transaction records, event templates for certain cross-chain bridges, and a small set of verified money laundering labels. However, the system cannot obtain off-chain identity information (e.g., KYC data). In addition, we assume that money laundering groups do not use privacy coins~\cite{harvey2020cryptocurrencies} (e.g., Monero, Zcash) for fund transfers, ensuring that their on-chain transactions remain traceable and analyzable in blockchain networks.


% \subsection{Problem Statement}



==> chapter/3-threat-model.tex <==


%All papers submitted should provide a threat model that clearly articulates the (i) envisioned attacker(s), (ii) threat surfaces (e.g., system components including but not limited to the underlying machine learning algorithm), (iii) generality and (iv) practicality of the attack.





\section{Threat Model} \label{sec:threat}


We consider a Crypto AML system composed of two core components: a \textit{detector}~$\mathcal{D}$ and an \textit{explainer}~$\mathcal{E}$.  

\begin{packeditemize}
    \item The \textit{detector} $\mathcal{D}$ has access to all public blockchain transactions $tx \in \mathcal{T}$ and determines whether each transaction is associated with money laundering. Formally,
\[
\mathcal{D}: \mathcal{T} \rightarrow \{0,1\}, \quad 
\mathcal{D}(tx) =
  \begin{cases}
    1, & \text{if } tx ~\text{is laundering,} \\
    0, & \text{otherwise.}
  \end{cases}
\]
    \item The \textit{explainer} $\mathcal{E}$ produces structured SARs for detected laundering transactions.  
\end{packeditemize}





When a set of laundering transactions forms a connected subgraph in the fund–flow graph, which we denote as a \textit{laundering flow} $L \subseteq \mathcal{T}$, the explainer can be modeled as:
\[
\mathcal{E}: \mathcal{L} \rightarrow \mathcal{R},
\]
where $\mathcal{L}$ is the set of laundering flows and $\mathcal{R}$ is the space of structured reports, each report $r \in \mathcal{R}$ consisting of a \textit{FlowDiagram}, \textit{Summary}, and \textit{RedFlags}.


\smallskip
\noindent\textbf{Adversary.}  
A launderer controls multiple blockchain addresses and strategically crafts transactions to obscure the provenance and destination of illicit funds.  

Such adversarial behaviors undermine AML systems in the following ways:

\begin{packeditemize}
  \item \textit{Contract-level camouflage:} embedding token swaps or internal transfers within a single transaction to conceal actual asset movement.
  \item \textit{Cross-chain laundering:} routing assets through bridges to other blockchains, breaking the continuity of fund tracing.
  \item \textit{Automated laundering:} employing bots to execute repetitive transactions at scale, diluting anomaly signals.
  \item \textit{Coordinated strategies:} combining multiple laundering techniques (e.g., swaps, dispersal, bridges) to form multi-chain, structurally complex laundering flows.
\end{packeditemize}

\smallskip
\noindent\textbf{Assumptions.}  
The detector and explainer operate solely on publicly observable on-chain data (e.g., transaction metadata and event logs) without relying on private data (e.g., exchange records, off-chain KYC information, heuristic blacklists). These assumptions align with real-world constraints in decentralized ecosystems.



\heading{Objective.}  
Given the above threat model, we aim to design a unified framework that bridges semantic-level behavioral inference and structural-level fund-flow analysis.  
This integration allows the detector–explainer pipeline to reason holistically about laundering behaviors, revealing hidden transactional intents, reconstructing cross-chain propagation, and delivering interpretable, regulator-oriented outputs.








%reference: https://www.usenix.org/system/files/usenixsecurity24-teoh.pdf

%1 形式化描述问题和任务
% 我们假设存在一个洗钱检测器，它可以访问公共区块链上的交易数据用于执行洗钱检测分析。检测器可被形式化建模为一个函数D:T-{0,1}。进一步，假设存在一个洗钱解释器，它可以访问D检测出来的洗钱交易，用于生成结构化的SAR。当若干洗钱交易构成一个连通子图，我们称为洗钱流。解释器 将每个洗钱流 映射为一个结构化报告。

%Assume that there is a Crypto ML\textbf{detector $\mathcal{D}$}, which has access to every public blockchain transaction $tx \in \mathcal{T}$ for laundering analysis. The detector $\mathcal{D}$ can be modelled as a function $\mathcal{D}(.): \mathcal{T} \rightarrow \{0,1\}$ where $\mathcal{T}$ is the set of transactions.  $\mathcal{D}(tx)=1$ indicates that transaction $tx$ is identified as \textit{money laundering}, and $D(tx)=0$ denotes \textit{non-laundering} behavior.  Furthermore, we assume that there is a Crypto ML \textbf{explainer $\mathcal{E}$}, which can generate structured SARs for detected money laundering transactions. 
%When a set of money laundering transactions forms a connected subgraph in the fund-flow graph, referred to as a laundering flow $L \subseteq \mathcal{T}$. The explainer $\mathcal{E}$ can be modelled as a function  $\mathcal{E}(.): \mathcal{L} \rightarrow \mathcal{R}$ where $\mathcal{L}$ is the set of laundering flows and $\mathcal{R}$ represents the space of structured reports. Each structured report $r \in \mathcal{R} = (\text{FlowDiagram},\; \text{Summary},\; \text{RedFlags})$.



%一个洗钱者在控制区块链地址之下，会制造很多洗钱交易。这些洗钱交易会被洗钱者的洗钱策略伪装成普通交易并且掩盖资金流向，compromise传统的detector in the following manners：
% Laundering with 合约层级伪装. 通过调用复杂合约洗钱者能在单笔可见交易中完成多步内部转账或者代币交换，掩盖真实的发送接收关系。
% Laundering to another blockchain. 利用跨链桥把资产转移到另一条链上，打断单链视角下的资金流连续性。
% Laundering by automation: 使用交易机器人批量并行执行相似交易以放大规模与速度
% Laundering with coordinated Strategies: 组合使用洗钱策略。

\begin{comment}

A launderer controls multiple blockchain addresses and initiates a large number of transactions that are deliberately disguised to conceal the true flow of illicit funds. Such behaviors can compromise the effectiveness of traditional detectors in several ways:
\begin{packeditemize}
    \item \textbf{Laundering with contract-level Camouflage.} Utilizing smart contracts to perform internal transfers or token swaps within a single visible transaction.
    \item \textbf{Laundering to another blockchain.}  Leveraging cross-chain bridges to transfer assets to another blockchain, breaking the continuity of fund tracing.
    \item \textbf{Laundering by automation.} Employing trading bots to execute similar transactions, increasing scale and diluting anomaly signals.
    \item \textbf{Coordinated laundering strategies.} Combining laundering techniques to construct cross-chain and structurally complex laundering flows.
\end{packeditemize}

    
\end{comment}

%鉴于上述威胁模型，我们采用交易语义与资金流双视角的检测思路：一方面解析交易语义以揭示隐藏意图，另一方面重建资金流关系以恢复真实流向，从而提升对复杂洗钱行为的识别与解释能力。

%Given the above threat model, we adopt a dual perspective of transaction semantics and fund-flow analysis to jointly capture hidden intents and true asset movements, improving detection and explainability of complex laundering behaviors.

%我写的怎么感觉都差点意思 
%Qin:我感觉写的挺好了 只是润了润语言 逻辑都在
 



 

%Figure~\ref{fig:threat} illustrates the overall threat model Crypto ML, highlighting the attack process and the corresponding defense process of AML detection and forensics. In the following, we detail the threat scenario, the attacker’s capabilities, the victim profile, and the defender’s capabilities.


% \heading{Threat scenario.}
% In a typical cryptocurrency money laundering incident, as the part \circlednum{1} to \circlednum{3} of Figure~\ref{fig:threat}  shows, the attacker first acquires illicit funds from the victim through hacking, fraud, ransomware attacks, and so on. Once these funds are transferred to addresses under the attacker’s control on the blockchain, the attacker employs various techniques to launder the funds. Following the incident, as the part \circlednum{4} to \circlednum{6} of Figure~\ref{fig:threat} shows, defenders attempt to identify suspicious laundering transactions and trace the associated fund flows from transaction data on the blockchain. Defenders then generate SARs to support AML compliance teams and law enforcement agencies~\cite{FAFT} in taking timely actions, such as freezing the detected funds to prevent further transfers or cash-outs.


% \heading{Threat scenario.} 
% In a typical cryptocurrency money laundering incident,  the attacker first acquires illicit funds from victims through financial crimes, and transfers these funds to addresses under their control on the blockchain. The attacker then employs various laundering techniques to obscure the origin and destination of the funds. Following the incident, defenders attempt to identify suspicious laundering transactions and trace fund flows. The detected cases are visualized as fund flow graphs and summarized as SARs to assist AML compliance teams and law enforcement~\cite{FAFT} in freezing or recovering illicit funds.


% \heading{Attacker capabilities.} The envisioned attacker is an individual or an organized group engaged in laundering illicit funds on the blockchain. These attackers share a common characteristic: they obtain illegal funds and exploit blockchain ecosystems to conceal the origins and destinations of the funds~\cite{lin2024denseflow}. As part \circlednum{2} of Figure~\ref{fig:threat} shows, we assume the attacker possesses the following capabilities:

% \begin{packeditemize}

% \item \textbf{Address control and automated transactions.} Attackers can create and operate an unlimited number of blockchain addresses and execute automated transactions via transaction bots~\cite{Automated}, which enables multi-layered and complex fund flows that increase tracing difficulty.

% \item \textbf{Diverse crypto ML techniques.} Attackers employ various laundering techniques, which are mentioned in the Introduction section (e.g., fund dispersal, token swaps, cross-chain transfers, and indirect transfers), composing them in staged ways to conceal fund origins, break trace continuity, and evade detection.


% \end{packeditemize}


% \heading{Victim profile.} As the part \circlednum{1} of Figure~\ref{fig:threat} shows, the victims are the original legitimate owners of the funds involved in Crypto ML incidents. The victims may be individual users or service platforms, such as centralized exchanges, DeFi protocols~\cite{qin21defi}. For example, an attacker may compromise a cryptocurrency exchange’s system and transfer large sums from the exchange’s wallet address to addresses under their control. It is hard for these victims to prevent such attacks and to track transactions on the blockchain, and they do not collaborate with the attacker’s laundering activities.

% \heading{Defender capabilities.}
% Defenders are AML detection and forensics systems (e.g., our \techName{}). Their objective is to identify and report suspicious ML transactions. The defender’s capabilities include: 

% \begin{packeditemize}

% \item \textbf{Blockchain data acquisition.} Owing to the transparency of the blockchain, defenders can collect on-chain data, including transaction records, smart contract calls, and event logs.

% \item \textbf{Suspicious transaction detection.} Defenders can detect ML transactions by rules, graph analysis, and artificial intelligence techniques.

% \item \textbf{Suspicious activity reporting.}  Once suspicious ML transactions are detected, defenders generate SARs to relevant authorities for further investigation and intervention. 



% \end{packeditemize}



% \begin{figure}[th]
% \begin{center}
% \includegraphics[width=0.5\textwidth]{Figs/threat model num.pdf}
% \end{center}
% \caption{\label{fig:threat} Crypto ML and its Threat model.}
% \end{figure}


% \subsection{Threat Model}


% \textbf{Protection Scenario.} In the scenario we assume, as shown in Figure~\ref{fig:threat}, there are three parties involved: victims, attackers, and the defender. (\textit{i}) \textbf{Victims} are blockchain investors and on-chain infrastructures, including fund-holding investors and financial infrastructures operating on the blockchain, such as centralized exchanges, decentralized finance protocols, and cross-chain bridges. In the blockchain network, these parties typically interact with others through one or more on-chain addresses, which may become compromised or defrauded; (\textit{ii}) \textbf{Attackers} are money laundering groups who quickly transfer and conceal them once the funds are stolen by them. They often control a large number of blockchain addresses and employ complex transaction patterns (such as multi-path fund splitting, and amount structuring) combined with various money laundering techniques, including token swaps, cross-chain transfers, and indirect transactions, to obscure the fund trail and evade tracing; (\textit{iii}) The \textbf{Defender} is the protection service provider(such as \techName{}), responsible for monitoring blockchain transactions, detecting potentially suspicious transactions and corresponding fund flows, and generating Suspicious Activity Reports (SARs) to facilitate regulatory review and investigation.
% %为什么被hacked或者defrauded需要说嘛


% %感觉现在system goal写的像介绍方法。
% \textbf{System Goal.} \techName{} aims to assist blockchain investors and on-chain financial infrastructures in safeguarding their assets and transaction security, responding to sophisticated money laundering activities, and generating SARs for compliance review and asset tracing. Its primary objective is to efficiently and accurately detect and explain suspicious laundering activities in large-scale blockchain networks. To achieve this, the system performs a comprehensive analysis of both the structural and semantic characteristics of transactions to enhance its ability to identify diverse laundering patterns. Based on the detection results, it produces SARs that include fund flow visualizations, summaries, and red flags, thereby supporting compliance teams in conducting in-depth analysis, tracing illicit funds, and making informed decisions.


% \textbf{Knowledge Assumption.} In our assumed scenario, the protection service provider has access to publicly available on-chain data, including blockchain transaction records, event templates for certain cross-chain bridges, and a small set of verified money laundering labels. However, the system cannot obtain off-chain identity information (e.g., KYC data). In addition, we assume that money laundering groups do not use privacy coins~\cite{harvey2020cryptocurrencies} (e.g., Monero, Zcash) for fund transfers, ensuring that their on-chain transactions remain traceable and analyzable in blockchain networks.


% \subsection{Problem Statement}



==> chapter/4-1-overview.tex <==
\subsection{Architecture Overview}
\label{subsec-archi}

\begin{figure*}[h]
\begin{center}
% \includegraphics[width=0.97\textwidth]{Figs/framework.png}
\includegraphics[width=0.97\textwidth]{Figs/framework_new.pdf}
\end{center}
\caption{\label{fig:framework} Overview of \techName{}.}
\end{figure*}


% \techName{} serves as a Crypto AML framework designed to enhance the detection performance of complex money laundering transactions while providing explainable results. As illustrated in Figure~\ref{fig:framework}, the overall process for \techName{} involves four phases: \circlednum{1} semantic awareness; \circlednum{2} graph construction; \circlednum{3} semantics-structure fusion; and \circlednum{4} SAR generation.

% \textbf{Phase \circlednum{1}: Semantic Awareness.} In the first phase, \techName{} performs semantic awareness for each transaction, aiming to extract its underlying behavioral intent from raw blockchain data. The goal of this phase is to generate high-level semantic information that reflects the behaviors of transactions. To this end, \techName{} defines four common transaction semantics: direct transfers, indirect transfers, cross-chain transfers and token swaps, and designs parsing strategies for each. Specifically, direct transfers are identified by detecting simple transfers; indirect transfers are detected by comparing multiple records under the same transaction hash to trace intermediate fund movements; cross-chain interactions are parsed by matching contract addresses and analyzing on-chain event data to extract the target chain and receiving address; and token swaps are recognized by analyzing the types of tokens and the in-out flow within the same transactions hash. Finally, \techName{} generates both semantic labels and structured semantic text for each transaction. These semantic representations serve as input to language models and provide support for structure-semantics fusion and SAR generation.


% \textbf{Phase \circlednum{2}: Graph Construction.} To capture the flow of funds between transactions, in the second phase, \techName{} constructs a multi-directed graph (MultiDiGraph)~\cite{Dan20Model} from raw transaction data, where each node represents an address and each edge corresponds to a transaction, along with its detailed attributes. This graph forms a foundation for structural representation. However, building a graph solely based on address-level transaction links is insufficient to reveal how funds actually move between individual transactions, nor can it fully capture complex money laundering patterns such as layering, and integration. To address the limitation, \techName{} further constructs upstream, downstream, and parallel transaction subgraphs on top of the basic transaction graph for each transaction. These subgraphs offer essential structural information (such as fund sources, destinations, and flow paths) that helps uncover sophisticated laundering patterns and generate SARs.

% \textbf{Phase \circlednum{3}: Semantics-structure Fusion.} After semantic awareness and graph construction, \techName{} enters the third phase: structure-semantic fusion. The goal of this phase is to integrate the transaction's graph-based structural information with its behavior-level semantics, enabling a more comprehensive representation of each transaction and thereby improving the accuracy of money laundering detection. Specifically, \techName{} encodes each transaction's semantic-aware descriptions, including the transaction intent text and fund flow description generated in the previous two phases, using a fine-tuned large language model. In parallel, Graph Convolutional Networks (GCNs) are trained to extract structural embeddings based on the transaction graph. To capture the interaction between structural and semantic views, \techName{} applies a structure-semantic cross-attention mechanism to fuse both types of embeddings. The resulting joint representation preserves both the neighborhood-aware structural patterns and the behavior-driven semantic intent, enabling deep modeling of complex laundering activities. 

% \textbf{Phase \circlednum{4}: SAR Generation.} In the final phase, \techName{} first leverages the fused representations from the previous stages to identify suspicious money laundering transactions using a Multi-Layer Perceptron (MLP) classifier. Then, \techName{} incorporates each transaction semantics and its flow of fund to prompt a large language model to generate a SAR for suspicious money laundering transactions. The final output includes: a visualized money laundering flow subgraph; a summary description of the laundering path; and red flags indicating the suspicious money laundering transaction. By introducing the explanation generation mechanism, \techName{} establishes a AML framework from structural and semantic understanding to human-readable explanation, thereby enhancing the explainability and regulatory usability of detection results.




% \techName{} is a Crypto AML framework designed to improve the detection of complex money laundering activities while providing explainable outputs. As shown in Figure~\ref{fig:framework}, the framework operates in four phases. Phase \circlednum{1} (\emph{Semantic Awareness}) extracts high-level behavioral semantics from raw blockchain transactions, capturing intents such as direct/indirect transfers, token swaps, and cross-chain transfers. Phase \circlednum{2} (\emph{Graph Construction}) models transaction relationships as a multi-directed graph and derives upstream, downstream, and parallel subgraphs to reveal fund flows. Phase \circlednum{3} (\emph{Semantics–Structure Fusion}) integrates semantic and structural representations through joint embedding to provide a richer description of each transaction. Phase \circlednum{4} (\emph{SAR Generation}) detects suspicious transactions and produces investigator-friendly reports, including flow visualizations, path summaries, and red flags, enhancing both explainability and regulatory usability.



\techName{} aims to improve the detection of complex money laundering activities while providing explainable outputs. As illustrated in Figure~\ref{fig:framework}, it operates in four phases. 

\begin{packeditemize}

\item Phase-\circlednum{1} (\emph{semantic awareness}) provides transaction-level semantic understanding by extracting high-level behavioral intents from transaction data. It can identify direct/indirect transfers, token swaps, and cross chain transfers.  

\item Phase-\circlednum{2} (\emph{fund flow awareness}) model transactions as a multi-directed graph and derives upstream, downstream, and parallel subgraphs to reveal fund flows. It overcomes the limitation of address-centric transaction graphs.

\item Phase-\circlednum{3} (\emph{semantics–structure fusion}) integrates both views through fused embedding and yields a richer transaction representation. It bridges the gap between semantic and structural modeling.

\item Phase-\circlednum{4} (\emph{SAR generation}) detects suspicious transactions and generates reports with flow visualisations, path summaries, and red flags. It provides explainable outputs.

\end{packeditemize}


==> chapter/4-2-semantic-awareness.tex <==
\subsection{(Phase-\circlednum{1}) Semantic Awareness}
\label{subsec-semantic}

In this phase, \techName{} performs semantic awareness for each transaction to extract underlying behavioral intent from raw blockchain data.  

We define the set of transactions as 
$$\mathcal{T} = \{ \text{TX}_{h_1}, \text{TX}_{h_2}, \dots, \text{TX}_{h_n} \},$$
\textit{where the element $\mathrm{TX}_{h_i}$ represents the group of transactions sharing the same transaction hash $h_i$.} For each element, we formally define

$$\text{TX}_{h_i} = \{ \text{\text{tx}}_{h_i}^1, \text{\text{tx}}_{h_i}^2, \dots, \text{\text{tx}}_{h_i}^{m_i} \},$$ \textit{where $m_i$ denotes the number of constituent transactions under hash $h_i$.}
Each transaction is represented as:
$$\text{\text{tx}}_{h_i}^j = (\text{h}_i, \text{from}_j, \text{to}_j, \text{time}_j,\text{token}_j, \text{amount}_j, \text{gasfee}_j, \text{log}_j),$$ 
\textit{where $\text{from}_j$ and  $\text{to}_j$ denote the sender and receiver address, $\text{time}_j$ is the timestamp, $\text{token}_j$ specifies the token name, $\text{amount}_j$ the transferred value, $\text{gasfee}_j$ is the transaction fee, and $\text{log}_j$ represents event logs. }

We further define the set of transaction semantics as
$$\mathcal{S} =\{\text{T}_{dir},\text{T}_{ind},\text{T}_{swp},\text{T}_{crs}\}, $$
\textit{where $\text{T}_{dir},\text{T}_{ind},\text{T}_{swp}$, and $\text{T}_{crs}$  refer to direct transfer, indirect transfer, token swap, and cross-chain transfer}. 


A mapping function $f_{\mathrm{sem}}:\text{\text{tx}}_{h_i}^j \rightarrow \mathcal{S}$ assigns each transaction to one semantic type based on its behavioral pattern.
For each semantic type $\text{T}_s \in \mathcal{S}$, 
we define a parsing rule $\mathcal{R}_x(\text{\text{tx}}_{h_i}^j)$ 
that evaluates to \textsf{true} if the transaction $\text{\text{tx}}_{h_i}^j$ 
satisfies the conditions of $\text{T}_s$, and \textsf{false} otherwise. 
The semantic mapping function $f_{\mathrm{sem}}$ then assigns 
the transaction $\text{\text{tx}}_{h_i}^j$ to the unique $\text{T}_s$ whose 
$\mathcal{R}_x(\text{\text{tx}}_{h_i}^j)$ is satisfied.

\heading{Defining transaction semantics.} Then, we define aforementioned four transaction semantics with parsing rules.



\begin{packeditemize}


\smallskip
\item\underline{\textit{Direct transfer}} ($\text{T}_{dir}$). 
If a transaction does not satisfy the conditions of token swap, indirect transfer, or cross-chain transfer, it is classified as a \emph{direct transfer}.  
Formally,
\[
\mathcal{R}_{dir}(\text{tx}_{h_i}^j) : 
\neg\mathcal{R}_{swp}(\text{tx}_{h_i}^j) \ \land\ 
\neg\mathcal{R}_{ind}(\text{tx}_{h_i}^j) \ \land\ 
\neg\mathcal{R}_{crs}(\text{tx}_{h_i}^j).
\]
If $\mathcal{R}_{dir}(\text{tx}_{h_i}^j)$ holds, then the semantic mapping function assigns $\text{f}_{sem}(\text{tx}_{h_i}^j) = \text{T}_{dir}$.

\item\underline{\textit{Token swap}} ($\text{T}_{swp}$). In a transaction group\footnote{A \textit{transaction group} refers to a set of internal transactions that share the same transaction hash and are executed atomically within a single Ethereum transaction. 
Each group may contain multiple internal transfers triggered by smart contract calls (e.g., token swaps, liquidity operations, or multi-hop settlements), all finalized under one outer transaction hash.} sharing the same transaction hash, if the sender of one transaction also appears as the receiver in another transaction within the same group, and the two transactions involve different tokens, the semantic type is classified as a \emph{token swap}. Formally, we define
\[
\mathcal{R}_{swp}(\text{tx}_{h_i}^j) : \exists\, \text{tx}_{h_i}^x \in \mathcal{I}(\text{tx}_{h_i}^j) \ \text{s.t.} \ \text{token}_x \neq \text{token}_j,
\]
\textit{where $\mathcal{I}(\text{tx}_{h_i}^j) = \{\, \text{tx}_{h_i}^x \in \text{TX}_{h_i} \setminus \{ \text{tx}_{h_i}^j \} \mid \text{to}_x = \text{from}_j \,\}$ denotes the set of ingoing transactions of the sender within the group.} 
If $\mathcal{R}_{swp}(\text{tx}_{h_i}^j)$ holds, then the semantic mapping function assigns $\text{f}_{sem}(\text{tx}_{h_i}^j) = \text{T}_{swp}$.




\smallskip
\item\underline{\textit{Cross-chain transfer}} ($\text{T}_{crs}$).  If the receiver of a transaction is a cross-chain bridge contract address, and the transaction log contains identifiable information about the destination blockchain and recipient address, the semantic type is classified as a \emph{cross-chain transfer}.  
Formally,  
\[
\mathcal{R}_{crs}(\text{tx}_{h_i}^j) : (\text{to}_j \in \mathcal{A}_{bridge}) \ \land\ \text{parse}(\text{log}_j),
\]
\textit{where $\mathcal{A}_{bridge}$ denotes the set of cross-chain bridge contract addresses\footnote{The set of addresses can be obtained and updated from the official documentation of cross-chain bridges.}, and $\text{parse}(\text{log}_j)$ represents a parsing function that extracts relevant fields (e.g., destination chain and destination address) from the transaction logs.} If $\mathcal{R}_{crs}(\text{tx}_{h_i}^j)$ holds, then the semantic mapping function assigns $\text{f}_{sem}(\text{tx}_{h_i}^j) = \text{T}_{crs}$.



\smallskip
\item\underline{\textit{Indirect transfer}} ($\text{T}_{ind}$).
Within a transaction group sharing the same transaction hash, if the receiver of one transaction also acts as the sender in another transaction of the same group, and both transactions involve the same token, the semantic type is classified as an \emph{indirect transfer}.  
Formally,
\[
\mathcal{R}_{ind}(\text{tx}_{h_i}^j) : \exists\, \text{tx}_{h_i}^y \in \mathcal{O}(\text{tx}_{h_i}^j) \ \text{s.t.} \ \text{token}_y = \text{token}_j,
\]
\textit{where $ \mathcal{O}(\text{tx}_{h_i}^j) = \{\, \text{tx}_{h_i}^y \in \text{TX}_{h_i} \setminus \{ \text{tx}_{h_i}^j \} \mid \text{from}_y = \text{to}_j \,\} $
denotes the set of outgoing transactions of the receiver within the group.}  
If $\mathcal{R}_{ind}(\text{tx}_{h_i}^j)$ holds, then the semantic mapping function assigns $\text{f}_{sem}(\text{tx}_{h_i}^j) = \text{T}_{ind}$.




\end{packeditemize}

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.47\textwidth]{Figs/semantics_line_str.pdf}
\end{center}
\caption{\label{fig:tmp} Semantics template text.}
\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.38\textwidth]{Figs/example_semantics.pdf}
\end{center}
% \caption{\label{fig:exa} Example of a real transaction 
% (\textcolor{black}{\text{0x6c10}}). The red transaction is the target transaction to be analyzed, and the green transaction is its incoming transaction.\qw{change with example meaning} }
\caption{\label{fig:exa} Example of token swap transaction parsing: {0xa4b2} swap stETH to ETH.}
\end{figure}


\smallskip
After assigning a semantics type to each transaction, we generate a semantics text to describe its behavioral intent. For each semantic type, we apply a fixed template to populate key fields (e.g., transaction hash, sender, receiver, amount, token, contract, time, gas fee, and other type-specific attributes) from the transaction. Figure~\ref{fig:tmp} illustrates these templates, where placeholders (e.g., {{$\text{amount}_j$}}, {{$\text{token}_j$}}) are substituted with the content of each transaction. Algorithm~\ref{alg:semantics} further summarizes the procedure.


\heading{Runing examples.}  Figure~\ref{fig:exa} shows an example of semantics awareness of a real transaction. We focus on $\text{tx}_{\text{0x6c10}}^{1}$, where address \hlhref{https://etherscan.io/address/0xA4B2Fd68593B6F34E51cB9eDB66E71c1B4Ab449e}{{0xa4b2}} transfers 4,000 stETH to \hlhref{https://etherscan.io/address/0x6BB000067005450704003100632eB93ea00c0000}{{0x6bb0}}.
This transaction belongs to a transaction group sharing the same hash (\hlhref{https://etherscan.io/tx/0x6c108f99a7d1f2a627a5b6a6a1984d054d5dc17f7bcc423bcc926c7d69f766f6}{{0x6c10}}), consisting of 12 transactions in total.


 
Following Algorithm~\ref{alg:semantics}, we inspect the incoming transactions $\mathcal{I}(\text{tx}_{0x6c10}^1)$ of the sender \hlhref{https://etherscan.io/address/0xA4B2Fd68593B6F34E51cB9eDB66E71c1B4Ab449e}{{0xa4b2}} within the same group and identify $\text{tx}_{0x6c10}^{10}$, where address \hlhref{https://etherscan.io/address/0x0000000000bbF5c5Fd284e657F01Bd000933C96D}{0x0000} transfers 3,970 ETH to \hlhref{https://etherscan.io/address/0xA4B2Fd68593B6F34E51cB9eDB66E71c1B4Ab449e}{{0xa4b2}}.
This satisfies $\mathcal{R}_{swp}$, indicating that $\text{f}_{sem}(\text{tx}_{0x6c10}^1) = \text{T}_{swp}$.
Finally, using the token-swap template illustrated in Figure~\ref{fig:tmp}, \techName{} generates the corresponding semantic description text:

% \begin{quote}
% \footnotesize
% {Token Swap: In transaction 0x6c10, account 0xa4b2 used account 0x6bb0 to swap 4000 stETH into 3970 ETH at time 2025-02-21 15:27:47, with gas fee 1.7e-3 ETH.}
% \end{quote}

% \vspace{-0.1in}
\begin{center}
  % \fbox{
\colorbox{blue!9}{
\begin{minipage}{0.95\linewidth}
  (\textit{Token swap}) In transaction \hlhref{https://etherscan.io/tx/0x6c108f99a7d1f2a627a5b6a6a1984d054d5dc17f7bcc423bcc926c7d69f766f6}{{0x6c10}}, address \hlhref{https://etherscan.io/address/0xA4B2Fd68593B6F34E51cB9eDB66E71c1B4Ab449e}{{0xa4b2}} used address \hlhref{https://etherscan.io/address/0x6BB000067005450704003100632eB93ea00c0000}{{0x6bb0}} to swap 4,000 stETH into 3,970 ETH at time 2025-02-21 15:27:47, with gas fee 1.7e-3 ETH.
\end{minipage}
      }
 %  }
\end{center}


%准备感知语义的交易是0xa4b2-->0x6bb0 4000stETH（可以在图上画交易编号），该交易所在的交易群有11条交易，0x00c6-->0x21e2 560stETH;0x00c6-->0xdc24 3440stETH; 0x6bb0-->0x00c6 4000stETH; 0xa4b2-->0x6bb0 4000stETH; 0x21e2-->0xcc60 558ETH;0xcc60-->0x6a00 3988ETH; 0x6a00-->0x6bb0 3988ETH;0x6b00-->0x0000 3988ETH;0x0000-->0xa4b2 3970ETH;0x2e5e-->0x0000 0ETH（这些交易信息只用在图中体现）。根据算法一的流程，,该交易的sender的incoming transactions中存在一条交易0x0000-->0xa4b2 3970ETH，可以判断出该交易符合 Rswp。然后用图二的模板以及该交易的信息生成该交易的semantics text.

% \input{Alg/semantics_alg}



%\qs{comment about direct and fund dispersal}
% 对了，我之前在Intro定义成Fund dispersal手法，但其实这里是描述direct transfer, 会不会有点矛盾? 周四可以讨论下 -- 好！

==> chapter/4-3-graph-construction.tex <==
\subsection{(Phase-\circlednum{2}) Fund Flow Awareness}
\label{fund_flow_aware}

After identifying transaction intent, the second phase models transaction relationships as a graph to capture how funds move structurally.
To this end, we first represent the entire transaction network as a multi-directed graph (MultiDiGraph)~\cite{Dan20Model}, and then construct \textit{upstream}, \textit{downstream}, and \textit{parallel} subgraphs for each transaction to capture sources, destinations, and concurrent fund flows.

Formally, the transaction network is defined as a MultiDiGraph $G=(V,E,X,A)$, where $V$ denotes the set of blockchain addresses, and $E$ represents the set of directed transaction edges. Each edge $e \in E$ is described as
$e=\{from,to,amount,token,time,\text{T}_s\}$,
where $from$ and $to$ denote the sender and receiver addresses, $amount$ is the transferred value, $token$ the token name, $time$ the transaction timestamp, and $\text{T}s$ the semantic type identified in the semantic-awareness phase.
The node feature matrix $X$ records the number of transactions associated with each address, while the adjacency matrix $A$ captures the network topology, where $A{ij}$ indicates the number of transactions from node $i$ to node $j$.

While the MultiDiGraph $G$ captures all transaction relationships, it is too large and contains many irrelevant edges for analyzing a specific transaction. To provide a localized structural view of its fund flow, we derive the following three types of transaction subgraphs. Each subgraph reveals different aspects of the transaction’s fund movement.



\begin{packeditemize}
    
\item \underline{\textit{Upstream subgraph}} ($SubG_{up}$) characterizes the funding path of a target transaction $e_{tg}$, representing the set of transactions and addresses that transfer relevant funds to the sender of $e_{tg}$ prior to $e_{tg}$. To construct $SubG_{up}$, \techName{} combines transaction time, semantics type, and token names to identify potential funding sources as upstream transaction candidates. 

Specifically, among all transactions that occurred within the time window threshold $\tau_t$ before $e_{tg}$, we retain those whose actual receiver equals the sender of $e_{tg}$ and whose token matches that of $e_{tg}$.
If an upstream transaction corresponds to an indirect or cross-chain transfer, its actual receiver must be the sender of $e_{tg}$; if it represents a token swap, the output token must match that of $e_{tg}$. After collecting all candidates, the transactions are time-ordered, and their transferred amounts are accumulated until the cumulative value reaches the flow ratio threshold $\tau_f$ of the amount in $e_{tg}$. Finally, the selected upstream transactions, together with $e_{tg}$, form $SubG_{up}$.

% time window 
% $\tau_t$, flow ratio $\tau_f$, and amount similarity $\tau_a$

\smallskip
\item \underline{\textit{Downstream subgraph}} ($SubG_{down}$) characterizes the fund outflow path of a target transaction $e_{tg}$. To construct $SubG_{down}$, \techName{} starts from the receiver address of $e_{tg}$ and retrieves all outgoing transactions that occur within $\tau_t$ after $e_{tg}$ and involve the same token name as $e_{tg}$.  From these transactions, \techName{} selects the earliest batch of outgoing transactions whose cumulative amount accounts for at least $\tau_f$ of the amount of $e_{tg}$. Finally, these downstream transactions, together with $e_{tg}$, form the downstream subgraph.

\smallskip
\item \underline{\textit{Parallel subgraph}} ($SubG_{para}$) captures fund flows that occur in parallel with a target transaction $e_{tg}$. To construct $SubG_{para}$, \techName{} begins at the receiver address of $e_{tg}$ and collects all incoming transactions occurring within $\tau_t$ after $e_{tg}$ and involving the same token name. From these, \techName{} identifies transactions whose amounts are close to that of $e_{tg}$ within the similarity threshold~$\tau_a$. Finally, these parallel transactions, together with $e_{tg}$, constitute the parallel subgraph.

\end{packeditemize}

\smallskip
\techName{} further classifies the fund movement patterns of the target transaction based on its subgraphs into five types: single outflow, entire disperse,  partial disperse, mix, and no forward. The detailed procedure is described in Algorithm~\ref{alg:flow_awareness}, lines. Based on the pattern type, \techName{} generates the flow text, summarizing the fund source, destination, distribution, and temporal characteristics. Figure~\ref{fig:tmp_flow_} presents the template of the flow text.


\begin{figure}[h]
\begin{center}
\includegraphics[width=0.47\textwidth]{Figs/template_subg.pdf}
\end{center}
\caption{\label{fig:tmp_flow_} Flow template text. }
\end{figure}


\begin{figure}[h]
\begin{center}
\includegraphics[width=0.42\textwidth]{Figs/example_graph.pdf}
\end{center}
\caption{\label{fig:exa_g} Example of subgraph construction of target transaction $e_{2}$. Subgraphs are color-coded for clarity. }
\end{figure}

% 优化caption

\heading{Runing examples.} Figure~\ref{fig:exa_g} illustrates an example of the construction of the upstream, downstream, and parallel subgraphs for a target transaction $e_{tg}$ (i.e., \hlhref{https://etherscan.io/tx/0xb570cf9587c99e978038c85e6f05d2fc50d12031ba3809102c66f71343b306c8}{$e_{2}$}). Here we apply the threshold settings used in our experiments (Section~\ref{sec:exps}).

\hlhref{https://etherscan.io/tx/0xe0a79310d14952ece3f7e72fae8c82aaf4c5d9d766918526a6a70b858f4e64ce}{$e_{1}$} occurs before \hlhref{https://etherscan.io/tx/0xb570cf9587c99e978038c85e6f05d2fc50d12031ba3809102c66f71343b306c8}{$e_{2}$} and has the same transfer amount, so it is regarded as a fund source. \hlhref{https://etherscan.io/tx/0x12a9f9347630615465c91d8bd79a21524ef2b73ff7a2ff2c3b3feeda112422d2}{$e_{5}$} and \hlhref{https://etherscan.io/tx/0x26540007067dc02e18948ff8e8038c552b7dffc81dce451a0d659b7d8bbc6dcb}{$e_{6}$} occur after \hlhref{https://etherscan.io/tx/0xb570cf9587c99e978038c85e6f05d2fc50d12031ba3809102c66f71343b306c8}{$e_{2}$} and are the earliest set of outgoing transactions of the receiver of \hlhref{https://etherscan.io/tx/0xb570cf9587c99e978038c85e6f05d2fc50d12031ba3809102c66f71343b306c8}{$e_{2}$} whose cumulative amount reaches $90\%$ of the amount of \hlhref{https://etherscan.io/tx/0xb570cf9587c99e978038c85e6f05d2fc50d12031ba3809102c66f71343b306c8}{$e_{2}$}, so they are classified as downstream transactions. 
 \hlhref{https://etherscan.io/tx/0x34bd630718364bec3859dc053f0ba202a85ae30f13c8365b47b647e84244a855}{$e_{4}$} is one of the incoming transactions of the receiver of \hlhref{https://etherscan.io/tx/0xb570cf9587c99e978038c85e6f05d2fc50d12031ba3809102c66f71343b306c8}{$e_{2}$}, whose amount differs from that of \hlhref{https://etherscan.io/tx/0xb570cf9587c99e978038c85e6f05d2fc50d12031ba3809102c66f71343b306c8}{$e_{2}$} by less than $5\%$, and is therefore included in ${SubG}_{para}$. According to Algorithm~\ref{alg:flow_awareness}, the cumulative downstream amount is greater than $0.9 \times e_{2}(amount)$ and the number of downstream transactions is greater than one, so the flow type is identified as entire disperse. Finally, \techName{} generates the corresponding flow text summarizing its source:



% \vspace{-0.1in}
\begin{center}
  % \fbox{
\colorbox{blue!9}{
\begin{minipage}{0.95\linewidth}
  (\textit{Entire disperse}) Receiver \hlhref{https://etherscan.io/address/0xd99f81773bb3b7eED44BD21C297Fd352Bccc6C5d}{0xd99f} dispersed 61.2 ETH from sender \hlhref{https://etherscan.io/address/0x8a4f03ca00400795119934c2ed458d8dd74a1dad}{0x8a4f} into 2 transactions within 2 minutes.
\end{minipage}
      }
 %  }
\end{center}


% \input{Alg/construct_alg}

==> chapter/4-4-semantics-flow-fusion.tex <==
\subsection{(Phase-\circlednum{3}) Semantics-Flow Fusion}
\label{subsec-fusion}

We now enter the third phase. We aim to integrate both semantic and structural information of each transaction. The goal is to produce a unified representation that enhances the accuracy of money laundering detection.


We encode the semantic and flow descriptions of each transaction using a fine-tuned LLM, while a graph convolutional network (GCN)~\cite{kipf2016semi} is trained in parallel to extract structural embeddings from the transaction MultiDiGraph. We then employ a cross-attention mechanism to fuse the two embeddings to capture cross-modal dependencies between the semantic and structural views.
The joint representation preserves both transaction semantics and fund-flow patterns, enabling deep modeling of complex laundering activities.

\begin{packeditemize}
     
\smallskip    
\item\underline{\textit{Text embedding via LLM}} (Figure~\ref{fig:llm}). 
\techName{} concatenates  the semantics text $\text{Txt}_{sem}$ with the flow text $\text{Txt}_{flow}$ to form a complete transaction text description $\text{Txt} = Concat(\text{Txt}_{sem},\text{Txt}_{flow})$. 
Given that general-purpose language models have limited understanding of cryptocurrency transaction contexts, we perform domain-specific supervised fine-tuning on the LlaMA3 model~\cite{grattafiori2024llama} using an instruction-tuning paradigm~\cite{wei2021finetuned} implemented with Low-Rank Adaptation (LoRA)~\cite{hu2022lora} for parameter-efficient training.  

Each training instance follows the standard instruction-tuning format, comprising three elements: \textit{instruction}, \textit{input}, and \textit{output}.
The instruction specifies the classification task and output format, the input is the transaction text description, and the output is the transaction label (ML or normal). After fine-tuning, the transaction description $\text{Txt}$ is passed into the adapted model to generate its text embedding, denoted as $\text{H}_{txt}$.

 
% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.5\textwidth]{Figs/fine-tuning.pdf}
% \end{center}
% \caption{\label{fig:llm} Generate text embedding via fine-tuning LLM. }
% \end{figure}

\begin{figure}[h]
\begin{center}
% \includegraphics[width=0.48\textwidth]{Figs/text_embed_big.png}
\includegraphics[width=0.48\textwidth]{Figs/lora.pdf}
\end{center}
\caption{\label{fig:llm} Generate text embedding via fine-tuning LLM. }
\end{figure}


\smallskip    
\item\underline{\textit{Structure embedding via GCN.}} \techName{} uses the transaction MultiDiGraph as input to capture the topological relationships and contextual information of transactions within the global transaction graph. Each address is initially assigned a feature vector representing the number of transactions associated with that address. We then employ a two-layer GCN~\cite{kipf2016semi} to iteratively update the node features, resulting in node embeddings with a broader receptive field and richer contextual information. Formally, the layer-wise propagation is defined as: 
$$\text{H}^{(l+1)} = \sigma\left( \tilde{\text{D}}^{-\frac{1}{2}} \tilde{\text{A}} \tilde{\text{D}}^{-\frac{1}{2}} \text{H}^{(l)} \text{W}^{(l)} \right),$$ 
\textit{where $\tilde{A}$ is the adjacency matrix with self-loops, $\tilde{\text{D}}$ is its degree matrix, $\text{H}^{(l)}$ is the address embedding at layer $l$, $\text{W}^{(l)}$ is the trainable weight matrix, and $\sigma(\cdot)$ is the activation function.} 
For each transaction, the embeddings of the sender and receiver from the final GCN layer are concatenated to form the structural representation:
$$ \text{H}_{str}=\mathrm{Concat}\left(\text{H}^{(L)}_{from},\; \text{H}^{(L)}_{to}\right),$$ \textit{where $L=2$ in \techName{}.}


\smallskip    
\item\underline{\textit{Fusion embedding via cross-attention.}} To enable deep interaction between semantic and structural views, \techName{} fuses the text embedding~$H_{txt}$ and the structural embedding $H_{str}$ via a bi-directional cross-attention mechanism~\cite{lu2019vilbert}. Before fusion, both embeddings are projected into a shared latent space of dimension through learnable linear transformations to ensure feature alignment: 
$$\tilde{\text{H}}_{txt} = \text{W}_{txt} \text{H}_{txt}, \tilde{\text{H}}_{str} = \text{W}_{str} \text{H}_{str}.$$ 
The cross-attention module performs information fusion. In the structure-to-text direction, structure embeddings act as queries to retrieve relevant text information from the text embeddings, and in the text-to-structure direction, text embeddings serve as queries to capture structural patterns from structure embeddings: 
% \[
% \text{F}_{s2t} = \mathrm{Attn}\big(
%     \underbrace{\tilde{\text{H}}_{struct}}_{Query},
%     \underbrace{\tilde{\text{H}}_{text}}_{Key},
%     \underbrace{\tilde{\text{H}}_{text}}_{Value}
% \big),\\
% ~\text{F}_{t2s} = \mathrm{Attn}\big(
%     \underbrace{\tilde{\text{H}}_{text}}_{Query},
%     \underbrace{\tilde{\text{H}}_{struct}}_{Key},
%     \underbrace{\tilde{\text{H}}_{struct}}_{Value}
% \big).
% \]




\begin{align*}
\text{F}_{s2t} &= \mathrm{Attn}\big(
    \underbrace{\tilde{\text{H}}_{struct}}_{\text{Query}},
    \underbrace{\tilde{\text{H}}_{text}}_{\text{Key}},
    \underbrace{\tilde{\text{H}}_{text}}_{\text{Value}}
\big), \\
\text{F}_{t2s} &= \mathrm{Attn}\big(
    \underbrace{\tilde{\text{H}}_{text}}_{\text{Query}},
    \underbrace{\tilde{\text{H}}_{struct}}_{\text{Key}},
    \underbrace{\tilde{\text{H}}_{struct}}_{\text{Value}}
\big).
\end{align*}


The two attention outputs are concatenated and normalized~\cite{ba2016layer} to form the final fused representation: 
$$\text{H}_{fused} = LayerNorm\left( [\text{F}_{s2t} \,\|\, \text{F}_{t2s}] \right).$$

\end{packeditemize}





 

==> chapter/4-5-SAR-generation.tex <==
\subsection{(Phase-\circlednum{4}) SAR Generation} 
\label{subsec-sar}


In the SAR generation phase, \techName{} aims to detect money laundering transactions and transform the detection results into the reports for forensic investigation. 

We leverage the fusion embeddings to identify money laundering transactions using a Multi-Layer Perceptron (MLP) classifier~\cite{tolstikhin2021mlp}. For transactions flagged as suspicious, a visualization module reconstructs the corresponding fund-flow graph, illustrating the path of laundered assets. In addition, the transaction semantics and flow information are incorporated into prompts for LLMs, which generates concise summaries of the laundering process along with key red flags that indicate suspicious behavior.

\begin{packeditemize}

\item\underline{\textit{ML transaction detection.}} \techName{} takes the fusion embeddings $H_{fused}$ as input to the MLP classifier to detect money laundering transactions:
\[\hat{y} = \arg\max_{k \in \{0,1\}} \left[ W_2 \cdot \mathrm{ReLU}(W_1 H_{fuse} + b_1) + b_2 \right]_k, 
\]
\textit{where \(W_1, W_2\) and \(b_1, b_2\) are trainable parameters, \(\mathrm{ReLU}(\cdot)\) is the rectified linear unit activation function, \(\arg\max\) returns the index of the larger logit, and \([\cdot]_k\) denotes the \(k\)-th element, and \(\hat{y}\) is the predicted class label (0 for normal, 1 for money laundering).}

\smallskip  
\item\underline{\textit{ML flow visualization.}} The visualization module merges multiple related money laundering transaction subgraphs and renders them as a Sankey diagram, providing a holistic view of multi-hop fund flows. Figure~\ref{fig:flow_eg} illustrates\footnote{The figure is static. An interactive version in our SARs supports hover tooltips: edges show tx details; nodes show per-address tx counts.}  an example of a money laundering flow.
\end{packeditemize}


% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.48\textwidth]{Figs/tx_flow_eg.pdf}
% \end{center}
% \caption{\label{fig:flow_eg}Example of ML flow Sankey diagram. }
% \end{figure}
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.45\textwidth]{Figs/eg_flow_frame.pdf}
\end{center}
\caption{\label{fig:flow_eg}Example of ML flow. Edge width is proportional to the transfer amount, edge color indicates the token name, and purple squares represent addresses.}
\end{figure}

% Hovering over an edge displays the detailed transaction information, and hovering over a purple square shows the number of transactions associated with that address.

% (i.e. attacker)


\heading{Red flags.} \techName{} combines the transaction descriptions from each money laundering flow with analysis instructions (e.g., generating fund flow summary, listing red flag) into a prompt, which is then fed to GPT-4o. GPT-4o is selected for its strong long-context understanding and reasoning capabilities~\cite{shahriar2024putting}. 

Figures~\ref{fig:middle} and~\ref{fig:down} illustrate typical GPT-4o outputs: the green section provides a concise fund-flow summary outlining key phases from fund injection to conversion and distribution, while the red panel enumerates red flag indicators that capture high-risk behavioral patterns such as rapid multi-hop transfers, repeated swaps, identical chunk sizes, and account reuse. These outputs can be directly embedded into SARs, allowing investigators to quickly identify laundering typologies and suspicious transactions.



% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.48\textwidth]{Figs/summary.pdf}
% \end{center}
% \caption{\label{fig:sum_eg} Example of summary of ML process and red flags generated by GPT-4o.}
% \end{figure}



==> chapter/4-approach.tex <==

% \cleardoublepage

\section{Design of \techName{}} \label{sec:approach}

We first present an overview (\S\ref{subsec-archi}) of our framework. We then show the details of each phase (\S\ref{subsec-semantic}-\S\ref{subsec-sar}).


\input{chapter/4-1-overview}

\input{chapter/4-2-semantic-awareness}

\input{chapter/4-3-graph-construction}

\input{chapter/4-4-semantics-flow-fusion}

\input{chapter/4-5-SAR-generation}







==> chapter/5-1-settings.tex <==



\begin{figure}[h]
\begin{center}
\includegraphics[width=0.43\textwidth]{Figs/daily_stats.pdf}
\end{center}
\caption{\label{fig:sum_daily} Daily distribution of transactions in \textit{BybitML}. The stacked bars represent the number of normal and  ML transactions, and the purple line indicates the  ML ratio. }
\end{figure}


% \heading{New dataset.} We contribute a new multi-chain benchmark dataset, \textit{BybitML}\footnote{\url{https://osf.io/nx7aj/overview?view_only=663038fbea43491bb4010011c7f28b23}}, derived from one of the largest real-world money laundering incident, Bybit hack,  to date~\cite{bybit25}. 
% We collected transactions on Ethereum and Bitcoin from the two weeks following the Bybit Hack incident. Then, we filtered (i) \textit{money laundering transactions} based on the \textsc{ML} label provided by Elliptic\footnote{\url{https://www.elliptic.co/platform/data-fabric}} and (ii) \textit{normal transactions} based on the \textsf{Normal} label provided by Arkm\footnote{\url{https://intel.arkm.com/}}, resulting in a 14-day benchmark dataset. 

% \qs{lllinkkkk}

\heading{New dataset.} We contribute \textit{BybitML}, 
a new multi-chain benchmark dataset constructed from the 2025 Bybit Hack, one of the largest real-world laundering incidents to date~\cite{bybit25}. 
We collect transactions on Ethereum and Bitcoin within the two weeks following the incident and assign ground-truth labels from established intelligence sources: 
(i) \textit{money-laundering transactions} using the \textsc{ML} tag from \hlhref{https://www.elliptic.co/platform/data-fabric}{Elliptic}, 
and (ii) \textit{normal transactions} using the \textsf{Normal} tag from \hlhref{https://intel.arkm.com/}{Arkham}. 
This results in a 14-day, multi-chain benchmark dataset that enables reproducible evaluation under realistic laundering conditions.


The dataset contains 2.75M transactions, comprising 230K ML transactions and 2.52M normal transactions. Figure~\ref{fig:sum_daily} illustrates the daily proportion of laundering versus normal transactions across the 14 days. The final
dataset is divided into two synchronized subsets: \textit{BybitML-
EC} (Ethereum) and \textit{BybitML-BC} (Bitcoin), supporting both intra-chain and cross-chain evaluation.

\heading{Baseline.}  We compare \textsc{FlowShield} with prior AML methods based on different techniques, including: 
\begin{packeditemize}
  \item \textit{heuristic}: 
  Cyclic~\cite{lv2023detection} detects cyclic transaction patterns, and XBlock~\cite{wu2023towards} uses blacklist poisoning to identify transactions linked to illicit addresses.
    
  \item \textit{machine learning}: 
  Multi-Layer Perceptron (MLP)~\cite{rosenblatt1958perceptron}, Logistic Regression (LR)~\cite{cox1958regression}, and Support Vector Machine (SVM)~\cite{cortes1995support} are trained on transaction-level statistical features for ML detection~\cite{elmougy2023demystifying}.

  \item \textit{graph learning}: 
  GCN~\cite{kipf2016semi} and GraphSAGE~\cite{hamilton2017inductive} leverage transaction graph structure for ML detection~\cite{Mara24anti}, while Tracer~\cite{wu2023tracer} tracks fund flows through subgraph search.

  \item \textit{LLM-based}: 
  Llama3~\cite{grattafiori2024llama}, fine-tuned on transaction texts, detects laundering behaviors from semantic patterns.
\end{packeditemize}


% \heading{Metric.} We employ four metrics: Precision ($\text{P}=\tfrac{\text{TP}}{\text{TP}+\text{FP}}$), Recall  ($\text{R} = \tfrac{\text{TP}}{\text{TP}+\text{FN}}$), F1 score ($\text{F1} = \tfrac{2\text{P}\text{R}}{\text{P}+\text{R}}$), and money coverage rate ($\text{MCR}= \tfrac{\text{V}(\text{TP})}{\text{V}(\text{TP}) + \text{V}(\text{FN})}$), where $\text{V}(\text{TP})$ and  $\text{V}(\text{FN})$  denote the total value of detected and undetected ML funds.

\heading{Metric.}  
We evaluate detection performance using four mainstream metrics:  {Precision (P)},  {Recall (R)},  {F1 score (F1)}, and  {money coverage rate (MCR)} (definition deferred to Appendix~\ref{apd-metrics}).

\heading{Threshold setting.}
~We empirically set the time window threshold~$\tau_t=24$, the flow ratio threshold~$\tau_f=0.9$, and the amount similarity threshold~$\tau_a=0.05$. These values are chosen based on empirical analysis (see Section~\ref{sec:disscusion}).




==> chapter/5-2-RQ1.tex <==
\subsection{RQ1: Effectiveness}

\input{Tabs/tab_effectiveness_avg}

\input{Tabs/tab_comparative_exp}



%增加内容：ETH数据集怎么做的，BTC怎么做的
% 考虑到不同区块链数据规模的差异，Bybit_EC数据量较大，因此我们采用按天划分的方式，对每一天的数据分别进行建模与评估；而 Bybit_BC数据量相对较小，因此在整体上进行一次性训练与评估。
%此外，为了评估在实际应用场景下的处理能力，我们还测试了模型在不同规模数据集下的检测耗时，以分析其可扩展性表现。

\heading{Setup.} We evaluate \techName{} on the \textit{BybitML} dataset by comparing its performance with multiple baselines. Due to the difference in data scale between the two blockchains, we perform day-by-day training and evaluation for the larger \textit{BybitML-EC} dataset, while the smaller \textit{BybitML-EC} dataset is trained and evaluated as a whole. To assess the scalability of \textsc{FlowShield} in realistic deployment scenarios, we measure its detection time across different dataset sizes.

%baselines. To better simulate real-world deployment, we adopt a day-by-day evaluation, where each day's data is modeled and assessed independently. 

For supervised methods, each day's data is split into training, validation, and test sets with a 6:2:2 ratio, and independent models are trained. Unsupervised methods require no training and are directly applied to the full daily dataset. For fine-tuning LlaMA3, we sample 5,000 records using stratified sampling to reduce training time, while the remaining data is reserved for testing. 

%All experiments are repeated five times, and average results are reported.（LLM的没有重复做5次）


%两个数据集上效果好-->在稀疏不均衡数据上好-->数据处理时间短且扩展性高
% \heading{Results.} Table~\ref{tab:avg_metrics_ec} and~\ref{tab:avg_metrics_bc} 

\heading{Results.}  Table~\ref{tab:avg_metrics} shows that \techName{} outperforms all baselines on both \textit{Bybit-EC} and \textit{Bybit-BC}, achieving the highest precision, recall, and F1 score while maintaining a high MCR. Although SAGE attains the best MCR on \textit{Bybit-EC}, its lower precision indicates higher FP. In contrast, \techName{} maintains the highest precision with an MCR of 88\%, underscoring its practical effectiveness, where both precision and effective fund-tracing are crucial.


%增加描述后三天所有baselines的效果大幅下降，但是我们方法没有下降：在第 12 到 14 天中，大部分基线方法的性能明显下降，这一阶段对应洗钱流程的后期，交易结构稀疏且标签样本分布不均。传统方法仅能捕捉表层特征，图方法在结构信号减弱时性能下降，基于 LLM 的语义方法虽能理解交易语义但缺乏结构约束，同样不稳定。相比之下，\textsc{FlowShield} 融合语义与资金流信息，既能捕捉交易行为逻辑，又能建模结构关联，因此在后期仍保持稳定性能。
Table~\ref{tab:avg_f1} shows that \textsc{FlowShield} remains robust under sparse and imbalanced data conditions. From Day~\circled{12} to~\circled{14}, when the laundering process enters its late stage with fewer transactions and highly skewed labels~(Figure~\ref{fig:sum_daily}), most baselines exhibit a sharp performance decline. \textit{Heuristic} and \textit{machine learning} methods fail to adapt due to their reliance on shallow numerical features, while \textit{graph-based} models degrade as structural signals diminish. \textit{LLM-based} approaches capture limited semantic cues but lacks structural grounding, resulting in instability.  
In contrast, \textsc{FlowShield} fuses semantic reasoning with flow-aware structure learning, enabling it to preserve behavioral consistency and sustain stable performance throughout the laundering timeline.


\begin{figure}[h]
\begin{center}
\includegraphics[width=0.43\textwidth]{Figs/BTC_Flowshield_scalability.pdf}
\end{center}
\vspace{-0.1in}
\caption{\label{fig:scalability}Detection time of \textsc{FlowShield} under different transaction numbers, showing linear scalability. }
\end{figure}



%detection time的结果描述： Figure~\ref{fig:scalability}  展现了\textsc{FlowShield} 在大规模交易数据上仍能保持高效的检测效率. 随着交易数量从 5 万增长至 50 万，系统的总检测时间几乎呈线性增长，且每笔交易的平均检测时间始终稳定在约 0.02 毫秒，远低于链上交易验证时间。
Figure~\ref{fig:scalability} demonstrates scalability.  As the transaction volume increases from 50K to 500K, the total detection time grows linearly. The average per-transaction latency remains around 0.02ms, far below typical on-chain confirmation times.  
These results confirm that \textsc{FlowShield} scales efficiently to large transaction sets and supports real-time laundering detection in practical blockchain environments.


\begin{center}
  % \fbox{
\colorbox{teal!9}{
\begin{minipage}{0.95\linewidth}
\textbf{Answer to RQ1}: \textsc{FlowShield} achieves superior detection performance, reaching an average F1 of 97.4\% on \textit{Bybit-EC} and 97.7\% on \textit{Bybit-BC}, outperforming the best baseline by 6.2\% and 3.4\%, respectively. It remains stable under sparse and imbalanced data and exhibits strong scalability with an average transaction detection time of only 0.02 ms, enabling efficient large-scale detection.
% \techName{} outperforms all baselines, achieving the best average precision (\qw{fill x\%}), recall (\qw{x\%}), and F1 score (\qw{x\%}) while maintaining stable performance across 14 days. It strikes a good balance between detection accuracy and fund coverage, making it well-suited for real-world AML scenarios. 
\end{minipage}
      }
 %  }
\end{center}



==> chapter/5-3-RQ2.tex <==
\subsection{RQ2: Component Contribution}

\heading{Setup.} We conducted ablation experiments. We removed three modules individually while keeping all other settings unchanged. We then trained/tested those modified variants and compared average values of key performance metrics.


\begin{figure}[h]
\begin{center}
\includegraphics[width=0.45\textwidth]{Figs/ablation_results.pdf}
\end{center}
\vspace{-0.1in}
\caption{\label{fig:ablation} Ablation experiments. We remove each component (semantics, flow, fusion) to compare performance.}
\end{figure}


\heading{Results} (Figure~\ref{fig:ablation}). The complete \techName{} achieves the best performance across all performance metrics, demonstrating that the joint contribution of flow awareness, semantic awareness, and fusion is essential for effective detection. 

When semantic awareness is removed, both precision and recall decrease significantly, leading to the largest drop in F1 score and underscoring the importance of semantic information for comprehensively characterizing transaction behaviors. Without flow awareness, Recall drops noticeably, indicating that flow information is critical for capturing the flow of ML transactions. Without the semantics-structure fusion module, the model can still utilize semantic and structural features independently and thus maintain reasonably high precision and recall. However, its overall performance remains inferior to the complete system, showing that the interaction between semantics and structure is vital.




% \vspace{-0.1in}
\begin{center}
  % \fbox{
\colorbox{teal!9}{
\begin{minipage}{0.95\linewidth}
\textbf{Answer to RQ2}: Every component contributes to detection performance. Removing any of them leads to a performance drop. Instead, their combination yields complementary benefits, with best results across all metrics.  
\end{minipage}
      }
 %  }
\end{center}

==> chapter/5-4-RQ3.tex <==
\subsection{RQ3: Strategy Analysis}

\heading{Setup.} We analyze the laundering transactions identified by the model on each day. We classify these transactions into semantic types, and further examine behavioral features within each category to capture common evasion tactics. In addition, we analyze token swap behaviors to summarize frequently used swap pairs, and investigate cross-chain transfers from the perspectives of destination blockchains and receiving addresses.

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.42\textwidth]{Figs/semantic_tx_num.pdf}
\end{center}
\caption{\label{fig:seman_num}Distribution of money laundering transaction semantics across days.}
\end{figure}


% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.2\textwidth]{Figs/au_tran_ratio.pdf}
% \end{center}
% \caption{\label{fig:au_tra_ratio}}
% \end{figure}



% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.2\textwidth]{Figs/au_tran_day.pdf}
% \end{center}
% \caption{\label{fig:au_tra_day}}
% \end{figure}

\heading{Semantics distribution} (Figure~\ref{fig:seman_num}).
Direct transfers dominate, representing the most straightforward approach that launderers commonly rely on. Cross-chain transfers and token swaps increase noticeably in the early days, reflecting a tendency of launderers to quickly move funds to other blockchains or convert illicit assets into alternative tokens to complicate tracing. In contrast, indirect transfers remain relatively rare, since these transactions typically require smart contracts to perform multi-step transfers within a single transaction, making them less frequently used.

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.48\textwidth]{Figs/swap_pair_activity_heatmap.pdf}
\end{center}
\caption{\label{fig:swap_heat}Heatmap of token swap intensity across 14 days.}
\end{figure}

%图 (b) 展示了 14 天内规避行为的演化过程：第 1 天 Automation 占比高，表明在盗窃初期攻击者主要依赖自动化批量分散资金以防止被冻结；随着时间推移，Automation 占比下降而 Transit 占比上升，说明资金逐步进入多跳中转和跨链转移。

\heading{Token swap intensity} (Figure~\ref{fig:swap_heat}). The swap between DAI and ETH is the most frequent, reaching its peak on day 2 and day 4. This indicates that, in the early stage of ML, launderers prefer the swap between the stablecoin (DAI) and the native token (ETH). In addition, swaps between stablecoins (e.g., USDC→USDT) appear multiple times, suggesting that launderers deliberately leveraged various stablecoin to further obfuscate fund flows. Overall, the activity of swaps declined significantly after day 10, implying that the core ML have been completed. Moreover, cross-chain related token swaps, such as DAI→WBTC, are also observed. These swaps indicate that the funds gradually entered the cross-chain transfer stage, aiming to migrate assets to the Bitcoin blockchain.




\begin{figure}[h]
\begin{center}
\includegraphics[width=0.43\textwidth]{Figs/cross_value.pdf}
\end{center}
\caption{\label{fig:cross_value}Cumulative cross-chain amount of ETH and DAI.}
\end{figure}


\heading{Cross-chain analysis} (Figure~\ref{fig:cross_value}). We observe that the launderer predominantly transferred funds from Ethereum to the Bitcoin blockchain by the \hlhref{https://thorchain.org/}{Thorchain bridge}, with only a single transaction routed to BNB Smart Chain. In total, we detect 1,878 cross-chain addresses on Bitcoin, uncovering approximately US\$930M in cross-chain laundering. 
The launderers usually deposit ETH and DAI to the bridge. The cumulative volume of ETH far exceeds that of DAI. Further examination of the receiving addresses on Bitcoin shows that while most addresses received only one or two transactions, a small number of addresses act as aggregation points. For example, address \hlhref{ https://blockstream.info/address/bc1qjm4u92xpcahtmhtjrp3r4vdy6reg4yg4lvz79z}{{bc1qjm}} on Bitcoin received funds from Ethereum via 195 transactions, and address \hlhref{https://blockstream.info/address/bc1qcpylyx6w4mqfks9ehun7mwqmq3ndgf8nd2mkpj}{ {bc1qcp}}  consolidated the funds from Ethereum around 6,654 ETH, indicating centralized collection behavior.

% bc1qjm4u92xpcahtmhtjrp3r4vdy6reg4yg4lvz79z
% https://blockstream.info/address/bc1qjm4u92xpcahtmhtjrp3r4vdy6reg4yg4lvz79z
% \hlhref{ https://blockstream.info/address/bc1qcpylyx6w4mqfks9ehun7mwqmq3ndgf8nd2mkpj}{ {bc1qcp}} 


\begin{figure}[h]
\centering
\begin{subfigure}{0.23\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figs/au_tran_ratio.pdf}
  \caption{By semantics.}
  \label{fig:au_tra_ratio}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figs/au_tran_day.pdf}
  \caption{By day.}
  \label{fig:au_tra_day}
\end{subfigure}
\label{fig:au_tra}
\caption{Evasion behavior analysis. (a) distribution of Automation, Transit, and Other behaviors across transaction semantics; (b) distribution of these behaviors over 14 days.}

\end{figure}



\heading{Evasion behaviors.} Launderers often adopt evasion behaviors to circumvent regulation and tracing. \textit{Automation} refers to the use of scripts to conduct programmatic transfers, while \textit{transit} refers to transactions that immediately forward the entire received amount to the next address. In the detected ML transactions, those with similar amounts and within a short time are labelled as \textit{automation}; those whose funds are immediately and fully forwarded downstream are labelled as \textit{transit}; all remaining are regarded as \textit{other}. 

Figure~\ref{fig:au_tra_ratio} shows differences in evasion behaviors across transaction semantics: in direct transfers, \textit{automation} accounts for a larger proportion, indicating that launderers tend to rely on automated scripts to disperse funds; cross-chain transactions are dominated by \textit{transit} behavior, indicating that funds are relayed through intermediaries before entering bridges to avoid direct exposure of hacker addresses. 

Figure~\ref{fig:au_tra_day} illustrates the evolution of evasion behaviors over 14 days: on day 1, \textit{automation} dominates, indicating that in the early stage, launderers relied on automated fund dispersal to evade freezing. \textit{Automation} and \textit{transit} exhibit similar temporal patterns, both start with a high proportion on day 1, drop sharply in the following days, show a slight rebound around day 3 to 5, and then fluctuate at lower levels. This similarity suggests that launderers may adjust these two behaviors in tandem.




% \vspace{-0.1in}
\begin{center}
  % \fbox{
\colorbox{teal!9}{
\begin{minipage}{0.95\linewidth}
\textbf{Answer to RQ3}: \textsc{FlowShield} can identify multiple strategies. 
Automated transfers disperse funds in the early stage.  Token swaps dominate in the mid stage. Cross-chain transfers appear throughout the process and show transit patterns, with most funds moving from Ethereum to Bitcoin via Thorchain. On Bitcoin, most receiver addresses are short-lived, and few act as aggregation points. 
\end{minipage}
      }
 %  }
\end{center}

==> chapter/5-5-RQ4.tex <==
\subsection{RQ4: In-the-wild Detection}

\heading{Setup.} Since money laundering activities are continuous while labeled data are often delayed, we design an in-the-wild detection experiment to evaluate the generalization ability of \textsc{FlowShield} in real-world scenarios. We use one week of data and apply the model trained on day~$t$ directly to detect transactions on day~$t\!+\!1$ without retraining, simulating performance on unseen future data.

\input{Tabs/tab_wild_exp}



% 从第 \circledc{6} 天到第 \circledc{10} 天，\textsc{FlowShield} 在各项指标上持续保持稳定表现，F1 始终高于 96%，MCR 大多超过 90%。其中，第 \circledc{7} 天出现一次 MCR 下探至 83% 的情况，主要原因在于当日存在少量金额异常巨大的洗钱交易，其行为模式偏离了主流特征，从而影响了整体资金覆盖率；但值得注意的是，当日的 F1 依然高达 99.3%，说明模型对绝大多数洗钱行为仍保持精确识别能力。

% 第 \circledc{12} 天的 F1 出现显著下降。结合图 \ref{fig:seman_num} 与图 \ref{fig:au_tra_day} 可见，第 \circledc{11} 天与第 \circledc{12} 天的语义分布和规避方式发生了突然变化，引发了突发性的模式漂移，自然造成性能波动。尽管如此，第 \circledc{12} 天的 MCR 仍保持在 95% 以上，体现出 \textsc{FlowShield} 对主要非法资金流的持续覆盖能力。

% 整体来看，\textsc{FlowShield} 在跨日期场景中展现出强劲的稳定性和鲁棒性：即便面对突发的策略变动与“逆势”高金额交易，其对绝大部分洗钱资金的识别与覆盖能力仍然保持可靠。
\heading{Results} (Table~\ref{tab:wild}). \textsc{FlowShield} maintains high in-the-wild detection performance in most periods. Compared with the original settings (Orig.), the performance of Wild only drops slightly, indicating that \textsc{FlowShield} exhibits robustness in cross-day detection. 
From day \circledc{6} to day \circledc{10}, F1 score stays around 96\% and MCR mostly above 90\%. The only exception is day \circledc{7}, where the MCR dips to 83\% due to a few atypical high-value ML transactions that deviate from typical laundering patterns. Even so, the F1 score on that day remains 99.3\%, showing that \textsc{FlowShield} still correctly identifies nearly all laundering activities. A decline in F1 score is observed on day \circledc{12}. As shown in Fig.~\ref{fig:seman_num} and Fig.~\ref{fig:au_tra_day}, day \circledc{11} and day \circledc{12} exhibit abrupt shifts in semantic distribution and evasion behaviors, causing a sudden change in laundering patterns and resulting performance fluctuation.  Despite this shift, the MCR on day \circledc{12} remains above 95\%, showing \textsc{FlowShield}'s continued ability to cover major laundering flows. 

% Overall, \textsc{FlowShield} demonstrates strong cross-day stability and robustness: even under abrupt strategy shifts and extremely high-value transactions, it consistently delivers reliable detection and high fund coverage.

% A decline in F1 is observed on day \circledc{12}. As shown in Fig.~\ref{fig:seman_num} and Fig.~\ref{fig:au_tra_day}, the semantic distribution and evasion behaviors on day \circledc{11} and day \circledc{12} undergo abrupt changes, leading to a sudden shift in laundering patterns and naturally causing performance fluctuations. Despite this shift, the MCR on day \circledc{12} remains above 95\%, demonstrating \textsc{FlowShield}'s continued ability to cover major illicit fund flows.



% Overall, \textsc{FlowShield} exhibits strong stability and robustness in cross-day scenarios: even in the presence of sudden strategy changes and extremely high-value transactions,  \textsc{FlowShield} consistently maintains reliable detection and high fund coverage.


% Specifically, from day \circledc{6} to day \circledc{11}, F1 remains above 96\% and MCR mostly exceeds 90\%. On day \circledc{12}, however, F1 drops significantly to 66.3\%. As illustrated in ~\ref{fig:seman_num} and ~\ref{fig:au_tra_day}, the semantic distribution and evasion behaviors on day \circledc{11} and day \circledc{12} differ substantially, making it difficult for the model to fully capture the new patterns without retraining. Despite the fluctuation in F1, MCR consistently remains above 95\%. One exception occurs on day \circledc{7}, where the MCR is relatively low due to several high-value ML transactions that are not detected.


% \vspace{-0.1in}
\begin{center}
  % \fbox{
\colorbox{teal!9}{
\begin{minipage}{0.95\linewidth}
\textbf{Answer to RQ4}: \textsc{FlowShield} scales effectively in practice.  Without retraining on new data, it maintains high recall and MCR in most periods, and adapt to dynamical ML behaviors.  Performance drops on certain days but still covers the majority of illicit fund flows.
\end{minipage}
      }
 %  }
\end{center}

==> chapter/5-6-RQ5.tex <==
\subsection{RQ5: SARs Quality}


\heading{Setup.} We feed the detected money laundering fund flows into GenAI tools (i.e., ChatGPT-4o) to generate SARs. SAR can assist in generating explainable outcomes such as the summary of fund flow and the laundering red flags. 

To evaluate the validity of SARs, we invited three human experts with strong blockchain security backgrounds to conduct a manual evaluation. We randomly selected 30 SARs from the detection results, and each participant rated them on a 1–10 scale across three dimensions: (i) \textit{correctness}: whether the report accurately reflects the actual transaction flow; (ii) \textit{explainability}: whether the report is clear and facilitates the understanding of complex fund flows; and (iii) \textit{convincingness}: whether the report provides strong evidence to justify the suspiciousness.


\begin{figure}[h]
\begin{center}
\includegraphics[width=0.45\textwidth]{Figs/SARs_Evaluation_GroupedBar_Participants.pdf}
\end{center}
\caption{\label{fig:sar_rate} Average SARs quality evaluation scores.}
\end{figure}


\heading{Results} (Figure~\ref{fig:sar_rate}). On average, SARs scored above 8.5 across all three dimensions, confirming a high quality. Participants further noted that SARs are user-friendly, combining detailed transaction information with high-level flow summaries and multi-dimensional risk indicators. Minor issues remain, including occasional verbosity and less accurate interpretations of gas fees.





% \vspace{-0.1in}
\begin{center}

\colorbox{teal!9}{
\begin{minipage}{0.95\linewidth}
\textbf{Answer to RQ5}: SARs enable explainable detection results. They provide human-friendly descriptions of laundering flows with highlighted red flags.
\end{minipage}
      }

\end{center}


==> chapter/5-experiements.tex <==
\section{Our Evaluation} \label{sec:exps}



Our experiments are designed to answer the following research questions (RQs):

\begin{packeditemize}
\item RQ1 \textit{(effectiveness):} Does our method outperform existing crypto AML solutions?

\item RQ2 \textit{(component contribution):} Does each component contribute to the overall detection performance?

\item RQ3 \textit{(strategy analysis):} Which laundering strategies can \textsc{FlowShield} identify, and what distinctive characteristics do they exhibit?

\item RQ4 \textit{(generalization):} Can \textsc{FlowShield} trained in one time period generalize to another, effectively detecting ML transactions?

\item \textit{RQ5 (SARs explainability):} Do SARs improve the explainability of detection results?
\end{packeditemize}


\input{chapter/5-1-settings}

\input{chapter/5-2-RQ1}

\input{chapter/5-3-RQ2}

\input{chapter/5-4-RQ3}

\input{chapter/5-5-RQ4}

\input{chapter/5-6-RQ5}




==> chapter/5-security-analysis.tex <==
\section{Security analysis}
why our method worksshouxian 

==> chapter/6-related-works.tex <==
\section{Extended Related Works} \label{sec:related}

% \noindent\textbf{Crypto AML.}~~
% Existing Crypto AML approaches primarily fall into three categories: heuristic rule-based methods, traditional machine learning-based methods, and graph-based methods.
% Heuristic rule-based methods rely on predefined rules derived from known laundering patterns, such as blacklists~\cite{wu2023towards}, cyclic flows~\cite{lv2023detection}, or mixer usage~\cite{kuccuk2023investigation}. These methods are straightforward and effective for capturing known typologies, but fail against novel or obfuscated laundering strategies. Traditional machine learning-based methods train classifiers on features extracted from transactions. Examples include feature refinement~\cite{elmougy2023demystifying}, active learning~\cite{wang2024graphalm}, and anomaly detection~\cite{zhou2023visual}. They are more adaptive than rules but depend on feature engineering and often ignore relational context. Graph-based methods model the transaction data as networks to uncover laundering accounts or transactions.Subgraph search (e.g., DenseFlow~\cite{lin2024denseflow}, Tracer~\cite{wu2023tracer}), graph embeddings (e.g., GTN2Vec~\cite{liu2023graph}, Sub2Vec~\cite{bellei2024shape}), and GNNs~\cite{alarab2020competence,lo2023inspection,nicholls2023fraudlens,hyun2023anti,guo2023lb,song2024illicit} have been applied. Despite their improved capacity for complex pattern recognition, they remain structure-centric, lack integrated transaction semantics, and offer limited audit-ready explanations for compliance workflows.

The core studies were addressed earlier; we add a brief extension related to blockchain financial security.

\heading{Financial incidents.} 
The blockchain ecosystem witnesses escalating financial security incidents from protocol design to user interaction. DeFi ecosystem alone has suffered cumulative losses exceeding US\$3B~\cite{zhou2023sok}. These incidents broadly fall into three interrelated categories: 

\begin{packeditemize}
\item \textit{Protocol-level exploits.} DeFi protocols introduce complex interdependencies between decentralized exchanges, lending markets, and price oracles, creating new surfaces for transaction manipulation and economic exploitation. Attacks such as price manipulation~\cite{zhang2025following} and frontrunning~\cite{front21Torres,ma2025surviving} allow adversaries to extract millions of dollars within minutes by exploiting oracle latency or mempool visibility. These incidents expose systemic fragility in the incentive and execution layers of DeFi protocols.
\item \textit{Smart contract vulnerabilities.}
Flaws at the implementation level directly lead to crypto theft. Misconfigurations and programming mistakes have been repeatedly exploited in the wild (e.g, confused deputy vulnerabilities~\cite{291283}, storage collisions in upgradeable contracts~\cite{pancollisionrepair}), resulting in multi-million-dollar losses~\cite{255252}.
\item \textit{User-level scams and frauds.} The attack exploits users’ behavioral trust rather than protocol logic, further contributing to massive on-chain losses. These include address poisoning~\cite{tsuchiya2025blockchain}, giveaway scams~\cite{li2023double}, honeypot contracts~\cite{torres2019art}, rug pulls~\cite{spammer23fed}, and phishing campaigns~\cite{TxPhish23He}. 
\end{packeditemize}

Those studies concentrate on identifying on-chain exploits. However, the post-attack phase (i.e., how stolen assets are subsequently laundered) remains underexplored. It is a major step to convert compromised assets into spendable value. Our work fills this gap.


%A wide range of financial security issues become severer. DeFi ecosystem has lost more than 3 billion USD~\cite{zhou2023sok} in recent years. Scams and phishing attacks also pose severe threats to users. DeFi exploits and transaction manipulation mainly target protocol-level risks such as price manipulation~\cite{zhang2025following} and frontrunning~\cite{front21Torres,ma2025surviving}, which demonstrates that attackers can gain millions of USD in a very short period of time through such attacks. Representative examples include address poisoning~\cite{tsuchiya2025blockchain}, giveaway scams~\cite{li2023double}, honeypot contracts\cite{torres2019art}, rug pulls~\cite{spammer23fed}, and phishing~\cite{TxPhish23He}. And Smart contract vulnerabilities directly lead to Crypto theft. Studies show that flaws such as the confused deputy vulnerability~\cite{291283} and storage collision in upgradeable contracts~\cite{pancollisionrepair} can be exploited in the wild, which have already been compromised with million-dollar damages~\cite{255252}. While these studies highlight the severe financial security on blockchain, much less attention has been paid to how illicit funds are subsequently laundered, even though ML is the necessary step for attackers to cash out.


\heading{LLMs for blockchain security.} 
LLMs show strong potential in enhancing blockchain security, particularly in smart contract vulnerability detection~\cite{xu2024large}. Chen et al.~\cite{chen2025chatgpt} conduct a large-scale empirical study on ChatGPT’s capability for smart-contract vulnerability detection, revealing high recall but limited precision and stability across different vulnerability types. Sun et al.~\cite{sun2024gptscan} propose GPTScan, combining LLM reasoning with static analysis to detect logic vulnerabilities. Chen et al.~\cite{chen2024identifying} present SOChecker, which employs a fine-tuned LLaMA model to complete incomplete Stack Overflow code snippets and then performs symbolic execution to detect latent vulnerabilities. Beyond general vulnerability detection, recent studies extend LLMs to specialized and hybrid reasoning tasks. Wu et al.~\cite{wu2024semantic} propose Semantic Sleuth, a zero-shot Chain-of-Thought framework for uncovering Ponzi-scheme contracts, and Zhang et al.~\cite{zhang2024detecting} integrate LLM-based semantic annotation with rule-based reasoning to detect accounting and monetary logic errors. 

We also noted extended applications of LLMs in constructing transaction graphs~\cite{lei2025large}, formalising contract verifications \cite{liu2024propertygpt}, and simulating malicious exploits~\cite{gervais2025ai,xiao2025prompt}. However, their use in assisting crypto anti–money-laundering remains unexplored. Our work addresses it.

% \heading{LLM-assisted semantic analsyses.} 

==> chapter/7-conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}


% We presented \textsc{FlowShield}, a new Crypto AML framework that unifies transaction semantics, fund-flow modeling, semantics–structure fusion and SAR generation.  \textsc{FlowShield} achieves a 97.4\% average F1 score and 88\% fund coverage, outperforming nine baselines including GCN (80.2\%), SAGE (87.3\%), and Llama3 (91.2\%), and generates high-quality explainable SARs on large-scale real-world laundering data.

%We presented \textsc{FlowShield}, a new Crypto AML framework that integrates transaction semantics with fund-flow structures, enabling a unified understanding of both behavioral intent and asset movements. It further leverages semantics-structure fusion and SAR generation to deliver accurate and explainable detection at scale.

We presented \textsc{FlowShield}, a Crypto AML framework that delivers accurate, scalable, and explainable detection. It fuses transaction semantics with fund-flow structures via a unified fusion mechanism and generates high-quality SARs, capturing behavioural intent and asset movement.

We also constructed and released \textit{BybitML} (rooted in the largest Bybit Hack incident), the first multi-chain money-laundering benchmark dataset covering both Ethereum and Bitcoin. We evaluate \textsc{FlowShield} on it, and experimental results show that our framework significantly outperforms nine baselines. It effectively detects complex laundering behaviors, including US\$930M in cross-chain laundering, and maintains stable cross-period generalization. In addition, \textsc{FlowShield} achieves near real-time detection efficiency and produces high-quality, explainable SARs.



%We present \textsc{FlowShield}, a novel security system for Crpto AML detection to effectively detect and explain complex ML behaviors. The system leverages transaction semantics awareness to capture transactional intents and employs fund-flow awareness to reveal the structure and path of complex fund flows. A semantics–structure fusion mechanism enables interactions between semantic and structural information, thereby enhancing the detection of diverse ML strategies. \textsc{FlowShield} further utilizes LLM to automatically generate SARs that provide accurate, explainable, and convincing summaries of ML flow and red flags. 
%In future work, we aim to extend the system to more complex scenarios, including privacy coins~\cite{yang2025anonymizing}, mixing services~\cite{lubbertsenghost}, and post-cross-chain fund tracing, as well as to explore its potential for real-time detection.


%\qw{bib comments} 
%关于bib： 1. 有的entry没有journal或者conference信息 2. 有些题目的大写字母要保留 比如Etheruem Menero这种特定的 用花括号括上那个大写的字母 {E}thereum 3. 不是很出名的会议或者期刊 如果是弱相关就去掉好了 比如Mathematics/ieee access啥的 还有很多顶会的可以替代  4. 会议期刊全称保持格式一致 就是全名加简写 这样一眼看上去是refine过的东西 而且有的全称呼不是很熟悉大家 最好加上简写  比如Annual Computer Security Applications Conference (ACSAC) 5. 那个misc和online不知道有何区别 是否需要统一 然后这种网站的 加上个retrieved by Nov 2025时间note 6. [56]这个文章好像引用了两次 不同的label 去掉一个重复的
%以上我调整了部分 整体review一下文章里这几十个哈 



%Flowsheild主要还是在追踪账户模型为主的区块链，所以在交易建模环节和方法模块其实针对的都是账户模型的交易。但是呢，因为有些跨链交易是会把资金跨到UTXO模型的，我们的方法是可以解析到，跨到哪个链，以及对应的地址。但是如果这个链是UTXO-based的，那么我们是无法继续向后追踪的。

==> chapter/8-discussion.tex <==
\section{Discussion}\label{sec:disscusion}



%Timely Intervention Before Funds Become Anonymized. 区块链匿名性技术支持匿名增强洗钱手段，如混币洗钱。匿名增强的洗钱手段通常出现在本文所检测出的洗钱行为之后，且其涉及的资金占比较小。因此，若系统能够及时识别这些匿名增强手段的前序洗钱交易，即可在资金进入完全匿名化阶段前实现有效遏制。例如，在 Bybit hack 案例中，攻击者先通过资金分散、代币换币、合约间接转账及跨链转移等方式，将赃款从以太坊链逐步转移至比特币链，最终仅约 20% 的资金流入混币器以进一步掩盖来源。由此可见，对前序洗钱行为的检测为防范匿名增强洗钱提供了可行路径。

%\heading{Timely Intervention Before Funds Become Anonymized.} 


% \heading{\qw{add one more disucssion?}}


% 阈值影响 为什么这么设置阈值？
% 在 Phase 2（Fund Flow Awareness） 中，我们在构建每个洗钱地址的局部交易子图时引入了三个核心阈值参数：时间窗口阈值、资金流比例阈值（flow ratio threshold） 和 金额相似度阈值（amount similarity threshold）。
% 若阈值设置过大，可能引入大量无关的交易；若阈值设置过小，部分真实的洗钱路径会被截断。
% 我们基于实证统计结果确定了以下阈值设定：
% 时间窗口阈值（24h）：96% 的相邻洗钱交易时间间隔小于 24 小时；
% 资金流比例阈值（≥0.9）：超过 97% 的上游或下游交易金额总额和占目标交易的高于 0.9。
% 金额相似度阈值（≤5%）：相似金额簇内平均偏差为 5%。
% 这些阈值是可调节的参数，用户可对其进行自适应调整，以在不同场景下实现最优的资金流建模效果。
\heading{How we determine threshold parameters?}
In Phase 2 (Fund Flow Awareness), we introduce three threshold parameters when constructing the transaction subgraphs: time window 
$\tau_t$, flow ratio $\tau_f$, and amount similarity $\tau_a$. Setting these thresholds too high may include a large number of irrelevant transactions, while overly strict thresholds may truncate genuine laundering paths. Based on empirical analysis, we determine the following configurations: \textit{i)} approximately 96\% of consecutive laundering transactions occur within 24 hours, so $\tau_t$ is set to 24; \textit{ii)} over 97\% of upstream and downstream transaction value ratios are greater than 0.9,  so $\tau_f$ is set to 0.9; \textit{iii)} the average deviation within similar-amount clusters is about 5\%, so $\tau_a$ is set to 0.05. These thresholds are adjustable and can be adaptively tuned according to different needs to achieve optimal fund-flow modeling performance.


%FlowShield 能否识别不同跨链桥的洗钱交易？ 
%FlowShield 框架支持通用化识别利用多种跨链桥的跨链洗钱。通过解析跨链桥交易的事件日志，系统能够提取目标链、接收地址及跨链资产等信息，从而还原资金的跨链流向。只需要维护跨链桥的合约地址和事件 ABI，即可拓展跨链洗钱检测。
\heading{Can \techName{} detect cross-chain laundering across different bridges?} 
\techName{} provides generalized detection of cross-chain laundering across heterogeneous bridge protocols. By parsing bridge-specific event logs, it extracts the destination chain, recipient address, token identifiers, and locked/released asset values, enabling full reconstruction of cross-chain fund trajectories. This approach works for both lock–mint and burn–redeem designs, as well as router-based multi-hop bridges.

To remain compatible with new or updated protocols, \techName{} only requires an up-to-date registry of bridge contract addresses and event ABIs, making cross-chain laundering detection extensible and maintainable at scale.


%Qin: 都可以 这个主要是把p13那页填满写一个topic或者俩都可以 俩的话就短点
%最后appendix给两个algorithm加点论述介绍啥的吧 填一些字 不然太松了格式上 把algo喂给gpt出文字就可以 然后二次过一下那种 很快
%conclusion你可以看着改 我是之前写的 应该没cover很多新的 conclusion总体上我感觉保持简单 突出这个framwwork的特点 比如可以cover comlicated strategy啥的 然后同时效果很好 这里不用介绍原理了就（比如几个模块啥的）
%Table1如果有能加的就加（原理之类的也可以其实 效果 数据集 任何都可以） 没有就这样也行


% \qw{final comments.} 


% 为什么不用现有数据集呢？为什么要自己收集？
% 如表~\ref{tab:aml_comparison} 所示，现有主流的加密货币反洗钱数据集（如 Elliptic 和 EthereumHeist）均为单链数据集，无法支持跨链洗钱行为的分析与检测。此外，Elliptic 数据集仅提供经过高度归一化的数值特征，缺乏真实的交易细节（如交易金额与时间等）。EthereumHeist 数据集的洗钱标签则来源于启发式规则，而非权威标注，因此可能引入大量假阳性噪声。为克服这些局限，我们构建并发布了 BybitML (2025)——首个基于真实事件的多链洗钱数据集，具有丰富的语义标注、资金流重建与跨链交易覆盖。
% 没提年份最新hh
% \qs{put dataset in intro or discussion sec?}
% 有点想放在intro的Then, we implement and evaluate FLOWSHIELD on our newly curated dataset, BybitML.之后
\heading{Why we need a new dataset?} We have reasons. 
As shown in Table~\ref{tab:aml_comparison}, two mainstream datasets \textit{Elliptic} and \textit{EthereumHesit} are limited to a single chain and therefore cannot support the detection of cross-chain laundering. Moreover, both dataset has limitations. 

\begin{packeditemize}
    \item \textit{Elliptic} only provides highly normalized numerical features and lacks essential transaction details (e.g., amount, time), making it unsuitable for behavior-level analysis. \item \textit{EthereumHesit} derives its laundering labels through heuristic rules rather than authoritative ground truth, which may introduce false-positive noise. 
\end{packeditemize}

Thus, we construct and release \textit{BybitML}, the first multi-chain laundering dataset built from a real-world incident with rich semantic annotations and fund-flow reconstruction.

\heading{Why anonymized AML are seemingly excluded?} Our approach in fact already covers such cases, and in a straightforward way. It operates as a pre-emptive detection mechanism, identifying suspicious assets before they enter anonymity-enhancing laundering stages such as mixers. Empirically, we observe that only a small portion of illicit funds ever reach these stages. For instance, in the Bybit hack case, the launderer dispersed and swapped tokens, performed inter-contract transfers, and conducted cross-chain migrations from Ethereum to Bitcoin. Ultimately, only about 20\% of the stolen assets flowed into mixers to further conceal their origin~\cite{LazarusBounty}. These observations suggest that detecting upstream laundering behaviors  (e.g., fund splitting, frequent token swaps, and cross-chain movements) offers a practical strategy to mitigate anonymity-enhanced laundering.

%Blockchain anonymity technologies enable anonymity-enhancing laundering techniques, such as mixer-based laundering. These anonymity-enhancing methods typically occur after the laundering behaviors detected in this study and involve a relatively small portion of the total funds. Therefore, if the system can promptly identify the precursor laundering transactions preceding these anonymity-enhancing steps, it can effectively intervene before the funds enter the fully anonymized stage. For example, in the Bybit hack case, the attackers first combined fund dispersal, token swaps, indirect contract-based transfers, and cross-chain movements to gradually move stolen assets from Ethereum to Bitcoin, and ultimately only about 20\% of the funds were routed into a mixer to further obscure their origin~\cite{LazarusBounty}. This indicates that detecting precursor laundering behaviors provides a practical and effective means to prevent anonymity-enhancing laundering.

\heading{If we can do more?} While \techName{} has successfully demonstrated strong performance and interpretability in detecting diverse laundering behaviors, we outline following promising directions to extend \techName{}. These directions aim to improve its real-world applicability and expand its coverage of complex laundering behaviors:
\begin{packeditemize}

\item \textit{Real-time \underline{online} detection system.} 
% 当前的检测流程主要在离线环境中运行。未来的工作可进一步将系统扩展为实时的在线检测框架，使其能够持续接收并处理区块链流式数据，对潜在的洗钱交易进行即时识别与预警。这样的端到端系统能够显著缩短检测延迟，提升反洗钱响应的及时性与实用性。
Our current detection process operates primarily in an offline setting, similar to other Crypto AML techniques. Future work will focus on extending the system into a real-time online detection framework capable of continuously ingesting and processing blockchain streaming data. Such an end-to-end system would enable the timely identification and alerting of potential laundering activities, significantly reducing detection latency and improving the responsiveness and practicality of AML operations.


\item \textit{Anonymity-enhanced laundering detection.}
% 我们的 \techName{} 能够识别匿名增强洗钱之前的前序洗钱行为，从而在资金进入完全匿名化阶段前实现有效遏制。未来的研究将进一步探索如何对匿名增强阶段本身进行建模与检测，例如识别混币器的资金关联关系。这将使系统实现对洗钱全流程的更全面覆盖。
Our scheme can identify precursor behaviors that occur before anonymity-enhanced laundering, allowing early intervention before funds become fully anonymized. Future work will explore modeling and detecting the anonymity-enhanced laundering activities such as identifying laundering fund linkages within mixers. This will enable more comprehensive coverage of the entire laundering process.
\end{packeditemize}

% \noindent\textbf{The scope of our study.}~~


% \noindent\textbf{Future work.}~~


==> chapter/A1-ethical.tex <==


% \section*{Ethics Considerations}
% % \textbf{Within up to one page, explain the ethical considerations of your work. This appendix must have exactly this title, otherwise you will risk desk rejection. Carefully study the Ethics Guidelines before submitting your paper.}

% %and it is important to clarify that we do not engage in any exploitative activities.

% %\qw{double check \url{https://sp2026.ieee-security.org/cfpapers.html}}

% \heading{Data source and privacy protection.} We have taken into account the ethical considerations of our study and ensured that every stage of the study adhered to established ethical principles. Specifically, all data used in this work were obtained from publicly accessible blockchain transaction records and contain no personally identifiable information. Blockchain addresses are inherently pseudonymous identifiers, and we did not attempt to perform de-anonymization or track individual identities. 


% \heading{Legal and ethical compliance.} It is important to clarify that we do not engage in any exploitative activities. The primary goal of this research is to enhance the effectiveness and explainability of money laundering detection, thereby supporting compliance teams and regulatory authorities, rather than providing any utility for illicit activities. All experiments were conducted strictly on historical public data, and no attacks, disruptions, or manipulations of real-world systems were involved.


% \heading{Proactive community engagement.}  
% Throughout this study, we proactively engaged with AML stakeholders to validate our findings and ensure responsible disclosure. We reported verified laundering traces to established bounty boards and AML reporting channels (e.g., Lazarus Bounty), facilitating coordinated mitigation efforts while respecting user privacy and jurisdictional compliance boundaries.  Our work contributes to a safer, more transparent, and accountable blockchain ecosystem.

% \section*{Ethical Considerations}

% \heading{Data privacy and protection.}
% All data used in this work come from publicly accessible blockchain transaction records and contain no personally identifiable information. Blockchain addresses are pseudonymous identifiers, and we do not attempt to de-anonymize users or infer real-world identities. We report results at the transaction/address level only as needed for forensic analysis, and avoid publishing any additional linkage information beyond what is already publicly observable on-chain.

% \heading{Consent and human involvement.}
% Our study does not involve interacting with users, collecting private data, or conducting interventions on live systems; all analyses are performed retrospectively on historical public records. The only human involvement is the manual evaluation of SARs by invited experts, which is limited to assessing report quality and does not require access to sensitive personal data.

% \heading{Bias and limitations.}
% We acknowledge potential bias arising from data being drawn from a specific incident and period, as well as class imbalance and evolving laundering behaviors over time. To mitigate over-claiming, we evaluate across multiple days and report multiple metrics (including money coverage rate) to reflect both detection accuracy and financial impact. We position the findings as evidence for the studied setting rather than universal guarantees across all laundering ecosystems.

% \heading{Potential misuse and responsible use.}
% This work is intended to support compliance and forensic investigation, not to facilitate illicit activity. While we describe laundering patterns at a high level, we avoid providing step-by-step operational guidance that would meaningfully lower the barrier for laundering. Any released artifacts (e.g., code/models) are intended for research and defensive use, and should be deployed with appropriate governance, monitoring, and access controls in line with legal and regulatory requirements.

% \heading{Community engagement.}
% When appropriate, we engage with AML stakeholders and responsible reporting channels to support mitigation efforts (e.g., reporting verified traces to established bounty/AML channels) while respecting privacy and jurisdictional boundaries.





% \section{GenAI Disclosure}
% %1. 原创性（Originality）
% % we state: ‘LLMs were used for editorial purposes in this manuscript, and all outputs were inspected by the authors to ensure accuracy and originality. 
% % 在论文撰写过程中，我们仅使用LLM 进行语言润色，不涉及内容生成。 论文中的所有研究内容、方法设计、实验结果、图表与表格均由作者独立完成，所有文献综述和相关工作调研均由作者独立检索、阅读和总结，未借助任何 LLM 工具。

% % 2.透明性
% %我们提出的 FlowShield 框架包含两个使用 LLM 的模块：
% % Semantics–Flow Fusion 模块：使用开源模型 Llama 3 生成交易语义文本的嵌入向量，用于实现语义信息与结构信息的融合。
% % SAR Generation 模块：使用 GPT-4o 模型生成可疑资金流摘要与red flags的自然语言报告，用于SAR的生成。
% % 其中，Llama 3 属于 开源模型（由 Meta 发布），GPT-4o 为 闭源的商用模型（由 OpenAI 提供）。为降低随机性影响，我们固定了LLM的调用参数，并记录了 prompt 模板与相关代码，开源代码仓库中详细记录，以保证复现性。

% %3.责任
% % 数据来源： 所使用的数据全部来自区块链公开可获取的链上交易信息，不涉及任何个人隐私或敏感数据，亦不包含现实世界身份信息。
% % why llm necessary: 利用 LLM 出色的语义理解能力和自然语言生成能力，分别获得文本嵌入和SAR
% % why choose the model: Llama 3 开源、可本地部署，能够在保证性能的同时节约成本; GPT-4o 信息理解和文本生成能力优异，适合生成高质量的洗钱资金流总结与警示标志。
% % 我们严格控制查询与调用次数，确保每个数据样本仅进行一次 LLM 处理，以降低资源消耗。
% % 实验运行环境为： NVIDIA RTX 4090 GPU（24 GB VRAM）与 46 GB 系统内存。

% \heading{Originality.} 
% GenAI was used for editorial purposes in this manuscript, and all outputs were inspected by the authors to ensure accuracy and originality. During the preparation of this manuscript, GenAI was used for language polishing. All other components of the manuscript, including but not limited to research content, figures, tables, or experimental results, were developed without the assistance of GenAI.

% \heading{Transparency.} 
% Our proposed \techName{} framework includes two modules that employ LLMs: (i) The \textit{text–structure fusion} module utilizes the open-source Llama3 model to generate text embeddings of transactions; 
% and (ii) The \textit{SAR generation} module employs GPT-4o to produce natural-language summaries of ML flows and identify red flags, facilitating the creation of structured and explainable SARs. 
% Llama3, released by Meta, is an open-source model that can be executed locally, whereas GPT-4o, provided by OpenAI, is a commercial closed-source model. 
% To reduce stochasticity, we fixed key parameters (e.g., temperature and max tokens) and documented all prompt templates and the relative code in our open-source code repository to facilitate reproducibility and transparency. 

% \heading{Responsibility.} 
% All data used in this study are publicly accessible on-chain transaction records and do not contain any personal, private, or sensitive information. 
% The use of LLMs in \textsc{FlowShield} serves two main purposes: 
% \textit{i)} to leverage the text understanding capabilities of LLMs in generating text embeddings for capturing latent fund-flow intentions during the \textit{Semantics–Flow Fusion} stage;  and \textit{ii)} to utilize their natural-language generation capability to automatically produce structured SARs, improving interpretability and practical usability.  We selected Llama3 for its open-source nature, local deployability, and cost efficiency, and GPT-4o for its superior information reasoning and text generation quality. 
% To minimize environmental impact, each data sample was processed only once by the LLM.  

% % 是否会对bridge users影响大？


% % 对criminal的影响


==> chapter/A2-open-sci.tex <==
\section*{Open Science}
% \textbf{Within up to one page, this appendix must list all artifacts necessary to evaluate the contribution of the paper and make clear how the review committees can access each artifact. This appendix must have exactly this title, otherwise you will risk desk rejection. }


This research complies with the open science policy. We have made the following artifacts available online to replicate our work at:~\url{https://osf.io/nx7aj/?view_only=1b3e2d72e8484abe8ec8bd487256586f}. More details about the Flowshield can be found in "Readme.md".

\begin{itemize}
    \item Code: The full implementation of FlowShield, with modularized code covering all four phases.

    \item Dataset: Transaction data of the BybitHack incident, including  ML and normal transactions spanning 14 days. The processed semantics embeddings and fund flow embeddings are also included.

\end{itemize}



==> chapter/A3-alg.tex <==

% \section{Pseudocode of FlowShield}
% \label{apd-alg}

% \begin{algorithm}[]
% \caption{Semantics Parsing}
% \scriptsize
% \DontPrintSemicolon
% \KwIn{Transaction set $\mathcal{E}$, parsing rules $\mathcal{R}_{swp}$, $\mathcal{R}_{ind}$, $\mathcal{R}_{crs}$, semantics template ${\mathsf{Tmp}}_{s}$}

% \KwOut{Semantics type $\mathsf{S}_k$ and semantics text $\mathsf{Txt}_{sem}$ for each transaction}

% \For{each transaction $t_k$ in $\mathcal{E}$}{
%     \uIf{$\mathcal{R}_{S_{swp}}(t_k)=1$}{
%         $\text{f}_{sem}(t_k) = \text{S}_{swp}$
%     }
%     \uElseIf{$\mathcal{R}_{S_{ind}}(t_k)=1$}{
%         $\text{f}_{sem}(t_k) = \text{S}_{ind}$
%     }
%     \uElseIf{$\mathcal{R}_{S_{crs}}(t_k)=1$}{
%         $\text{f}_{sem}(t_k) = \text{S}_{crs}$
%     }
%     \Else{
%         $\text{f}_{sem}(t_k) = \text{S}_{dir}$
%     }
%     Generate semantics text via the template ${\text{Tmp}}_{s}$.}
% \label{alg:semantics}
% \end{algorithm}


\begin{algorithm}[]
\caption{Fund-flow Construction}
\scriptsize
\DontPrintSemicolon

\label{alg:flow_awareness}

\KwIn{Transaction MultiDiGraph $G $; flow template ${\mathsf{Tmp}}_{f}$; time window 
$\tau_t$, flow ratio $\tau_f$, and amount similarity $\tau_a$}
\KwOut{Upstream subgraph $SubG_{up}$, downstream subgraph $SubG_{down}$, parallel subgraph $SubG_{para}$, flow type $\text{T}_f$, and flow text $\mathsf{Txt}_{flow}$ for each transaction}

\For{each transaction edge $t_{tg} \in E$}{
    \tcp{\textcolor{teal}{Upstream subgraph extraction}}
    % $C_{in} \leftarrow$ incoming transactions to $e_{tg}(from)$ in $G$ before $e_{tg}(time)$ \;
    $C_{in} \leftarrow \mathrm{GetUpCandi}(G, t_{tg}, \tau_t)$ \;
    $\text{Tx}_{up} \leftarrow \{\mathrm{MatchTokenAmount}(C_{in}, t_{tg}, \tau_f) \}$\;
    % $U \leftarrow$ matchAmount($U$, $\tau_f$ \cdot amount$)$\;
    $SubG_{up} \leftarrow$ Subgraph induced by $\text{Tx}_{up} \cup \{ t_{tg} \}$\;
    
    \tcp{\textcolor{teal}{Downstream subgraph extraction}}
    % $C_{out} \leftarrow$ outgoing transactions from $e_{tg}(to)$ in $G$ after $e_{tg}(time)$ \;
    $C_{out} \leftarrow \mathrm{GetDwCandi}(G, t_{tg}, \tau_t)$ \;
    $\text{Tx}_{down} \leftarrow \{\mathrm{MatchTokenAmount}(C_{out}, t_{tg}, \tau_f)\}$\;
    $SubG_{down} \leftarrow$ subgraph induced by $\text{Tx}_{down}  \cup \{ t_{tg} \}$\;
    
    \tcp{\textcolor{teal}{Parallel subgraph extraction}}
    $C_{para} \leftarrow \mathrm{GetPaCandi}(G, t_{tg}, \tau_t)$ \;
    $\text{Tx}_{para}  \leftarrow \{\mathrm{MatchSimilarAmount}(C_{para}, t_{tg}, \tau_a)\}$\;
    $SubG_{para} \leftarrow$ subgraph induced by $\text{Tx}_{para} \cup \{ t_{tg} \}$\;
    
    % \tcp{\textcolor{teal}{Flow type classification}}
    % $sumA_{down} \leftarrow \sum_{e \in \text{Tx}_{down}} e(amount)$\;
    % \uIf{$ sumA_{down} \ge \tau_f \times e_{tg}(amount) $}{
    %     \uIf{$|\text{Tx}_{down}| = 1$}{$\text{T}_f \leftarrow$ single outflow}
    %     \Else{$\text{T}_f \leftarrow$ entire disperse}
    % }
    % \uElseIf{$|\text{Tx}_{para}| > 0$ \textbf{and} $sumA_{down} \ge e_{tg}(amount)$}{
    %     $\text{T}_f \leftarrow$ mix
    % }
    % \uElseIf{$|\text{Tx}_{down}| > 1$ \textbf{and} $sumA_{down} \le \tau_f \times e_{tg}(amount)$}{
    %     $\text{T}_f \leftarrow$ partial disperse
    % }
    % \uElseIf{$|Tx_{down}| = 0$}{
    %     $\text{T}_f \leftarrow$ no forward
    % }

        \tcp{\textcolor{teal}{Flow type classification}}
    $A_{\text{down}} \leftarrow \sum_{e \in \text{Tx}_{down}} e(\text{amount})$\;
    
    \uIf{$|\text{Tx}_{down}| = 0$}{
        $\text{T}_f \leftarrow$ No forward\;
    }
    \uElseIf{$|\text{Tx}_{\text{para}}| > 0$ \textbf{and} $A_{\text{down}} \ge t_{tg}(\text{amount})$}{
        $\text{T}_f \leftarrow$ Mix\;
    }
    \uElseIf{$A_{\text{down}} \ge \tau_f \cdot t_{tg}(\text{amount})$}{
        \uIf{$|\text{Tx}_{down}| = 1$}{
            $\text{T}_f \leftarrow$ Single outflow\;
        }
        \Else{
            $\text{T}_f \leftarrow$ Entire disperse\;
        }
    }
    \ElseIf{$|\text{Tx}_{down}| > 1$ \textbf{and} $A_{\text{down}} < \tau_f \cdot t_{tg}(\text{amount})$}{
        $\text{T}_f \leftarrow$ Partial disperse\;
    }

    
    \tcp{\textcolor{teal}{Flow text generation}}
    Use ${\text{Tmp}}_{f}$ with transaction information, and $\text{T}_f$ to generate flow text\;
}
\end{algorithm}




% Here We show the pseudocode. Algorithm~\ref{alg:semantics} illustrates the process of the semantics parsing module. Algorithm~\ref{alg:flow_awareness} describes the steps in the fund-flow construction stage.

% The semantics parsing module identifies the transaction type by sequentially applying a set of parsing rules. For each transaction, algorithm~\ref{alg:semantics} checks whether it satisfies the predefined patterns of swaps, indirect transfers, or cross-chain migrations. If none of these conditions hold, the transaction is classified as a direct transfer. After determining the semantics type, the module generates a corresponding natural-language description using a predefined template. This procedure ensures that every transaction is assigned both a structured semantics label and a human-readable semantics text.

% % \input{Alg/construct_alg}


% % \input{Alg/semantics_alg}


% The fund-flow construction module analyzes each transaction in the graph to uncover its upstream origins, downstream propagation, and parallel movement patterns. For every transaction, algorithm~\ref{alg:flow_awareness} first identifies candidate upstream, downstream, and parallel transactions within a constrained time window. It then applies flow-ratio and amount-similarity thresholds to filter these candidates and construct three localized subgraphs that reflect how the asset arrived, where it moves next, and whether similar transactions occur in parallel. Based on the aggregated downstream amounts and structural patterns, algorithm~\ref{alg:flow_awareness} categorizes the transaction into a flow type such as single outflow, entire disperse, partial disperse, mix, or no forward. Finally, it uses the flow template to generate a descriptive flow text summarizing the detected movement behavior.


% \input{Alg/construct_alg}

==> chapter/A4-fig-sars.tex <==
\section{Example of SAR}

% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.5\textwidth]{Figs/summary.pdf}
% \end{center}
% \caption{\label{fig:sum_eg} Example of summary of ML process and red flags generated by GPT-4o.}
% \end{figure}

% Figure~\ref{fig:sum_eg} shows the description of ML flow generated by GPT-4o, in which the left panel presents the fund flow summary, outlining key phases from fund injection to conversion and distribution, while the right panel lists red flags that reveal various potential high-risk patterns, such as rapid multi-hop transfers, repeated swaps, identical chunk sizes, and account reuse. 
% \begin{figure*}[t]
% \begin{center}
% \includegraphics[width=1\textwidth]{Figs/sar_summary.pdf}
% \end{center}
% \caption{\label{fig:sum_eg} Example of summary of ML process and red flags generated by GPT-4o.}
% \end{figure*}


% \begin{figure}[]
% \centering
% \begin{subfigure}{0.48\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{Figs/sar_summary-up.pdf}
%   \caption{}
%   \label{fig:up}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.48\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{Figs/sar_summary-down.pdf}
%   \caption{}
%   \label{fig:down}
% \end{subfigure}
% \caption{ Example of summary of ML process and red flags generated by GPT-4o.}
% \label{fig:flow_eg_new}
% \end{figure}


Here we present a SAR example of one laundering flow detected by \techName{}. 

Figure~\ref{fig:up} visualizes how illicit funds propagate through the transaction path. The flow spans four hops, beginning from a single upstream source and subsequently being transferred and swapped through a sequence of intermediary addresses. At the final stage, the funds are dispersed into multiple recipient addresses, forming a clear entire–disperse pattern.


Figure~\ref{fig:middle} presents a structured summary of the detected laundering flow. It outlines the overall process of how the illicit stETH is injected, converted, routed, and ultimately dispersed across multiple accounts. The summary also provides an estimate of the total amount laundered, offering a clear and interpretable overview of the entire laundering flow.

Figure~\ref{fig:down} highlights the red-flag indicators identified in the flow. These indicators highlight suspicious behavioral patterns such as rapid fund movement, repeated token swaps, identical distribution chunk sizes, and recurrent reuse of the same intermediary contracts. The report also identifies signs of centralized coordination and potential automation. Together, these red flags provide an interpretable justification for why the flow is flagged as laundering.

% \begin{figure}[]
% \centering
% \begin{subfigure}{0.47\textwidth}
%   \centering
%   % \includegraphics[width=\textwidth]{Figs/tx_flow_big.pdf}
%   \includegraphics[width=\textwidth]{Figs/eg_flow_frame.pdf}
%   \caption{Sankey diagram of ML flow.}
%   \label{fig:up}
% \end{subfigure}

% \begin{subfigure}{0.46\textwidth}
%   \centering
%   % \includegraphics[width=\textwidth]{Figs/sar_summary-up.pdf}
%   \includegraphics[width=\textwidth]{Figs/summary_new.pdf}
%   \caption{Summary of ML flow.}
%   \label{fig:middle}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.47\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{Figs/redflags.pdf}
%   \caption{Red flag indicators.}
%   \label{fig:down}
% \end{subfigure}
% \caption{ An example of SAR of money laundering flow.}
% \label{fig:summary_new}
% \end{figure}

% ---------- 图 1：Sankey ----------
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/eg_flow_frame.pdf}
\caption{Sankey diagram of a money laundering flow.}
\label{fig:up}
\end{figure}

% ---------- 图 2：Summary ----------
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{Figs/summary_new.pdf}
\caption{Summary of the money laundering flow.}
\label{fig:middle}
\end{figure}

% ---------- 图 3：Red Flags ----------
% 如果你想这张更大，可以用 figure* 让它跨双栏
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{Figs/redflags.pdf}
\caption{Red-flag indicators associated with the money laundering flow.}
\label{fig:down}
\end{figure}


==> chapter/additional_text.tex <==
This flow has reached an unprecedented economic scale; in 2025 alone, illicit cryptocurrency volumes reached record highs, with approximately USD 158 billion in value moving through various obfuscation pipelines \cite{chainalysis2025}. While illicit activity often constitutes a small fraction of total on-chain volume, the concentration of these funds in professionalized laundering-as-a-service (LaaS) networks, such as Chinese-language money laundering ecosystems (CMLNs), which processed an estimated USD 16.1 billion in 2025, poses a systemic risk to market integrity \cite{chainalysis2026cmln, bis_bulletin_111}. These ecosystems operate through distinct service typologies, ranging from ``running point'' brokers who act as initial entry channels to ``money mule motorcades'' that execute complex layering schemes via networks of rented bank accounts and digital wallets. A prominent mechanism within this economy is the ``Black U'' service, where vendors purchase illicit stablecoins (like USDT) at a discount and utilize automated swapping infrastructure to clear large transactions \cite{chainalysis2026cmln, chainalysis2025}. To mitigate counterparty risk in this underground market, these vendors often operate on ``guarantee platforms'' like Huione, which function as illicit escrow services to insure transactions between criminals.

For financial institutions and Virtual Asset Service Providers (VASPs), this professionalization has resulted in a staggering compliance burden. Global financial crime compliance costs have surged, driven by intensified regulatory scrutiny and the quadrupling of global financial penalties \cite{bis_bulletin_111, fatf2025targeted}. The operational challenge is exacerbated by ``alert fatigue,'' where existing rule-based anti-money laundering (AML) frameworks suffer from error rates as high as 95--99\%, mistakenly flagging legitimate accounts and creating massive operational waste \cite{bis_bulletin_111, kykynezhdy2024}. This inefficiency stems from a fundamental inability to manage the ``trace discontinuity'' inherent in modern laundering, where assets are fragmented across decentralized finance (DeFi) protocols and cross-chain bridges \cite{huo2025shedding, fu2025sok}.

Current regulatory frameworks face a critical ``sunrise issue,'' where the inconsistent implementation of global standards, such as the FATF Travel Rule, creates fragmented compliance environments that illicit actors actively exploit \cite{fatf2025targeted}. Significant gaps persist; a substantial number of jurisdictions have yet to implement basic VASP licensing or risk assessment regimes, allowing criminal networks to leverage ``jurisdictional arbitrage'' by routing funds through non-compliant offshore exchanges or regions with weak enforcement \cite{fatf2025targeted, dupuis2021money}. Furthermore, the traditional intermediary-based regulatory model is increasingly strained by DeFi, where regulators struggle to identify responsible entities (VASPs) within automated protocols, leaving vast portions of the ecosystem effectively unsupervised \cite{remolina2024defi, fatf2025targeted}. This disconnect is exacerbated by a ``regulatory dialectic,'' where static compliance frameworks fail to keep pace with illicit actors who rapidly adopt privacy-enhancing technologies, such as mixers and cross-chain bridges, to evade detection \cite{dupuis2021money, huo2025shedding, ofsi2025crypto}.

The defining trend of 2025, ``chain-hopping,'' illustrates this gap in real time. Large-scale security incidents, most notably the February 2025 Bybit heist involving the theft of approximately USD 1.5 billion in Ethereum, showcase how attackers use internal contract calls and cross-chain swaps to break traditional value-continuity boundaries \cite{ding2026bybit, huo2025shedding}. For the business sector, these ``fragmented trails'' represent more than a security risk; they capture vital liquidity and complicate the integration of digital assets into mainstream economic activity. Consequently, there is an urgent demand for ``semantics-aware'' and ``fund-flow-aware'' detection models that can provide the explainable forensic evidence required for institutional-grade compliance and global regulatory standards.

